Candidate strongly lensed type Ia supernovae in the Zwicky Transient Facility archive

Gravitationally lensed type Ia supernovae (glSNe Ia) are unique astronomical tools that can be used to study cosmological parameters, distributions of dark matter, the astrophysics of the supernovae, and the intervening lensing galaxies themselves. A small number of highly magnified glSNe Ia have been discovered by ground-based telescopes such as the Zwicky Transient Facility (ZTF), but simulations predict that a fainter population may also exist. We present a systematic search for glSNe Ia in the ZTF archive of alerts distributed from June 1 2019 to September 1 2022. Using the AMPEL platform, we developed a pipeline that distinguishes candidate glSNe Ia from other variable sources. Initial cuts were applied to the ZTF alert photometry before forced photometry was obtained for the remaining candidates. Additional cuts were applied to refine the candidates based on their light curve colours, lens galaxy colours, and the resulting parameters from fits to the SALT2 SN Ia template. The candidates were also cross-matched with the DESI spectroscopic catalogue. Seven transients were identified that had an associated galaxy DESI redshift, which we present as glSN Ia candidates. Although superluminous supernovae (SLSNe) cannot be fully rejected as contaminants, two events, ZTF19abpjicm and ZTF22aahmovu, are significantly different from typical SLSNe and their light curves can be modelled as two-image glSN Ia systems. From this two-image modelling, we estimate time delays of 22 $\pm$ 3 and 34 $\pm$ 1 days for the two events, respectively, which suggests that we have uncovered a population of glSNe Ia with longer time delays. The pipeline is currently being applied to the live ZTF alert stream to identify and follow-up future candidates while active, and it could be the foundation for glSNe Ia searches in future surveys, such as the Rubin Observatory Legacy Survey of Space and Time.

==> aanda <==
@ARTICLE{Ahn2012a,
   author = {{Ahn}, C.~P. and {Alexandroff}, R. and {Allende Prieto}, C. and
	{Anderson}, S.~F. and {Anderton}, T. and {Andrews}, B.~H. and
	{Aubourg}, {\'E}. and {Bailey}, S. and {Balbinot}, E. and {Barnes}, R. and et al.},
    title = "{The Ninth Data Release of the Sloan Digital Sky Survey: First Spectroscopic Data from the SDSS-III Baryon Oscillation Spectroscopic Survey}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1207.7137},
 primaryClass = "astro-ph.IM",
 keywords = {atlases, catalogs, surveys },
     year = 2012,
    month = dec,
   volume = 203,
      eid = {21},
    pages = {21},
      doi = {10.1088/0067-0049/203/2/21},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJS..203...21A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Arendse2024,
       author = {{Arendse}, Nikki and {Dhawan}, Suhail and {Sagu{\'e}s Carracedo}, Ana and {Peiris}, Hiranya V. and {Goobar}, Ariel and {Wojtak}, Radek and {Alves}, Catarina and {Biswas}, Rahul and {Huber}, Simon and {Birrer}, Simon and {The LSST Dark Energy Science Collaboration}},
        title = "{Detecting strongly lensed type Ia supernovae with LSST}",
      journal = {\mnras},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2024,
        month = jul,
       volume = {531},
       number = {3},
        pages = {3509-3523},
          doi = {10.1093/mnras/stae1356},
archivePrefix = {arXiv},
       eprint = {2312.04621},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024MNRAS.531.3509A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Ashall2021,
       author = {{Ashall}, C. and {Lu}, J. and {Hsiao}, E.~Y. and {Hoeflich}, P. and {Phillips}, M.~M. and {Galbany}, L. and {Burns}, C.~R. and {Contreras}, C. and {Krisciunas}, K. and {Morrell}, N. and {Stritzinger}, M.~D. and {Suntzeff}, N.~B. and {Taddia}, F. and {Anais}, J. and {Baron}, E. and {Brown}, P.~J. and {Busta}, L. and {Campillay}, A. and {Castell{\'o}n}, S. and {Corco}, C. and {Davis}, S. and {Folatelli}, G. and {F{\"o}rster}, F. and {Freedman}, W.~L. and {Gonzal{\'e}z}, C. and {Hamuy}, M. and {Holmbo}, S. and {Kirshner}, R.~P. and {Kumar}, S. and {Marion}, G.~H. and {Mazzali}, P. and {Morokuma}, T. and {Nugent}, P.~E. and {Persson}, S.~E. and {Piro}, A.~L. and {Roth}, M. and {Salgado}, F. and {Sand}, D.~J. and {Seron}, J. and {Shahbandeh}, M. and {Shappee}, B.~J.},
        title = "{Carnegie Supernova Project: The First Homogeneous Sample of Super-Chandrasekhar-mass/2003fg-like Type Ia Supernovae}",
      journal = {\apj},
     keywords = {1728, 1668, 2109, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = dec,
       volume = {922},
       number = {2},
          eid = {205},
        pages = {205},
          doi = {10.3847/1538-4357/ac19ac},
archivePrefix = {arXiv},
       eprint = {2106.12140},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...922..205A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ashton2019,
       author = {{Ashton}, Gregory and {H{\"u}bner}, Moritz and {Lasky}, Paul D. and {Talbot}, Colm and {Ackley}, Kendall and {Biscoveanu}, Sylvia and {Chu}, Qi and {Divakarla}, Atul and {Easter}, Paul J. and {Goncharov}, Boris and {Hernandez Vivanco}, Francisco and {Harms}, Jan and {Lower}, Marcus E. and {Meadors}, Grant D. and {Melchor}, Denyz and {Payne}, Ethan and {Pitkin}, Matthew D. and {Powell}, Jade and {Sarin}, Nikhil and {Smith}, Rory J.~E. and {Thrane}, Eric},
        title = "{BILBY: A User-friendly Bayesian Inference Library for Gravitational-wave Astronomy}",
      journal = {\apjs},
     keywords = {gravitational waves, methods: data analysis, methods: statistical, stars: black holes, stars: neutron, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - High Energy Astrophysical Phenomena, General Relativity and Quantum Cosmology},
         year = 2019,
        month = apr,
       volume = {241},
       number = {2},
          eid = {27},
        pages = {27},
          doi = {10.3847/1538-4365/ab06fc},
archivePrefix = {arXiv},
       eprint = {1811.02042},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJS..241...27A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Assef2018,
       author = {{Assef}, R.~J. and {Stern}, D. and {Noirot}, G. and {Jun}, H.~D. and {Cutri}, R.~M. and {Eisenhardt}, P.~R.~M.},
        title = "{The WISE AGN Catalog}",
      journal = {\apjs},
     keywords = {galaxies: active, infrared: general, quasars: general, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2018,
        month = feb,
       volume = {234},
       number = {2},
          eid = {23},
        pages = {23},
          doi = {10.3847/1538-4365/aaa00a},
archivePrefix = {arXiv},
       eprint = {1706.09901},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJS..234...23A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bag2021,
       author = {{Bag}, Satadru and {Kim}, Alex G. and {Linder}, Eric V. and {Shafieloo}, Arman},
        title = "{Be It Unresolved: Measuring Time Delays from Lensed Supernovae}",
      journal = {\apj},
     keywords = {Strong gravitational lensing, Type Ia supernovae, Astrostatistics techniques, Cosmology, Sky surveys, Supernovae, 1643, 1728, 1886, 343, 1464, 1668, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = mar,
       volume = {910},
       number = {1},
          eid = {65},
        pages = {65},
          doi = {10.3847/1538-4357/abe238},
archivePrefix = {arXiv},
       eprint = {2010.03774},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...910...65B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@software{Barbary2021,
       author = {{Barbary}, Kyle},
        title = "{nestle: Nested sampling algorithms for evaluating Bayesian evidence}",
 howpublished = {Astrophysics Source Code Library, record ascl:2103.022},
         year = 2021,
        month = mar,
          eid = {ascl:2103.022},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ascl.soft03022B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Beck2021,
       author = {{Beck}, R{\'o}bert and {Szapudi}, Istv{\'a}n and {Flewelling}, Heather and {Holmberg}, Conrad and {Magnier}, Eugene and {Chambers}, Kenneth C.},
        title = "{PS1-STRM: neural network source classification and photometric redshift catalogue for PS1 3{\ensuremath{\pi}} DR1}",
      journal = {\mnras},
     keywords = {methods: data analysis, methods: numerical, catalogues, large-scale structure of Universe, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = jan,
       volume = {500},
       number = {2},
        pages = {1633-1644},
          doi = {10.1093/mnras/staa2587},
archivePrefix = {arXiv},
       eprint = {1910.10167},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.500.1633B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Bellm2019a,
       author = {{Bellm}, Eric C. and {Kulkarni}, Shrinivas R. and {Graham}, Matthew J. and {Dekany}, Richard and {Smith}, Roger M. and {Riddle}, Reed and {Masci}, Frank J. and {Helou}, George and {Prince}, Thomas A. and {Adams}, Scott M. and {Barbarino}, C. and {Barlow}, Tom and {Bauer}, James and {Beck}, Ron and {Belicki}, Justin and {Biswas}, Rahul and {Blagorodnova}, Nadejda and {Bodewits}, Dennis and {Bolin}, Bryce and {Brinnel}, Valery and {Brooke}, Tim and {Bue}, Brian and {Bulla}, Mattia and {Burruss}, Rick and {Cenko}, S. Bradley and {Chang}, Chan-Kao and {Connolly}, Andrew and {Coughlin}, Michael and {Cromer}, John and {Cunningham}, Virginia and {De}, Kishalay and {Delacroix}, Alex and {Desai}, Vandana and {Duev}, Dmitry A. and {Eadie}, Gwendolyn and {Farnham}, Tony L. and {Feeney}, Michael and {Feindt}, Ulrich and {Flynn}, David and {Franckowiak}, Anna and {Frederick}, S. and {Fremling}, C. and {Gal-Yam}, Avishay and {Gezari}, Suvi and {Giomi}, Matteo and {Goldstein}, Daniel A. and {Golkhou}, V. Zach and {Goobar}, Ariel and {Groom}, Steven and {Hacopians}, Eugean and {Hale}, David and {Henning}, John and {Ho}, Anna Y.~Q. and {Hover}, David and {Howell}, Justin and {Hung}, Tiara and {Huppenkothen}, Daniela and {Imel}, David and {Ip}, Wing-Huen and {Ivezi{\'c}}, {\v{Z}}eljko and {Jackson}, Edward and {Jones}, Lynne and {Juric}, Mario and {Kasliwal}, Mansi M. and {Kaspi}, S. and {Kaye}, Stephen and {Kelley}, Michael S.~P. and {Kowalski}, Marek and {Kramer}, Emily and {Kupfer}, Thomas and {Landry}, Walter and {Laher}, Russ R. and {Lee}, Chien-De and {Lin}, Hsing Wen and {Lin}, Zhong-Yi and {Lunnan}, Ragnhild and {Giomi}, Matteo and {Mahabal}, Ashish and {Mao}, Peter and {Miller}, Adam A. and {Monkewitz}, Serge and {Murphy}, Patrick and {Ngeow}, Chow-Choong and {Nordin}, Jakob and {Nugent}, Peter and {Ofek}, Eran and {Patterson}, Maria T. and {Penprase}, Bryan and {Porter}, Michael and {Rauch}, Ludwig and {Rebbapragada}, Umaa and {Reiley}, Dan and {Rigault}, Mickael and {Rodriguez}, Hector and {van Roestel}, Jan and {Rusholme}, Ben and {van Santen}, Jakob and {Schulze}, S. and {Shupe}, David L. and {Singer}, Leo P. and {Soumagnac}, Maayane T. and {Stein}, Robert and {Surace}, Jason and {Sollerman}, Jesper and {Szkody}, Paula and {Taddia}, F. and {Terek}, Scott and {Van Sistine}, Angela and {van Velzen}, Sjoert and {Vestrand}, W. Thomas and {Walters}, Richard and {Ward}, Charlotte and {Ye}, Quan-Zhi and {Yu}, Po-Chieh and {Yan}, Lin and {Zolkower}, Jeffry},
        title = "{The Zwicky Transient Facility: System Overview, Performance, and First Results}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2019,
        month = jan,
       volume = {131},
       number = {995},
        pages = {018002},
          doi = {10.1088/1538-3873/aaecbe},
archivePrefix = {arXiv},
       eprint = {1902.01932},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PASP..131a8002B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bellm2019b,
       author = {{Bellm}, Eric C. and {Kulkarni}, Shrinivas R. and {Barlow}, Tom and {Feindt}, Ulrich and {Graham}, Matthew J. and {Goobar}, Ariel and {Kupfer}, Thomas and {Ngeow}, Chow-Choong and {Nugent}, Peter and {Ofek}, Eran and {Prince}, Thomas A. and {Riddle}, Reed and {Walters}, Richard and {Ye}, Quan-Zhi},
        title = "{The Zwicky Transient Facility: Surveys and Scheduler}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2019,
        month = jun,
       volume = {131},
       number = {1000},
        pages = {068003},
          doi = {10.1088/1538-3873/ab0c2a},
archivePrefix = {arXiv},
       eprint = {1905.02209},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PASP..131f8003B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Betoule2014,
       author = {{Betoule}, M. and {Kessler}, R. and {Guy}, J. and {Mosher}, J. and {Hardin}, D. and {Biswas}, R. and {Astier}, P. and {El-Hage}, P. and {Konig}, M. and {Kuhlmann}, S. and {Marriner}, J. and {Pain}, R. and {Regnault}, N. and {Balland}, C. and {Bassett}, B.~A. and {Brown}, P.~J. and {Campbell}, H. and {Carlberg}, R.~G. and {Cellier-Holzem}, F. and {Cinabro}, D. and {Conley}, A. and {D'Andrea}, C.~B. and {DePoy}, D.~L. and {Doi}, M. and {Ellis}, R.~S. and {Fabbro}, S. and {Filippenko}, A.~V. and {Foley}, R.~J. and {Frieman}, J.~A. and {Fouchez}, D. and {Galbany}, L. and {Goobar}, A. and {Gupta}, R.~R. and {Hill}, G.~J. and {Hlozek}, R. and {Hogan}, C.~J. and {Hook}, I.~M. and {Howell}, D.~A. and {Jha}, S.~W. and {Le Guillou}, L. and {Leloudas}, G. and {Lidman}, C. and {Marshall}, J.~L. and {M{\"o}ller}, A. and {Mour{\~a}o}, A.~M. and {Neveu}, J. and {Nichol}, R. and {Olmstead}, M.~D. and {Palanque-Delabrouille}, N. and {Perlmutter}, S. and {Prieto}, J.~L. and {Pritchet}, C.~J. and {Richmond}, M. and {Riess}, A.~G. and {Ruhlmann-Kleider}, V. and {Sako}, M. and {Schahmaneche}, K. and {Schneider}, D.~P. and {Smith}, M. and {Sollerman}, J. and {Sullivan}, M. and {Walton}, N.~A. and {Wheeler}, C.~J.},
        title = "{Improved cosmological constraints from a joint analysis of the SDSS-II and SNLS supernova samples}",
      journal = {\aap},
     keywords = {cosmology: observations, distance scale, dark energy, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = aug,
       volume = {568},
          eid = {A22},
        pages = {A22},
          doi = {10.1051/0004-6361/201423413},
archivePrefix = {arXiv},
       eprint = {1401.4064},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...568A..22B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bilicki2014,
       author = {{Bilicki}, Maciej and {Jarrett}, Thomas H. and {Peacock}, John A. and {Cluver}, Michelle E. and {Steward}, Louise},
        title = "{Two Micron All Sky Survey Photometric Redshift Catalog: A Comprehensive Three-dimensional Census of the Whole Sky}",
      journal = {\apjs},
     keywords = {catalogs, galaxies: distances and redshifts, large-scale structure of universe, methods: data analysis, methods: statistical, surveys, Astrophysics - Cosmology and Extragalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2014,
        month = jan,
       volume = {210},
       number = {1},
          eid = {9},
        pages = {9},
          doi = {10.1088/0067-0049/210/1/9},
archivePrefix = {arXiv},
       eprint = {1311.5246},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJS..210....9B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bilicki2016,
       author = {{Bilicki}, Maciej and {Peacock}, John A. and {Jarrett}, Thomas H. and {Cluver}, Michelle E. and {Maddox}, Natasha and {Brown}, Michael J.~I. and {Taylor}, Edward N. and {Hambly}, Nigel C. and {Solarz}, Aleksandra and {Holwerda}, Benne W. and {Baldry}, Ivan and {Loveday}, Jon and {Moffett}, Amanda and {Hopkins}, Andrew M. and {Driver}, Simon P. and {Alpaslan}, Mehmet and {Bland-Hawthorn}, Joss},
        title = "{WISE {\texttimes} SuperCOSMOS Photometric Redshift Catalog: 20 Million Galaxies over 3/pi Steradians}",
      journal = {\apjs},
     keywords = {catalogs, galaxies: distances and redshifts, large-scale structure of universe, methods: data analysis, methods: statistical, surveys, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2016,
        month = jul,
       volume = {225},
       number = {1},
          eid = {5},
        pages = {5},
          doi = {10.3847/0067-0049/225/1/5},
archivePrefix = {arXiv},
       eprint = {1607.01182},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJS..225....5B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Birrer2022,
       author = {{Birrer}, Simon and {Dhawan}, Suhail and {Shajib}, Anowar J.},
        title = "{The Hubble Constant from Strongly Lensed Supernovae with Standardizable Magnifications}",
      journal = {\apj},
     keywords = {758, 1643, 1668, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2022,
        month = jan,
       volume = {924},
       number = {1},
          eid = {2},
        pages = {2},
          doi = {10.3847/1538-4357/ac323a},
archivePrefix = {arXiv},
       eprint = {2107.12385},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022ApJ...924....2B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Blagorodnova2018,
       author = {{Blagorodnova}, Nadejda and {Neill}, James D. and {Walters}, Richard and {Kulkarni}, Shrinivas R. and {Fremling}, Christoffer and {Ben-Ami}, Sagi and {Dekany}, Richard G. and {Fucik}, Jason R. and {Konidaris}, Nick and {Nash}, Reston and {Ngeow}, Chow-Choong and {Ofek}, Eran O. and {O' Sullivan}, Donal and {Quimby}, Robert and {Ritter}, Andreas and {Vyhmeister}, Karl E.},
        title = "{The SED Machine: A Robotic Spectrograph for Fast Transient Classification}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = mar,
       volume = {130},
       number = {985},
        pages = {035003},
          doi = {10.1088/1538-3873/aaa53f},
archivePrefix = {arXiv},
       eprint = {1710.02917},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018PASP..130c5003B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Brescia2015,
       author = {{Brescia}, M. and {Cavuoti}, S. and {Longo}, G.},
        title = "{Automated physical classification in the SDSS DR10. A catalogue of candidate quasars}",
      journal = {\mnras},
     keywords = {methods: data analysis, techniques: photometric, catalogues, galaxies: active, quasars: general, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2015,
        month = jul,
       volume = {450},
       number = {4},
        pages = {3893-3903},
          doi = {10.1093/mnras/stv854},
archivePrefix = {arXiv},
       eprint = {1504.03857},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.450.3893B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Byler2017a,
       author = {{Byler}, Nell and {Dalcanton}, Julianne J. and {Conroy}, Charlie and
         {Johnson}, Benjamin D.},
        title = "{Nebular Continuum and Line Emission in Stellar Population Synthesis Models}",
      journal = {\apj},
     keywords = {galaxies: abundances, galaxies: ISM, galaxies: star formation, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = may,
       volume = {840},
       number = {1},
          eid = {44},
        pages = {44},
          doi = {10.3847/1538-4357/aa6c66},
archivePrefix = {arXiv},
       eprint = {1611.08305},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...840...44B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Calzetti2000a,
   author = {{Calzetti}, D. and {Armus}, L. and {Bohlin}, R.~C. and {Kinney}, A.~L. and 
	{Koornneef}, J. and {Storchi-Bergmann}, T.},
    title = "{The Dust Content and Opacity of Actively Star-forming Galaxies}",
  journal = {\apj},
   eprint = {astro-ph/9911459},
 keywords = {GALAXIES: STARBURST, INFRARED: GALAXIES, INFRARED: ISM: CONTINUUM, ISM: DUST, EXTINCTION},
     year = 2000,
    month = apr,
   volume = 533,
    pages = {682-695},
      doi = {10.1086/308692},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...533..682C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chabrier2003a,
   author = {{Chabrier}, G.},
    title = "{Galactic Stellar and Substellar Initial Mass Function}",
  journal = {\pasp},
   eprint = {astro-ph/0304382},
 keywords = {Galaxies: Luminosity Function, Mass Function, Invited Reviews},
     year = 2003,
    month = jul,
   volume = 115,
    pages = {763},
      doi = {10.1086/376392},
   adsurl = {http://adsabs.harvard.edu/abs/2003PASP..115..763C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chakradhari2014,
       author = {{Chakradhari}, N.~K. and {Sahu}, D.~K. and {Srivastav}, S. and {Anupama}, G.~C.},
        title = "{Supernova SN 2012dn: a spectroscopic clone of SN 2006gz}",
      journal = {\mnras},
     keywords = {techniques: photometric, techniques: spectroscopic, supernovae: general, supernovae: individual: SN 2012dn- galaxies: individual: ESO 462-016, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = sep,
       volume = {443},
       number = {2},
        pages = {1663-1679},
          doi = {10.1093/mnras/stu1258},
archivePrefix = {arXiv},
       eprint = {1406.6139},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.443.1663C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Chambers2016a,
       author = {{Chambers}, K.~C. and {Magnier}, E.~A. and {Metcalfe}, N. and {Flewelling}, H.~A. and {Huber}, M.~E. and {Waters}, C.~Z. and {Denneau}, L. and {Draper}, P.~W. and {Farrow}, D. and {Finkbeiner}, D.~P. and {Holmberg}, C. and {Koppenhoefer}, J. and {Price}, P.~A. and {Rest}, A. and {Saglia}, R.~P. and {Schlafly}, E.~F. and {Smartt}, S.~J. and {Sweeney}, W. and {Wainscoat}, R.~J. and {Burgett}, W.~S. and {Chastel}, S. and {Grav}, T. and {Heasley}, J.~N. and {Hodapp}, K.~W. and {Jedicke}, R. and {Kaiser}, N. and {Kudritzki}, R. -P. and {Luppino}, G.~A. and {Lupton}, R.~H. and {Monet}, D.~G. and {Morgan}, J.~S. and {Onaka}, P.~M. and {Shiao}, B. and {Stubbs}, C.~W. and {Tonry}, J.~L. and {White}, R. and {Ba{\~n}ados}, E. and {Bell}, E.~F. and {Bender}, R. and {Bernard}, E.~J. and {Boegner}, M. and {Boffi}, F. and {Botticella}, M.~T. and {Calamida}, A. and {Casertano}, S. and {Chen}, W. -P. and {Chen}, X. and {Cole}, S. and {Deacon}, N. and {Frenk}, C. and {Fitzsimmons}, A. and {Gezari}, S. and {Gibbs}, V. and {Goessl}, C. and {Goggia}, T. and {Gourgue}, R. and {Goldman}, B. and {Grant}, P. and {Grebel}, E.~K. and {Hambly}, N.~C. and {Hasinger}, G. and {Heavens}, A.~F. and {Heckman}, T.~M. and {Henderson}, R. and {Henning}, T. and {Holman}, M. and {Hopp}, U. and {Ip}, W. -H. and {Isani}, S. and {Jackson}, M. and {Keyes}, C.~D. and {Koekemoer}, A.~M. and {Kotak}, R. and {Le}, D. and {Liska}, D. and {Long}, K.~S. and {Lucey}, J.~R. and {Liu}, M. and {Martin}, N.~F. and {Masci}, G. and {McLean}, B. and {Mindel}, E. and {Misra}, P. and {Morganson}, E. and {Murphy}, D.~N.~A. and {Obaika}, A. and {Narayan}, G. and {Nieto-Santisteban}, M.~A. and {Norberg}, P. and {Peacock}, J.~A. and {Pier}, E.~A. and {Postman}, M. and {Primak}, N. and {Rae}, C. and {Rai}, A. and {Riess}, A. and {Riffeser}, A. and {Rix}, H.~W. and {R{\"o}ser}, S. and {Russel}, R. and {Rutz}, L. and {Schilbach}, E. and {Schultz}, A.~S.~B. and {Scolnic}, D. and {Strolger}, L. and {Szalay}, A. and {Seitz}, S. and {Small}, E. and {Smith}, K.~W. and {Soderblom}, D.~R. and {Taylor}, P. and {Thomson}, R. and {Taylor}, A.~N. and {Thakar}, A.~R. and {Thiel}, J. and {Thilker}, D. and {Unger}, D. and {Urata}, Y. and {Valenti}, J. and {Wagner}, J. and {Walder}, T. and {Walter}, F. and {Watters}, S.~P. and {Werner}, S. and {Wood-Vasey}, W.~M. and {Wyse}, R.},
        title = "{The Pan-STARRS1 Surveys}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = dec,
          eid = {arXiv:1612.05560},
        pages = {arXiv:1612.05560},
archivePrefix = {arXiv},
       eprint = {1612.05560},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016arXiv161205560C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chang2024,
       author = {{Chang}, Janet N.~Y. and {Dai}, Lixin and {Pfister}, Hugo and {Chowdhury}, Rudrani Kar and {Natarajan}, Priyamvada},
        title = "{Rates of Stellar Tidal Disruption Events Around Intermediate-Mass Black Holes}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2024,
        month = jul,
          eid = {arXiv:2407.09339},
        pages = {arXiv:2407.09339},
          doi = {10.48550/arXiv.2407.09339},
archivePrefix = {arXiv},
       eprint = {2407.09339},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024arXiv240709339C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Chen2017,
       author = {{Chen}, Ting-Wan and {Smartt}, Stephen J. and {Yates}, Rob M. and {Nicholl}, Matt and {Kr{\"u}hler}, Thomas and {Schady}, Patricia and {Dennefeld}, Michel and {Inserra}, Cosimo},
        title = "{Superluminous supernova progenitors have a half-solar metallicity threshold}",
      journal = {\mnras},
     keywords = {stars: magnetars, supernovae: general, supernovae: individual (SN 2011ke, SN 2012il, SN 2015bn, Gaia16apd), galaxies: abundances, galaxies: dwarf, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = sep,
       volume = {470},
       number = {3},
        pages = {3566-3573},
          doi = {10.1093/mnras/stx1428},
archivePrefix = {arXiv},
       eprint = {1605.04925},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.470.3566C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Childress2011,
       author = {{Childress}, M. and {Aldering}, G. and {Aragon}, C. and {Antilogus}, P. and {Bailey}, S. and {Baltay}, C. and {Bongard}, S. and {Buton}, C. and {Canto}, A. and {Chotard}, N. and {Copin}, Y. and {Fakhouri}, H.~K. and {Gangler}, E. and {Kerschhaggl}, M. and {Kowalski}, M. and {Hsiao}, E.~Y. and {Loken}, S. and {Nugent}, P. and {Paech}, K. and {Pain}, R. and {Pecontal}, E. and {Pereira}, R. and {Perlmutter}, S. and {Rabinowitz}, D. and {Runge}, K. and {Scalzo}, R. and {Thomas}, R.~C. and {Smadja}, G. and {Tao}, C. and {Weaver}, B.~A. and {Wu}, C.},
        title = "{Keck Observations of the Young Metal-poor Host Galaxy of the Super-Chandrasekhar-mass Type Ia Supernova SN 2007if}",
      journal = {\apj},
     keywords = {galaxies: dwarf, supernovae: general, supernovae: individual: SN 2007if, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = may,
       volume = {733},
       number = {1},
          eid = {3},
        pages = {3},
          doi = {10.1088/0004-637X/733/1/3},
archivePrefix = {arXiv},
       eprint = {1103.2324},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...733....3C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Chornock2013,
       author = {{Chornock}, R. and {Berger}, E. and {Rest}, A. and {Milisavljevic}, D. and {Lunnan}, R. and {Foley}, R.~J. and {Soderberg}, A.~M. and {Smartt}, S.~J. and {Burgasser}, A.~J. and {Challis}, P. and {Chomiuk}, L. and {Czekala}, I. and {Drout}, M. and {Fong}, W. and {Huber}, M.~E. and {Kirshner}, R.~P. and {Leibler}, C. and {McLeod}, B. and {Marion}, G.~H. and {Narayan}, G. and {Riess}, A.~G. and {Roth}, K.~C. and {Sanders}, N.~E. and {Scolnic}, D. and {Smith}, K. and {Stubbs}, C.~W. and {Tonry}, J.~L. and {Valenti}, S. and {Burgett}, W.~S. and {Chambers}, K.~C. and {Hodapp}, K.~W. and {Kaiser}, N. and {Kudritzki}, R. -P. and {Magnier}, E.~A. and {Price}, P.~A.},
        title = "{PS1-10afx at z = 1.388: Pan-STARRS1 Discovery of a New Type of Superluminous Supernova}",
      journal = {\apj},
     keywords = {supernovae: individual: PS1-10afx, surveys, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = apr,
       volume = {767},
       number = {2},
          eid = {162},
        pages = {162},
          doi = {10.1088/0004-637X/767/2/162},
archivePrefix = {arXiv},
       eprint = {1302.0009},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...767..162C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Collett2015,
       author = {{Collett}, Thomas E.},
        title = "{The Population of Galaxy-Galaxy Strong Lenses in Forthcoming Optical Imaging Surveys}",
      journal = {\apj},
     keywords = {gravitational lensing: strong, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2015,
        month = sep,
       volume = {811},
       number = {1},
          eid = {20},
        pages = {20},
          doi = {10.1088/0004-637X/811/1/20},
archivePrefix = {arXiv},
       eprint = {1507.02657},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...811...20C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Conroy2009a,
       author = {{Conroy}, Charlie and {Gunn}, James E. and {White}, Martin},
        title = "{The Propagation of Uncertainties in Stellar Population Synthesis Modeling. I. The Relevance of Uncertain Aspects of Stellar Evolution and the Initial Mass Function to the Derived Physical Properties of Galaxies}",
      journal = {\apj},
     keywords = {galaxies: evolution, galaxies: stellar content, stars: evolution, Astrophysics},
         year = 2009,
        month = jul,
       volume = {699},
       number = {1},
        pages = {486-506},
          doi = {10.1088/0004-637X/699/1/486},
archivePrefix = {arXiv},
       eprint = {0809.4261},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...699..486C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Craig2024,
       author = {{Craig}, Peter and {O'Connor}, Kyle and {Chakrabarti}, Sukanya and {Rodney}, Steven A. and {Pierel}, Justin R. and {McCully}, Curtis and {Perez-Fournon}, Ismael},
        title = "{A targeted search for strongly lensed supernovae with the Las Cumbres Observatory}",
      journal = {\mnras},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2024,
        month = oct,
       volume = {534},
       number = {2},
        pages = {1077-1092},
          doi = {10.1093/mnras/stae2103},
archivePrefix = {arXiv},
       eprint = {2111.01680},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024MNRAS.534.1077C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dalya2018,
       author = {{D{\'a}lya}, G. and {Galg{\'o}czi}, G. and {Dobos}, L. and {Frei}, Z. and {Heng}, I.~S. and {Macas}, R. and {Messenger}, C. and {Raffai}, P. and {de Souza}, R.~S.},
        title = "{GLADE: A galaxy catalogue for multimessenger searches in the advanced gravitational-wave detector era}",
      journal = {\mnras},
     keywords = {catalogues, galaxies: distances and redshifts, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = sep,
       volume = {479},
       number = {2},
        pages = {2374-2381},
          doi = {10.1093/mnras/sty1703},
archivePrefix = {arXiv},
       eprint = {1804.05709},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.479.2374D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Dekany2020,
       author = {{Dekany}, Richard and {Smith}, Roger M. and {Riddle}, Reed and {Feeney}, Michael and {Porter}, Michael and {Hale}, David and {Zolkower}, Jeffry and {Belicki}, Justin and {Kaye}, Stephen and {Henning}, John and {Walters}, Richard and {Cromer}, John and {Delacroix}, Alex and {Rodriguez}, Hector and {Reiley}, Daniel J. and {Mao}, Peter and {Hover}, David and {Murphy}, Patrick and {Burruss}, Rick and {Baker}, John and {Kowalski}, Marek and {Reif}, Klaus and {Mueller}, Phillip and {Bellm}, Eric and {Graham}, Matthew and {Kulkarni}, Shrinivas R.},
        title = "{The Zwicky Transient Facility: Observing System}",
      journal = {\pasp},
     keywords = {instrumentation: detectors, instrumentation: miscellaneous, methods: observational, surveys, techniques: photometric, time, Astrophysics - Instrumentation and Methods for Astrophysics, Physics - Instrumentation and Detectors, Physics - Optics},
         year = 2020,
        month = mar,
       volume = {132},
       number = {1009},
          eid = {038001},
        pages = {038001},
          doi = {10.1088/1538-3873/ab4ca2},
archivePrefix = {arXiv},
       eprint = {2008.04923},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020PASP..132c8001D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Denissenya2022,
       author = {{Denissenya}, Mikhail and {Bag}, Satadru and {Kim}, Alex G. and {Linder}, Eric V. and {Shafieloo}, Arman},
        title = "{Out of one, many: distinguishing time delays from lensed supernovae}",
      journal = {\mnras},
     keywords = {gravitational lensing: strong, transients: supernovae, cosmology: observations, methods: numerical, data analysis, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2022,
        month = mar,
       volume = {511},
       number = {1},
        pages = {1210-1217},
          doi = {10.1093/mnras/stac143},
archivePrefix = {arXiv},
       eprint = {2109.13282},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.511.1210D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DESILevi2013,
      author = {{Levi}, Michael and {Bebek}, Chris and {Beers}, Timothy and {Blum}, Robert and {Cahn}, Robert and {Eisenstein}, Daniel and {Flaugher}, Brenna and {Honscheid}, Klaus and {Kron}, Richard and {Lahav}, Ofer and {McDonald}, Patrick and {Roe}, Natalie and {Schlegel}, David and {representing the DESI collaboration}},
       title = "{The DESI Experiment, a whitepaper for Snowmass 2013}",
     journal = {arXiv e-prints},
    keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
        year = 2013,
       month = aug,
         eid = {arXiv:1308.0847},
       pages = {arXiv:1308.0847},
archivePrefix = {arXiv},
      eprint = {1308.0847},
primaryClass = {astro-ph.CO},
      adsurl = {https://ui.adsabs.harvard.edu/abs/2013arXiv1308.0847L},
     adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{DESI2016a,
       author = {{DESI Collaboration} and {Aghamousa}, Amir and {Aguilar}, Jessica and {Ahlen}, Steve and {Alam}, Shadab and {Allen}, Lori E. and {Allende Prieto}, Carlos and {Annis}, James and {Bailey}, Stephen and {Balland}, Christophe and {Ballester}, Otger and {Baltay}, Charles and {Beaufore}, Lucas and {Bebek}, Chris and {Beers}, Timothy C. and {Bell}, Eric F. and {Bernal}, Jos{\'e} Luis and {Besuner}, Robert and {Beutler}, Florian and {Blake}, Chris and {Bleuler}, Hannes and {Blomqvist}, Michael and {Blum}, Robert and {Bolton}, Adam S. and {Briceno}, Cesar and {Brooks}, David and {Brownstein}, Joel R. and {Buckley-Geer}, Elizabeth and {Burden}, Angela and {Burtin}, Etienne and {Busca}, Nicolas G. and {Cahn}, Robert N. and {Cai}, Yan-Chuan and {Cardiel-Sas}, Laia and {Carlberg}, Raymond G. and {Carton}, Pierre-Henri and {Casas}, Ricard and {Castander}, Francisco J. and {Cervantes-Cota}, Jorge L. and {Claybaugh}, Todd M. and {Close}, Madeline and {Coker}, Carl T. and {Cole}, Shaun and {Comparat}, Johan and {Cooper}, Andrew P. and {Cousinou}, M. -C. and {Crocce}, Martin and {Cuby}, Jean-Gabriel and {Cunningham}, Daniel P. and {Davis}, Tamara M. and {Dawson}, Kyle S. and {de la Macorra}, Axel and {De Vicente}, Juan and {Delubac}, Timoth{\'e}e and {Derwent}, Mark and {Dey}, Arjun and {Dhungana}, Govinda and {Ding}, Zhejie and {Doel}, Peter and {Duan}, Yutong T. and {Ealet}, Anne and {Edelstein}, Jerry and {Eftekharzadeh}, Sarah and {Eisenstein}, Daniel J. and {Elliott}, Ann and {Escoffier}, St{\'e}phanie and {Evatt}, Matthew and {Fagrelius}, Parker and {Fan}, Xiaohui and {Fanning}, Kevin and {Farahi}, Arya and {Farihi}, Jay and {Favole}, Ginevra and {Feng}, Yu and {Fernandez}, Enrique and {Findlay}, Joseph R. and {Finkbeiner}, Douglas P. and {Fitzpatrick}, Michael J. and {Flaugher}, Brenna and {Flender}, Samuel and {Font-Ribera}, Andreu and {Forero-Romero}, Jaime E. and {Fosalba}, Pablo and {Frenk}, Carlos S. and {Fumagalli}, Michele and {Gaensicke}, Boris T. and {Gallo}, Giuseppe and {Garcia-Bellido}, Juan and {Gaztanaga}, Enrique and {Pietro Gentile Fusillo}, Nicola and {Gerard}, Terry and {Gershkovich}, Irena and {Giannantonio}, Tommaso and {Gillet}, Denis and {Gonzalez-de-Rivera}, Guillermo and {Gonzalez-Perez}, Violeta and {Gott}, Shelby and {Graur}, Or and {Gutierrez}, Gaston and {Guy}, Julien and {Habib}, Salman and {Heetderks}, Henry and {Heetderks}, Ian and {Heitmann}, Katrin and {Hellwing}, Wojciech A. and {Herrera}, David A. and {Ho}, Shirley and {Holland}, Stephen and {Honscheid}, Klaus and {Huff}, Eric and {Hutchinson}, Timothy A. and {Huterer}, Dragan and {Hwang}, Ho Seong and {Illa Laguna}, Joseph Maria and {Ishikawa}, Yuzo and {Jacobs}, Dianna and {Jeffrey}, Niall and {Jelinsky}, Patrick and {Jennings}, Elise and {Jiang}, Linhua and {Jimenez}, Jorge and {Johnson}, Jennifer and {Joyce}, Richard and {Jullo}, Eric and {Juneau}, St{\'e}phanie and {Kama}, Sami and {Karcher}, Armin and {Karkar}, Sonia and {Kehoe}, Robert and {Kennamer}, Noble and {Kent}, Stephen and {Kilbinger}, Martin and {Kim}, Alex G. and {Kirkby}, David and {Kisner}, Theodore and {Kitanidis}, Ellie and {Kneib}, Jean-Paul and {Koposov}, Sergey and {Kovacs}, Eve and {Koyama}, Kazuya and {Kremin}, Anthony and {Kron}, Richard and {Kronig}, Luzius and {Kueter-Young}, Andrea and {Lacey}, Cedric G. and {Lafever}, Robin and {Lahav}, Ofer and {Lambert}, Andrew and {Lampton}, Michael and {Landriau}, Martin and {Lang}, Dustin and {Lauer}, Tod R. and {Le Goff}, Jean-Marc and {Le Guillou}, Laurent and {Le Van Suu}, Auguste and {Lee}, Jae Hyeon and {Lee}, Su-Jeong and {Leitner}, Daniela and {Lesser}, Michael and {Levi}, Michael E. and {L'Huillier}, Benjamin and {Li}, Baojiu and {Liang}, Ming and {Lin}, Huan and {Linder}, Eric and {Loebman}, Sarah R. and {Luki{\'c}}, Zarija and {Ma}, Jun and {MacCrann}, Niall and {Magneville}, Christophe and {Makarem}, Laleh and {Manera}, Marc and {Manser}, Christopher J. and {Marshall}, Robert and {Martini}, Paul and {Massey}, Richard and {Matheson}, Thomas and {McCauley}, Jeremy and {McDonald}, Patrick and {McGreer}, Ian D. and {Meisner}, Aaron and {Metcalfe}, Nigel and {Miller}, Timothy N. and {Miquel}, Ramon and {Moustakas}, John and {Myers}, Adam and {Naik}, Milind and {Newman}, Jeffrey A. and {Nichol}, Robert C. and {Nicola}, Andrina and {Nicolati da Costa}, Luiz and {Nie}, Jundan and {Niz}, Gustavo and {Norberg}, Peder and {Nord}, Brian and {Norman}, Dara and {Nugent}, Peter and {O'Brien}, Thomas and {Oh}, Minji and {Olsen}, Knut A.~G. and {Padilla}, Cristobal and {Padmanabhan}, Hamsa and {Padmanabhan}, Nikhil and {Palanque-Delabrouille}, Nathalie and {Palmese}, Antonella and {Pappalardo}, Daniel and {P{\^a}ris}, Isabelle and {Park}, Changbom and {Patej}, Anna and {Peacock}, John A. and {Peiris}, Hiranya V. and {Peng}, Xiyan and {Percival}, Will J. and {Perruchot}, Sandrine and {Pieri}, Matthew M. and {Pogge}, Richard and {Pollack}, Jennifer E. and {Poppett}, Claire and {Prada}, Francisco and {Prakash}, Abhishek and {Probst}, Ronald G. and {Rabinowitz}, David and {Raichoor}, Anand and {Ree}, Chang Hee and {Refregier}, Alexandre and {Regal}, Xavier and {Reid}, Beth and {Reil}, Kevin and {Rezaie}, Mehdi and {Rockosi}, Constance M. and {Roe}, Natalie and {Ronayette}, Samuel and {Roodman}, Aaron and {Ross}, Ashley J. and {Ross}, Nicholas P. and {Rossi}, Graziano and {Rozo}, Eduardo and {Ruhlmann-Kleider}, Vanina and {Rykoff}, Eli S. and {Sabiu}, Cristiano and {Samushia}, Lado and {Sanchez}, Eusebio and {Sanchez}, Javier and {Schlegel}, David J. and {Schneider}, Michael and {Schubnell}, Michael and {Secroun}, Aur{\'e}lia and {Seljak}, Uros and {Seo}, Hee-Jong and {Serrano}, Santiago and {Shafieloo}, Arman and {Shan}, Huanyuan and {Sharples}, Ray and {Sholl}, Michael J. and {Shourt}, William V. and {Silber}, Joseph H. and {Silva}, David R. and {Sirk}, Martin M. and {Slosar}, Anze and {Smith}, Alex and {Smoot}, George F. and {Som}, Debopam and {Song}, Yong-Seon and {Sprayberry}, David and {Staten}, Ryan and {Stefanik}, Andy and {Tarle}, Gregory and {Sien Tie}, Suk and {Tinker}, Jeremy L. and {Tojeiro}, Rita and {Valdes}, Francisco and {Valenzuela}, Octavio and {Valluri}, Monica and {Vargas-Magana}, Mariana and {Verde}, Licia and {Walker}, Alistair R. and {Wang}, Jiali and {Wang}, Yuting and {Weaver}, Benjamin A. and {Weaverdyck}, Curtis and {Wechsler}, Risa H. and {Weinberg}, David H. and {White}, Martin and {Yang}, Qian and {Yeche}, Christophe and {Zhang}, Tianmeng and {Zhao}, Gong-Bo and {Zheng}, Yi and {Zhou}, Xu and {Zhou}, Zhimin and {Zhu}, Yaling and {Zou}, Hu and {Zu}, Ying},
        title = "{The DESI Experiment Part I: Science,Targeting, and Survey Design}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2016,
        month = oct,
          eid = {arXiv:1611.00036},
        pages = {arXiv:1611.00036},
          doi = {10.48550/arXiv.1611.00036},
archivePrefix = {arXiv},
       eprint = {1611.00036},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016arXiv161100036D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DESI2016b,
       author = {{DESI Collaboration} and {Aghamousa}, Amir and {Aguilar}, Jessica and {Ahlen}, Steve and {Alam}, Shadab and {Allen}, Lori E. and {Allende Prieto}, Carlos and {Annis}, James and {Bailey}, Stephen and {Balland}, Christophe and {Ballester}, Otger and {Baltay}, Charles and {Beaufore}, Lucas and {Bebek}, Chris and {Beers}, Timothy C. and {Bell}, Eric F. and {Bernal}, Jos{\'e} Luis and {Besuner}, Robert and {Beutler}, Florian and {Blake}, Chris and {Bleuler}, Hannes and {Blomqvist}, Michael and {Blum}, Robert and {Bolton}, Adam S. and {Briceno}, Cesar and {Brooks}, David and {Brownstein}, Joel R. and {Buckley-Geer}, Elizabeth and {Burden}, Angela and {Burtin}, Etienne and {Busca}, Nicolas G. and {Cahn}, Robert N. and {Cai}, Yan-Chuan and {Cardiel-Sas}, Laia and {Carlberg}, Raymond G. and {Carton}, Pierre-Henri and {Casas}, Ricard and {Castander}, Francisco J. and {Cervantes-Cota}, Jorge L. and {Claybaugh}, Todd M. and {Close}, Madeline and {Coker}, Carl T. and {Cole}, Shaun and {Comparat}, Johan and {Cooper}, Andrew P. and {Cousinou}, M. -C. and {Crocce}, Martin and {Cuby}, Jean-Gabriel and {Cunningham}, Daniel P. and {Davis}, Tamara M. and {Dawson}, Kyle S. and {de la Macorra}, Axel and {De Vicente}, Juan and {Delubac}, Timoth{\'e}e and {Derwent}, Mark and {Dey}, Arjun and {Dhungana}, Govinda and {Ding}, Zhejie and {Doel}, Peter and {Duan}, Yutong T. and {Ealet}, Anne and {Edelstein}, Jerry and {Eftekharzadeh}, Sarah and {Eisenstein}, Daniel J. and {Elliott}, Ann and {Escoffier}, St{\'e}phanie and {Evatt}, Matthew and {Fagrelius}, Parker and {Fan}, Xiaohui and {Fanning}, Kevin and {Farahi}, Arya and {Farihi}, Jay and {Favole}, Ginevra and {Feng}, Yu and {Fernandez}, Enrique and {Findlay}, Joseph R. and {Finkbeiner}, Douglas P. and {Fitzpatrick}, Michael J. and {Flaugher}, Brenna and {Flender}, Samuel and {Font-Ribera}, Andreu and {Forero-Romero}, Jaime E. and {Fosalba}, Pablo and {Frenk}, Carlos S. and {Fumagalli}, Michele and {Gaensicke}, Boris T. and {Gallo}, Giuseppe and {Garcia-Bellido}, Juan and {Gaztanaga}, Enrique and {Pietro Gentile Fusillo}, Nicola and {Gerard}, Terry and {Gershkovich}, Irena and {Giannantonio}, Tommaso and {Gillet}, Denis and {Gonzalez-de-Rivera}, Guillermo and {Gonzalez-Perez}, Violeta and {Gott}, Shelby and {Graur}, Or and {Gutierrez}, Gaston and {Guy}, Julien and {Habib}, Salman and {Heetderks}, Henry and {Heetderks}, Ian and {Heitmann}, Katrin and {Hellwing}, Wojciech A. and {Herrera}, David A. and {Ho}, Shirley and {Holland}, Stephen and {Honscheid}, Klaus and {Huff}, Eric and {Hutchinson}, Timothy A. and {Huterer}, Dragan and {Hwang}, Ho Seong and {Illa Laguna}, Joseph Maria and {Ishikawa}, Yuzo and {Jacobs}, Dianna and {Jeffrey}, Niall and {Jelinsky}, Patrick and {Jennings}, Elise and {Jiang}, Linhua and {Jimenez}, Jorge and {Johnson}, Jennifer and {Joyce}, Richard and {Jullo}, Eric and {Juneau}, St{\'e}phanie and {Kama}, Sami and {Karcher}, Armin and {Karkar}, Sonia and {Kehoe}, Robert and {Kennamer}, Noble and {Kent}, Stephen and {Kilbinger}, Martin and {Kim}, Alex G. and {Kirkby}, David and {Kisner}, Theodore and {Kitanidis}, Ellie and {Kneib}, Jean-Paul and {Koposov}, Sergey and {Kovacs}, Eve and {Koyama}, Kazuya and {Kremin}, Anthony and {Kron}, Richard and {Kronig}, Luzius and {Kueter-Young}, Andrea and {Lacey}, Cedric G. and {Lafever}, Robin and {Lahav}, Ofer and {Lambert}, Andrew and {Lampton}, Michael and {Landriau}, Martin and {Lang}, Dustin and {Lauer}, Tod R. and {Le Goff}, Jean-Marc and {Le Guillou}, Laurent and {Le Van Suu}, Auguste and {Lee}, Jae Hyeon and {Lee}, Su-Jeong and {Leitner}, Daniela and {Lesser}, Michael and {Levi}, Michael E. and {L'Huillier}, Benjamin and {Li}, Baojiu and {Liang}, Ming and {Lin}, Huan and {Linder}, Eric and {Loebman}, Sarah R. and {Luki{\'c}}, Zarija and {Ma}, Jun and {MacCrann}, Niall and {Magneville}, Christophe and {Makarem}, Laleh and {Manera}, Marc and {Manser}, Christopher J. and {Marshall}, Robert and {Martini}, Paul and {Massey}, Richard and {Matheson}, Thomas and {McCauley}, Jeremy and {McDonald}, Patrick and {McGreer}, Ian D. and {Meisner}, Aaron and {Metcalfe}, Nigel and {Miller}, Timothy N. and {Miquel}, Ramon and {Moustakas}, John and {Myers}, Adam and {Naik}, Milind and {Newman}, Jeffrey A. and {Nichol}, Robert C. and {Nicola}, Andrina and {Nicolati da Costa}, Luiz and {Nie}, Jundan and {Niz}, Gustavo and {Norberg}, Peder and {Nord}, Brian and {Norman}, Dara and {Nugent}, Peter and {O'Brien}, Thomas and {Oh}, Minji and {Olsen}, Knut A.~G. and {Padilla}, Cristobal and {Padmanabhan}, Hamsa and {Padmanabhan}, Nikhil and {Palanque-Delabrouille}, Nathalie and {Palmese}, Antonella and {Pappalardo}, Daniel and {P{\^a}ris}, Isabelle and {Park}, Changbom and {Patej}, Anna and {Peacock}, John A. and {Peiris}, Hiranya V. and {Peng}, Xiyan and {Percival}, Will J. and {Perruchot}, Sandrine and {Pieri}, Matthew M. and {Pogge}, Richard and {Pollack}, Jennifer E. and {Poppett}, Claire and {Prada}, Francisco and {Prakash}, Abhishek and {Probst}, Ronald G. and {Rabinowitz}, David and {Raichoor}, Anand and {Ree}, Chang Hee and {Refregier}, Alexandre and {Regal}, Xavier and {Reid}, Beth and {Reil}, Kevin and {Rezaie}, Mehdi and {Rockosi}, Constance M. and {Roe}, Natalie and {Ronayette}, Samuel and {Roodman}, Aaron and {Ross}, Ashley J. and {Ross}, Nicholas P. and {Rossi}, Graziano and {Rozo}, Eduardo and {Ruhlmann-Kleider}, Vanina and {Rykoff}, Eli S. and {Sabiu}, Cristiano and {Samushia}, Lado and {Sanchez}, Eusebio and {Sanchez}, Javier and {Schlegel}, David J. and {Schneider}, Michael and {Schubnell}, Michael and {Secroun}, Aur{\'e}lia and {Seljak}, Uros and {Seo}, Hee-Jong and {Serrano}, Santiago and {Shafieloo}, Arman and {Shan}, Huanyuan and {Sharples}, Ray and {Sholl}, Michael J. and {Shourt}, William V. and {Silber}, Joseph H. and {Silva}, David R. and {Sirk}, Martin M. and {Slosar}, Anze and {Smith}, Alex and {Smoot}, George F. and {Som}, Debopam and {Song}, Yong-Seon and {Sprayberry}, David and {Staten}, Ryan and {Stefanik}, Andy and {Tarle}, Gregory and {Sien Tie}, Suk and {Tinker}, Jeremy L. and {Tojeiro}, Rita and {Valdes}, Francisco and {Valenzuela}, Octavio and {Valluri}, Monica and {Vargas-Magana}, Mariana and {Verde}, Licia and {Walker}, Alistair R. and {Wang}, Jiali and {Wang}, Yuting and {Weaver}, Benjamin A. and {Weaverdyck}, Curtis and {Wechsler}, Risa H. and {Weinberg}, David H. and {White}, Martin and {Yang}, Qian and {Yeche}, Christophe and {Zhang}, Tianmeng and {Zhao}, Gong-Bo and {Zheng}, Yi and {Zhou}, Xu and {Zhou}, Zhimin and {Zhu}, Yaling and {Zou}, Hu and {Zu}, Ying},
        title = "{The DESI Experiment Part II: Instrument Design}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2016,
        month = oct,
          eid = {arXiv:1611.00037},
        pages = {arXiv:1611.00037},
          doi = {10.48550/arXiv.1611.00037},
archivePrefix = {arXiv},
       eprint = {1611.00037},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016arXiv161100037D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DESI2022,
      author = {{DESI Collaboration} and {Abareshi}, B. and {Aguilar}, J. and {Ahlen}, S. and {Alam}, Shadab and {Alexander}, David M. and {Alfarsy}, R. and {Allen}, L. and {Allende Prieto}, C. and {Alves}, O. and {Ameel}, J. and {Armengaud}, E. and {Asorey}, J. and {Aviles}, Alejandro and {Bailey}, S. and {Balaguera-Antol{\'\i}nez}, A. and {Ballester}, O. and {Baltay}, C. and {Bault}, A. and {Beltran}, S.~F. and {Benavides}, B. and {BenZvi}, S. and {Berti}, A. and {Besuner}, R. and {Beutler}, Florian and {Bianchi}, D. and {Blake}, C. and {Blanc}, P. and {Blum}, R. and {Bolton}, A. and {Bose}, S. and {Bramall}, D. and {Brieden}, S. and {Brodzeller}, A. and {Brooks}, D. and {Brownewell}, C. and {Buckley-Geer}, E. and {Cahn}, R.~N. and {Cai}, Z. and {Canning}, R. and {Capasso}, R. and {Carnero Rosell}, A. and {Carton}, P. and {Casas}, R. and {Castander}, F.~J. and {Cervantes-Cota}, J.~L. and {Chabanier}, S. and {Chaussidon}, E. and {Chuang}, C. and {Circosta}, C. and {Cole}, S. and {Cooper}, A.~P. and {da Costa}, L. and {Cousinou}, M. -C. and {Cuceu}, A. and {Davis}, T.~M. and {Dawson}, K. and {de la Cruz-Noriega}, R. and {de la Macorra}, A. and {de Mattia}, A. and {Della Costa}, J. and {Demmer}, P. and {Derwent}, M. and {Dey}, A. and {Dey}, B. and {Dhungana}, G. and {Ding}, Z. and {Dobson}, C. and {Doel}, P. and {Donald-McCann}, J. and {Donaldson}, J. and {Douglass}, K. and {Duan}, Y. and {Dunlop}, P. and {Edelstein}, J. and {Eftekharzadeh}, S. and {Eisenstein}, D.~J. and {Enriquez-Vargas}, M. and {Escoffier}, S. and {Evatt}, M. and {Fagrelius}, P. and {Fan}, X. and {Fanning}, K. and {Fawcett}, V.~A. and {Ferraro}, S. and {Ereza}, J. and {Flaugher}, B. and {Font-Ribera}, A. and {Forero-Romero}, J.~E. and {Frenk}, C.~S. and {Fromenteau}, S. and {G{\"a}nsicke}, B.~T. and {Garcia-Quintero}, C. and {Garrison}, L. and {Gazta{\~n}aga}, E. and {Gerardi}, F. and {Gil-Mar{\'\i}n}, H. and {Gontcho a Gontcho}, S. and {Gonzalez-Morales}, Alma X. and {Gonzalez-de-Rivera}, G. and {Gonzalez-Perez}, V. and {Gordon}, C. and {Graur}, O. and {Green}, D. and {Grove}, C. and {Gruen}, D. and {Gutierrez}, G. and {Guy}, J. and {Hahn}, C. and {Harris}, S. and {Herrera}, D. and {Herrera-Alcantar}, Hiram K. and {Honscheid}, K. and {Howlett}, C. and {Huterer}, D. and {Ir{\v{s}}i{\v{c}}}, V. and {Ishak}, M. and {Jelinsky}, P. and {Jiang}, L. and {Jimenez}, J. and {Jing}, Y.~P. and {Joyce}, R. and {Jullo}, E. and {Juneau}, S. and {Kara{\c{c}}ayl{\i}}, N.~G. and {Karamanis}, M. and {Karcher}, A. and {Karim}, T. and {Kehoe}, R. and {Kent}, S. and {Kirkby}, D. and {Kisner}, T. and {Kitaura}, F. and {Koposov}, S.~E. and {Kov{\'a}cs}, A. and {Kremin}, A. and {Krolewski}, Alex and {L'Huillier}, B. and {Lahav}, O. and {Lambert}, A. and {Lamman}, C. and {Lan}, Ting-Wen and {Landriau}, M. and {Lane}, S. and {Lang}, D. and {Lange}, J.~U. and {Lasker}, J. and {Le Guillou}, L. and {Leauthaud}, A. and {Le Van Suu}, A. and {Levi}, Michael E. and {Li}, T.~S. and {Magneville}, C. and {Manera}, M. and {Manser}, Christopher J. and {Marshall}, B. and {Martini}, Paul and {McCollam}, W. and {McDonald}, P. and {Meisner}, Aaron M. and {Mena-Fern{\'a}ndez}, J. and {Meneses-Rizo}, J. and {Mezcua}, M. and {Miller}, T. and {Miquel}, R. and {Montero-Camacho}, P. and {Moon}, J. and {Moustakas}, J. and {Mueller}, E. and {Mu{\~n}oz-Guti{\'e}rrez}, Andrea and {Myers}, Adam D. and {Nadathur}, S. and {Najita}, J. and {Napolitano}, L. and {Neilsen}, E. and {Newman}, Jeffrey A. and {Nie}, J.~D. and {Ning}, Y. and {Niz}, G. and {Norberg}, P. and {Noriega}, Hern{\'a}n E. and {O'Brien}, T. and {Obuljen}, A. and {Palanque-Delabrouille}, N. and {Palmese}, A. and {Zhiwei}, P. and {Pappalardo}, D. and {PENG}, X. and {Percival}, W.~J. and {Perruchot}, S. and {Pogge}, R. and {Poppett}, C. and {Porredon}, A. and {Prada}, F. and {Prochaska}, J. and {Pucha}, R. and {P{\'e}rez-Fern{\'a}ndez}, A. and {P{\'e}rez-R{\`a}fols}, I. and {Rabinowitz}, D. and {Raichoor}, A. and {Ramirez-Solano}, S. and {Ram{\'\i}rez-P{\'e}rez}, C{\'e}sar and {Ravoux}, C. and {Reil}, K. and {Rezaie}, M. and {Rocher}, A. and {Rockosi}, C. and {Roe}, N.~A. and {Roodman}, A. and {Ross}, A.~J. and {Rossi}, G. and {Ruggeri}, R. and {Ruhlmann-Kleider}, V. and {Sabiu}, C.~G. and {Safonova}, S. and {Said}, K. and {Saintonge}, A. and {Salas Catonga}, Javier and {Samushia}, L. and {Sanchez}, E. and {Saulder}, C. and {Schaan}, E. and {Schlafly}, E. and {Schlegel}, D. and {Schmoll}, J. and {Scholte}, D. and {Schubnell}, M. and {Secroun}, A. and {Seo}, H. and {Serrano}, S. and {Sharples}, Ray M. and {Sholl}, Michael J. and {Silber}, Joseph Harry and {Silva}, D.~R. and {Sirk}, M. and {Siudek}, M. and {Smith}, A. and {Sprayberry}, D. and {Staten}, R. and {Stupak}, B. and {Tan}, T. and {Tarl{\'e}}, Gregory and {Tie}, Suk Sien and {Tojeiro}, R. and {Ure{\~n}a-L{\'o}pez}, L.~A. and {Valdes}, F. and {Valenzuela}, O. and {Valluri}, M. and {Vargas-Maga{\~n}a}, M. and {Verde}, L. and {Walther}, M. and {Wang}, B. and {Wang}, M.~S. and {Weaver}, B.~A. and {Weaverdyck}, C. and {Wechsler}, R. and {Wilson}, Michael J. and {Yang}, J. and {Yu}, Y. and {Yuan}, S. and {Y{\`e}che}, Christophe and {Zhang}, H. and {Zhang}, K. and {Zhao}, Cheng and {Zhou}, Rongpu and {Zhou}, Zhimin and {Zou}, H. and {Zou}, J. and {Zou}, S. and {Zu}, Y. and {DESI Collaboration}},
       title = "{Overview of the Instrumentation for the Dark Energy Spectroscopic Instrument}",
     journal = {\aj},
    keywords = {Dark energy, Spectroscopy, Astronomical instrumentation, Spectrometers, Optical telescopes, 351, 1558, 799, 1554, 1174, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics},
        year = 2022,
       month = nov,
      volume = {164},
      number = {5},
         eid = {207},
       pages = {207},
         doi = {10.3847/1538-3881/ac882b},
archivePrefix = {arXiv},
      eprint = {2205.10939},
primaryClass = {astro-ph.IM},
      adsurl = {https://ui.adsabs.harvard.edu/abs/2022AJ....164..207A},
     adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DESISilber2023,
      author = {{Silber}, Joseph Harry and {Fagrelius}, Parker and {Fanning}, Kevin and {Schubnell}, Michael and {Aguilar}, Jessica Nicole and {Ahlen}, Steven and {Ameel}, Jon and {Ballester}, Otger and {Baltay}, Charles and {Bebek}, Chris and {Benton Beard}, Dominic and {Besuner}, Robert and {Cardiel-Sas}, Laia and {Casas}, Ricard and {Castander}, Francisco Javier and {Claybaugh}, Todd and {Dobson}, Carl and {Duan}, Yutong and {Dunlop}, Patrick and {Edelstein}, Jerry and {Emmet}, William T. and {Elliott}, Ann and {Evatt}, Matthew and {Gershkovich}, Irena and {Guy}, Julien and {Harris}, Stu and {Heetderks}, Henry and {Heetderks}, Ian and {Honscheid}, Klaus and {Illa}, Jose Maria and {Jelinsky}, Patrick and {Jelinsky}, Sharon R. and {Jimenez}, Jorge and {Karcher}, Armin and {Kent}, Stephen and {Kirkby}, David and {Kneib}, Jean-Paul and {Lambert}, Andrew and {Lampton}, Mike and {Leitner}, Daniela and {Levi}, Michael and {McCauley}, Jeremy and {Meisner}, Aaron and {Miller}, Timothy N. and {Miquel}, Ramon and {Mundet}, Juli{\'a} and {Poppett}, Claire and {Rabinowitz}, David and {Reil}, Kevin and {Roman}, David and {Schlegel}, David and {Serrano}, Santiago and {Van Shourt}, William and {Sprayberry}, David and {Tarl{\'e}}, Gregory and {Tie}, Suk Sien and {Weaverdyck}, Curtis and {Zhang}, Kai and {Azzaro}, Marco and {Bailey}, Stephen and {Becerril}, Santiago and {Blackwell}, Tami and {Bouri}, Mohamed and {Brooks}, David and {Buckley-Geer}, Elizabeth and {Castro}, Jose Pe{\~n}ate and {Derwent}, Mark and {Dey}, Arjun and {Dhungana}, Govinda and {Doel}, Peter and {Eisenstein}, Daniel J. and {Fahim}, Nasib and {Garcia-Bellido}, Juan and {Gazta{\~n}aga}, Enrique and {A Gontcho}, Satya Gontcho and {Gutierrez}, Gaston and {H{\"o}rler}, Philipp and {Kehoe}, Robert and {Kisner}, Theodore and {Kremin}, Anthony and {Kronig}, Luzius and {Landriau}, Martin and {Le Guillou}, Laurent and {Martini}, Paul and {Moustakas}, John and {Palanque-Delabrouille}, Nathalie and {Peng}, Xiyan and {Percival}, Will and {Prada}, Francisco and {Allende Prieto}, Carlos and {de Rivera}, Guillermo Gonzalez and {Sanchez}, Eusebio and {Sanchez}, Justo and {Sharples}, Ray and {Soares-Santos}, Marcelle and {Schlafly}, Edward and {Weaver}, Benjamin Alan and {Zhou}, Zhimin and {Zhu}, Yaling and {Zou}, Hu and {DESI Collaboration}},
       title = "{The Robotic Multiobject Focal Plane System of the Dark Energy Spectroscopic Instrument (DESI)}",
     journal = {\aj},
    keywords = {Dark energy, Astronomical instrumentation, Spectrometers, Galaxy spectroscopy, 351, 799, 1554, 2171, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics},
        year = 2023,
       month = jan,
      volume = {165},
      number = {1},
         eid = {9},
       pages = {9},
         doi = {10.3847/1538-3881/ac9ab1},
archivePrefix = {arXiv},
      eprint = {2205.09014},
primaryClass = {astro-ph.IM},
      adsurl = {https://ui.adsabs.harvard.edu/abs/2023AJ....165....9S},
     adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DESIMiller2023,
       author = {{Miller}, Timothy N. and {Doel}, Peter and {Gutierrez}, Gaston and {Besuner}, Robert and {Brooks}, David and {Gallo}, Giuseppe and {Heetderks}, Henry and {Jelinsky}, Patrick and {Kent}, Stephen M. and {Lampton}, Michael and {Levi}, Michael E. and {Liang}, Ming and {Meisner}, Aaron and {Sholl}, Michael J. and {Silber}, Joseph Harry and {Sprayberry}, David and {Aguilar}, Jessica Nicole and {de la Macorra}, Axel and {Eisenstein}, Daniel and {Fanning}, Kevin and {Font-Ribera}, Andreu and {Gazta{\~n}aga}, Enrique and {Gontcho A Gontcho}, Satya and {Honscheid}, Klaus and {Jimenez}, Jorge and {Joyce}, Dick and {Kehoe}, Robert and {Kisner}, Theodore and {Kremin}, Anthony and {Landriau}, Martin and {Le Guillou}, Laurent and {Magneville}, Christophe and {Martini}, Paul and {Miquel}, Ramon and {Moustakas}, John and {Nie}, Jundan and {Percival}, Will and {Poppett}, Claire and {Prada}, Francisco and {Rossi}, Graziano and {Schlegel}, David and {Schubnell}, Michael and {Seo}, Hee-Jong and {Sharples}, Ray and {Tarl{\'e}}, Gregory and {Vargas-Maga{\~n}a}, Mariana and {Zhou}, Zhimin and {the DESI Collaboration}},
        title = "{The Optical Corrector for the Dark Energy Spectroscopic Instrument}",
      journal = {\aj},
     keywords = {Dark energy, Astronomical instrumentation, Optical telescopes, Wide-field telescopes, Lenses, Prime focus, Primary mirror, 351, 799, 1174, 1800, 2347, 2354, 2345, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2024,
        month = aug,
       volume = {168},
       number = {2},
          eid = {95},
        pages = {95},
          doi = {10.3847/1538-3881/ad45fe},
archivePrefix = {arXiv},
       eprint = {2306.06310},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024AJ....168...95M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DESIGuy2023,
      author = {{Guy}, J. and {Bailey}, S. and {Kremin}, A. and {Alam}, Shadab and {Alexander}, D.~M. and {Allende Prieto}, C. and {BenZvi}, S. and {Bolton}, A.~S. and {Brooks}, D. and {Chaussidon}, E. and {Cooper}, A.~P. and {Dawson}, K. and {de la Macorra}, A. and {Dey}, A. and {Dey}, Biprateep and {Dhungana}, G. and {Eisenstein}, D.~J. and {Font-Ribera}, A. and {Forero-Romero}, J.~E. and {Gazta{\~n}aga}, E. and {Gontcho A Gontcho}, S. and {Green}, D. and {Honscheid}, K. and {Ishak}, M. and {Kehoe}, R. and {Kirkby}, D. and {Kisner}, T. and {Koposov}, Sergey E. and {Lan}, Ting-Wen and {Landriau}, M. and {Le Guillou}, L. and {Levi}, Michael E. and {Magneville}, C. and {Manser}, Christopher J. and {Martini}, P. and {Meisner}, Aaron M. and {Miquel}, R. and {Moustakas}, J. and {Myers}, Adam D. and {Newman}, Jeffrey A. and {Nie}, Jundan and {Palanque-Delabrouille}, N. and {Percival}, W.~J. and {Poppett}, C. and {Prada}, F. and {Raichoor}, A. and {Ravoux}, C. and {Ross}, A.~J. and {Schlafly}, E.~F. and {Schlegel}, D. and {Schubnell}, M. and {Sharples}, Ray M. and {Tarl{\'e}}, Gregory and {Weaver}, B.~A. and {Y{\'e}che}, Christophe and {Zhou}, Rongpu and {Zhou}, Zhimin and {Zou}, H.},
       title = "{The Spectroscopic Data Processing Pipeline for the Dark Energy Spectroscopic Instrument}",
     journal = {\aj},
    keywords = {Galaxy spectroscopy, High-redshift galaxies, Redshift surveys, 2171, 734, 1378, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics},
        year = 2023,
       month = apr,
      volume = {165},
      number = {4},
         eid = {144},
       pages = {144},
         doi = {10.3847/1538-3881/acb212},
archivePrefix = {arXiv},
      eprint = {2209.14482},
primaryClass = {astro-ph.IM},
      adsurl = {https://ui.adsabs.harvard.edu/abs/2023AJ....165..144G},
     adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DESIHahn2023,
      author = {{Hahn}, ChangHoon and {Wilson}, Michael J. and {Ruiz-Macias}, Omar and {Cole}, Shaun and {Weinberg}, David H. and {Moustakas}, John and {Kremin}, Anthony and {Tinker}, Jeremy L. and {Smith}, Alex and {Wechsler}, Risa H. and {Ahlen}, Steven and {Alam}, Shadab and {Bailey}, Stephen and {Brooks}, David and {Cooper}, Andrew P. and {Davis}, Tamara M. and {Dawson}, Kyle and {Dey}, Arjun and {Dey}, Biprateep and {Eftekharzadeh}, Sarah and {Eisenstein}, Daniel J. and {Fanning}, Kevin and {Forero-Romero}, Jaime E. and {Frenk}, Carlos S. and {Gazta{\~n}aga}, Enrique and {Gontcho A Gontcho}, Satya and {Guy}, Julien and {Honscheid}, Klaus and {Ishak}, Mustapha and {Juneau}, St{\'e}phanie and {Kehoe}, Robert and {Kisner}, Theodore and {Lan}, Ting-Wen and {Landriau}, Martin and {Le Guillou}, Laurent and {Levi}, Michael E. and {Magneville}, Christophe and {Martini}, Paul and {Meisner}, Aaron and {Myers}, Adam D. and {Nie}, Jundan and {Norberg}, Peder and {Palanque-Delabrouille}, Nathalie and {Percival}, Will J. and {Poppett}, Claire and {Prada}, Francisco and {Raichoor}, Anand and {Ross}, Ashley J. and {Safonova}, Sasha and {Saulder}, Christoph and {Schlafly}, Eddie and {Schlegel}, David and {Sierra-Porta}, David and {Tarle}, Gregory and {Weaver}, Benjamin A. and {Y{\`e}che}, Christophe and {Zarrouk}, Pauline and {Zhou}, Rongpu and {Zhou}, Zhimin and {Zou}, Hu},
       title = "{The DESI Bright Galaxy Survey: Final Target Selection, Design, and Validation}",
     journal = {\aj},
    keywords = {Observational cosmology, Cosmology, Redshift surveys, Galaxies, Galactic and extragalactic astronomy, Galaxy spectroscopy, Spectrophotometry, 1146, 343, 1378, 573, 563, 2171, 1556, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
        year = 2023,
       month = jun,
      volume = {165},
      number = {6},
         eid = {253},
       pages = {253},
         doi = {10.3847/1538-3881/accff8},
archivePrefix = {arXiv},
      eprint = {2208.08512},
primaryClass = {astro-ph.CO},
      adsurl = {https://ui.adsabs.harvard.edu/abs/2023AJ....165..253H},
     adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DESI2023,
       author = {{DESI Collaboration} and {Adame}, A.~G. and {Aguilar}, J. and {Ahlen}, S. and {Alam}, S. and {Aldering}, G. and {Alexander}, D.~M. and {Alfarsy}, R. and {Allende Prieto}, C. and {Alvarez}, M. and et al.},
        title = "{The Early Data Release of the Dark Energy Spectroscopic Instrument}",
      journal = {\aj},
     keywords = {Astronomy data reduction, Observational cosmology, Astronomy databases, Astronomy data analysis, Astronomy software, Surveys, Redshift surveys, 1861, 1146, 83, 1858, 1855, 1671, 1378, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2024,
        month = aug,
       volume = {168},
       number = {2},
          eid = {58},
        pages = {58},
          doi = {10.3847/1538-3881/ad3217},
archivePrefix = {arXiv},
       eprint = {2306.06308},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024AJ....168...58D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DESI2024,
      author = {{DESI Collaboration} and {Adame}, A.~G. and {Aguilar}, J. and {Ahlen}, S. and {Alam}, S. and {Aldering}, G. and {Alexander}, D.~M. and {Alfarsy}, R. and {Allende Prieto}, C. and {Alvarez}, M. and {Alves}, O. and {Anand}, A. and {Andrade-Oliveira}, F. and {Armengaud}, E. and {Asorey}, J. and {Avila}, S. and {Aviles}, A. and {Bailey}, S. and {Balaguera-Antol{\'\i}nez}, A. and {Ballester}, O. and {Baltay}, C. and {Bault}, A. and {Bautista}, J. and {Behera}, J. and {Beltran}, S.~F. and {BenZvi}, S. and {Beraldo e Silva}, L. and {Bermejo-Climent}, J.~R. and {Berti}, A. and {Besuner}, R. and {Beutler}, F. and {Bianchi}, D. and {Blake}, C. and {Blum}, R. and {Bolton}, A.~S. and {Brieden}, S. and {Brodzeller}, A. and {Brooks}, D. and {Brown}, Z. and {Buckley-Geer}, E. and {Burtin}, E. and {Cabayol-Garcia}, L. and {Cai}, Z. and {Canning}, R. and {Cardiel-Sas}, L. and {Carnero Rosell}, A. and {Castander}, F.~J. and {Cervantes-Cota}, J.~L. and {Chabanier}, S. and {Chaussidon}, E. and {Chaves-Montero}, J. and {Chen}, S. and {Chen}, X. and {Chuang}, C. and {Claybaugh}, T. and {Cole}, S. and {Cooper}, A.~P. and {Cuceu}, A. and {Davis}, T.~M. and {Dawson}, K. and {de Belsunce}, R. and {de la Cruz}, R. and {de la Macorra}, A. and {de Mattia}, A. and {Demina}, R. and {Demirbozan}, U. and {DeRose}, J. and {Dey}, A. and {Dey}, B. and {Dhungana}, G. and {Ding}, J. and {Ding}, Z. and {Doel}, P. and {Doshi}, R. and {Douglass}, K. and {Edge}, A. and {Eftekharzadeh}, S. and {Eisenstein}, D.~J. and {Elliott}, A. and {Escoffier}, S. and {Fagrelius}, P. and {Fan}, X. and {Fanning}, K. and {Fawcett}, V.~A. and {Ferraro}, S. and {Ereza}, J. and {Flaugher}, B. and {Font-Ribera}, A. and {Forero-S{\'a}nchez}, D. and {Forero-Romero}, J.~E. and {Frenk}, C.~S. and {G{\"a}nsicke}, B.~T. and {Garc{\'\i}a}, L. {\'A}. and {Garc{\'\i}a-Bellido}, J. and {Garcia-Quintero}, C. and {Garrison}, L.~H. and {Gil-Mar{\'\i}n}, H. and {Golden-Marx}, J. and {Gontcho A Gontcho}, S. and {Gonzalez-Morales}, A.~X. and {Gonzalez-Perez}, V. and {Gordon}, C. and {Graur}, O. and {Green}, D. and {Gruen}, D. and {Guy}, J. and {Hadzhiyska}, B. and {Hahn}, C. and {Han}, J.~J. and {Hanif}, M.~M.~S. and {Herrera-Alcantar}, H.~K. and {Honscheid}, K. and {Hou}, J. and {Howlett}, C. and {Huterer}, D. and {Ir{\v{s}}i{\v{c}}}, V. and {Ishak}, M. and {Jana}, A. and {Jiang}, L. and {Jimenez}, J. and {Jing}, Y.~P. and {Joudaki}, S. and {Jullo}, E. and {Joyce}, R. and {Juneau}, S. and {Kizhuprakkat}, N. and {Kara{\c{c}}ayl{\i}}, N.~G. and {Karim}, T. and {Kehoe}, R. and {Kent}, S. and {Khederlarian}, A. and {Kim}, S. and {Kirkby}, D. and {Kisner}, T. and {Kitaura}, F. and {Kneib}, J. and {Koposov}, S.~E. and {Kov{\'a}cs}, A. and {Kremin}, A. and {Krolewski}, A. and {L'Huillier}, B. and {Lahav}, O. and {Lambert}, A. and {Lamman}, C. and {Lan}, T. -W. and {Landriau}, M. and {Lang}, D. and {Lange}, J.~U. and {Lasker}, J. and {Le Guillou}, L. and {Leauthaud}, A. and {Levi}, M.~E. and {Li}, T.~S. and {Linder}, E. and {Lyons}, A. and {Magneville}, C. and {Manera}, M. and {Manser}, C.~J. and {Margala}, D. and {Martini}, P. and {McDonald}, P. and {Medina}, G.~E. and {Medina-Varela}, L. and {Meisner}, A. and {Mena-Fern{\'a}ndez}, J. and {Meneses-Rizo}, J. and {Mezcua}, M. and {Miquel}, R. and {Montero-Camacho}, P. and {Moon}, J. and {Moore}, S. and {Moustakas}, J. and {Mueller}, E. and {Mundet}, J. and {Mu{\~n}oz-Guti{\'e}rrez}, A. and {Myers}, A.~D. and {Nadathur}, S. and {Napolitano}, L. and {Neveux}, R. and {Newman}, J.~A. and {Nie}, J. and {Niz}, G. and {Norberg}, P. and {Noriega}, H.~E. and {Paillas}, E. and {Palanque-Delabrouille}, N. and {Palmese}, A. and {Zhiwei}, P. and {Parkinson}, D. and {Penmetsa}, S. and {Percival}, W.~J. and {P{\'e}rez-Fern{\'a}ndez}, A. and {P{\'e}rez-R{\`a}fols}, I. and {Pieri}, M. and {Poppett}, C. and {Porredon}, A. and {Prada}, F. and {Pucha}, R. and {Raichoor}, A. and {Ram{\'\i}rez-P{\'e}rez}, C. and {Ramirez-Solano}, S. and {Rashkovetskyi}, M. and {Ravoux}, C. and {Rocher}, A. and {Rockosi}, C. and {Ross}, A.~J. and {Rossi}, G. and {Ruggeri}, R. and {Ruhlmann-Kleider}, V. and {Sabiu}, C.~G. and {Said}, K. and {Saintonge}, A. and {Samushia}, L. and {Sanchez}, E. and {Saulder}, C. and {Schaan}, E. and {Schlafly}, E.~F. and {Schlegel}, D. and {Scholte}, D. and {Schubnell}, M. and {Seo}, H. and {Shafieloo}, A. and {Sharples}, R. and {Sheu}, W. and {Silber}, J. and {Sinigaglia}, F. and {Siudek}, M. and {Slepian}, Z. and {Smith}, A. and {Sprayberry}, D. and {Stephey}, L. and {Su{\'a}rez-P{\'e}rez}, J. and {Sun}, Z. and {Tan}, T. and {Tarl{\'e}}, G. and {Tojeiro}, R. and {Ure{\~n}a-L{\'o}pez}, L.~A. and {Vaisakh}, R. and {Valcin}, D. and {Valdes}, F. and {Valluri}, M. and {Vargas-Maga{\~n}a}, M. and {Variu}, A. and {Verde}, L. and {Walther}, M. and {Wang}, B. and {Wang}, M.~S. and {Weaver}, B.~A. and {Weaverdyck}, N. and {Wechsler}, R.~H. and {White}, M. and {Xie}, Y. and {Yang}, J. and {Y{\`e}che}, C. and {Yu}, J. and {Yuan}, S. and {Zhang}, H. and {Zhang}, Z. and {Zhao}, C. and {Zheng}, Z. and {Zhou}, R. and {Zhou}, Z. and {Zou}, H. and {Zou}, S. and {Zu}, Y. and {DESI Collaboration}},
       title = "{Validation of the Scientific Program for the Dark Energy Spectroscopic Instrument}",
     journal = {\aj},
    keywords = {Cosmology, Redshift surveys, 343, 1378, Astrophysics - Cosmology and Nongalactic Astrophysics},
        year = 2024,
       month = feb,
      volume = {167},
      number = {2},
         eid = {62},
       pages = {62},
         doi = {10.3847/1538-3881/ad0b08},
archivePrefix = {arXiv},
      eprint = {2306.06307},
primaryClass = {astro-ph.CO},
      adsurl = {https://ui.adsabs.harvard.edu/abs/2024AJ....167...62A},
     adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DESI2024III,
       author = {{DESI Collaboration} and {Adame}, A.~G. and {Aguilar}, J. and {Ahlen}, S. and {Alam}, S. and {Alexander}, D.~M. and {Alvarez}, M. and {Alves}, O. and {Anand}, A. and {Andrade}, U. and {Armengaud}, E. and {Avila}, S. and {Aviles}, A. and {Awan}, H. and {Bailey}, S. and {Baltay}, C. and {Bault}, A. and {Behera}, J. and {BenZvi}, S. and {Beutler}, F. and {Bianchi}, D. and {Blake}, C. and {Blum}, R. and {Brieden}, S. and {Brodzeller}, A. and {Brooks}, D. and {Buckley-Geer}, E. and {Burtin}, E. and {Calderon}, R. and {Canning}, R. and {Carnero Rosell}, A. and {Cereskaite}, R. and {Cervantes-Cota}, J.~L. and {Chabanier}, S. and {Chaussidon}, E. and {Chaves-Montero}, J. and {Chen}, S. and {Chen}, X. and {Claybaugh}, T. and {Cole}, S. and {Cuceu}, A. and {Davis}, T.~M. and {Dawson}, K. and {de la Macorra}, A. and {de Mattia}, A. and {Deiosso}, N. and {Dey}, A. and {Dey}, B. and {Ding}, Z. and {Doel}, P. and {Edelstein}, J. and {Eftekharzadeh}, S. and {Eisenstein}, D.~J. and {Elliott}, A. and {Fagrelius}, P. and {Fanning}, K. and {Ferraro}, S. and {Ereza}, J. and {Findlay}, N. and {Flaugher}, B. and {Font-Ribera}, A. and {Forero-S{\'a}nchez}, D. and {Forero-Romero}, J.~E. and {Garcia-Quintero}, C. and {Gazta{\~n}aga}, E. and {Gil-Mar{\'\i}n}, H. and {Gontcho}, S. Gontcho A and {Gonzalez-Morales}, A.~X. and {Gonzalez-Perez}, V. and {Gordon}, C. and {Green}, D. and {Gruen}, D. and {Gsponer}, R. and {Gutierrez}, G. and {Guy}, J. and {Hadzhiyska}, B. and {Hahn}, C. and {Hanif}, M.~M. S and {Herrera-Alcantar}, H.~K. and {Honscheid}, K. and {Howlett}, C. and {Huterer}, D. and {Ir{\v{s}}i{\v{c}}}, V. and {Ishak}, M. and {Juneau}, S. and {Kara{\c{c}}ayl{\i}}, N.~G. and {Kehoe}, R. and {Kent}, S. and {Kirkby}, D. and {Kremin}, A. and {Krolewski}, A. and {Lai}, Y. and {Lan}, T. -W. and {Landriau}, M. and {Lang}, D. and {Lasker}, J. and {Le Goff}, J.~M. and {Le Guillou}, L. and {Leauthaud}, A. and {Levi}, M.~E. and {Li}, T.~S. and {Linder}, E. and {Lodha}, K. and {Magneville}, C. and {Manera}, M. and {Margala}, D. and {Martini}, P. and {Maus}, M. and {McDonald}, P. and {Medina-Varela}, L. and {Meisner}, A. and {Mena-Fern{\'a}ndez}, J. and {Miquel}, R. and {Moon}, J. and {Moore}, S. and {Moustakas}, J. and {Mudur}, N. and {Mueller}, E. and {Mu{\~n}oz-Guti{\'e}rrez}, A. and {Myers}, A.~D. and {Nadathur}, S. and {Napolitano}, L. and {Neveux}, R. and {Newman}, J.~A. and {Nguyen}, N.~M. and {Nie}, J. and {Niz}, G. and {Noriega}, H.~E. and {Padmanabhan}, N. and {Paillas}, E. and {Palanque-Delabrouille}, N. and {Pan}, J. and {Penmetsa}, S. and {Percival}, W.~J. and {Pieri}, M. and {Pinon}, M. and {Poppett}, C. and {Porredon}, A. and {Prada}, F. and {P{\'e}rez-Fern{\'a}ndez}, A. and {P{\'e}rez-R{\`a}fols}, I. and {Rabinowitz}, D. and {Raichoor}, A. and {Ram{\'\i}rez-P{\'e}rez}, C. and {Ramirez-Solano}, S. and {Rashkovetskyi}, M. and {Rezaie}, M. and {Rich}, J. and {Rocher}, A. and {Rockosi}, C. and {Roe}, N.~A. and {Rosado-Marin}, A. and {Ross}, A.~J. and {Rossi}, G. and {Ruggeri}, R. and {Ruhlmann-Kleider}, V. and {Samushia}, L. and {Sanchez}, E. and {Saulder}, C. and {Schlafly}, E.~F. and {Schlegel}, D. and {Schubnell}, M. and {Seo}, H. and {Sharples}, R. and {Silber}, J. and {Slosar}, A. and {Smith}, A. and {Sprayberry}, D. and {Swanson}, J. and {Tan}, T. and {Tarl{\'e}}, G. and {Trusov}, S. and {Vaisakh}, R. and {Valcin}, D. and {Valdes}, F. and {Vargas-Maga{\~n}a}, M. and {Verde}, L. and {Walther}, M. and {Wang}, B. and {Wang}, M.~S. and {Weaver}, B.~A. and {Weaverdyck}, N. and {Wechsler}, R.~H. and {Weinberg}, D.~H. and {White}, M. and {Yu}, J. and {Yu}, Y. and {Yuan}, S. and {Y{\`e}che}, C. and {Zaborowski}, E.~A. and {Zarrouk}, P. and {Zhang}, H. and {Zhao}, C. and {Zhao}, R. and {Zhou}, R. and {Zou}, H.},
        title = "{DESI 2024 III: Baryon Acoustic Oscillations from Galaxies and Quasars}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2024,
        month = apr,
          eid = {arXiv:2404.03000},
        pages = {arXiv:2404.03000},
          doi = {10.48550/arXiv.2404.03000},
archivePrefix = {arXiv},
       eprint = {2404.03000},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024arXiv240403000D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DESI2024IV,
       author = {{DESI Collaboration} and {Adame}, A.~G. and {Aguilar}, J. and {Ahlen}, S. and {Alam}, S. and {Alexander}, D.~M. and {Alvarez}, M. and {Alves}, O. and {Anand}, A. and {Andrade}, U. and {Armengaud}, E. and {Avila}, S. and {Aviles}, A. and {Awan}, H. and {Bailey}, S. and {Baltay}, C. and {Bault}, A. and {Bautista}, J. and {Behera}, J. and {BenZvi}, S. and {Beutler}, F. and {Bianchi}, D. and {Blake}, C. and {Blum}, R. and {Brieden}, S. and {Brodzeller}, A. and {Brooks}, D. and {Buckley-Geer}, E. and {Burtin}, E. and {Calderon}, R. and {Canning}, R. and {Carnero Rosell}, A. and {Cereskaite}, R. and {Cervantes-Cota}, J.~L. and {Chabanier}, S. and {Chaussidon}, E. and {Chaves-Montero}, J. and {Chen}, S. and {Chen}, X. and {Claybaugh}, T. and {Cole}, S. and {Cuceu}, A. and {Davis}, T.~M. and {Dawson}, K. and {de la Cruz}, R. and {de la Macorra}, A. and {de Mattia}, A. and {Deiosso}, N. and {Dey}, A. and {Dey}, B. and {Ding}, J. and {Ding}, Z. and {Doel}, P. and {Edelstein}, J. and {Eftekharzadeh}, S. and {Eisenstein}, D.~J. and {Elliott}, A. and {Fagrelius}, P. and {Fanning}, K. and {Ferraro}, S. and {Ereza}, J. and {Findlay}, N. and {Flaugher}, B. and {Font-Ribera}, A. and {Forero-S{\'a}nchez}, D. and {Forero-Romero}, J.~E. and {Garcia-Quintero}, C. and {Gazta{\~n}aga}, E. and {Gil-Mar{\'\i}n}, H. and {Gontcho}, S. Gontcho A and {Gonzalez-Morales}, A.~X. and {Gonzalez-Perez}, V. and {Gordon}, C. and {Green}, D. and {Gruen}, D. and {Gsponer}, R. and {Gutierrez}, G. and {Guy}, J. and {Hadzhiyska}, B. and {Hahn}, C. and {Hanif}, M.~M. S and {Herrera-Alcantar}, H.~K. and {Honscheid}, K. and {Howlett}, C. and {Huterer}, D. and {Ir{\v{s}}i{\v{c}}}, V. and {Ishak}, M. and {Juneau}, S. and {Kara{\c{c}}ayli}, N.~G. and {Kehoe}, R. and {Kent}, S. and {Kirkby}, D. and {Kremin}, A. and {Krolewski}, A. and {Lai}, Y. and {Lan}, T. -W. and {Landriau}, M. and {Lang}, D. and {Lasker}, J. and {Le Goff}, J.~M. and {Le Guillou}, L. and {Leauthaud}, A. and {Levi}, M.~E. and {Li}, T.~S. and {Linder}, E. and {Lodha}, K. and {Magneville}, C. and {Manera}, M. and {Margala}, D. and {Martini}, P. and {Maus}, M. and {McDonald}, P. and {Medina-Varela}, L. and {Meisner}, A. and {Mena-Fern{\'a}ndez}, J. and {Miquel}, R. and {Moon}, J. and {Moore}, S. and {Moustakas}, J. and {Mueller}, E. and {Mu{\~n}oz-Guti{\'e}rrez}, A. and {Myers}, A.~D. and {Nadathur}, S. and {Napolitano}, L. and {Neveux}, R. and {Newman}, J.~A. and {Nguyen}, N.~M. and {Nie}, J. and {Niz}, G. and {Noriega}, H.~E. and {Padmanabhan}, N. and {Paillas}, E. and {Palanque-Delabrouille}, N. and {Pan}, J. and {Penmetsa}, S. and {Percival}, W.~J. and {Pieri}, M.~M. and {Pinon}, M. and {Poppett}, C. and {Porredon}, A. and {Prada}, F. and {P{\'e}rez-Fern{\'a}ndez}, A. and {P{\'e}rez-R{\`a}fols}, I. and {Rabinowitz}, D. and {Raichoor}, A. and {Ram{\'\i}rez-P{\'e}rez}, C. and {Ramirez-Solano}, S. and {Rashkovetskyi}, M. and {Ravoux}, C. and {Rezaie}, M. and {Rich}, J. and {Rocher}, A. and {Rockosi}, C. and {Roe}, N.~A. and {Rosado-Marin}, A. and {Ross}, A.~J. and {Rossi}, G. and {Ruggeri}, R. and {Ruhlmann-Kleider}, V. and {Samushia}, L. and {Sanchez}, E. and {Saulder}, C. and {Schlafly}, E.~F. and {Schlegel}, D. and {Schubnell}, M. and {Seo}, H. and {Sharples}, R. and {Silber}, J. and {Sinigaglia}, F. and {Slosar}, A. and {Smith}, A. and {Sprayberry}, D. and {Tan}, T. and {Tarl{\'e}}, G. and {Trusov}, S. and {Vaisakh}, R. and {Valcin}, D. and {Valdes}, F. and {Vargas-Maga{\~n}a}, M. and {Verde}, L. and {Walther}, M. and {Wang}, B. and {Wang}, M.~S. and {Weaver}, B.~A. and {Weaverdyck}, N. and {Wechsler}, R.~H. and {Weinberg}, D.~H. and {White}, M. and {Yu}, J. and {Yu}, Y. and {Yuan}, S. and {Y{\`e}che}, C. and {Zaborowski}, E.~A. and {Zarrouk}, P. and {Zhang}, H. and {Zhao}, C. and {Zhao}, R. and {Zhou}, R. and {Zou}, H.},
        title = "{DESI 2024 IV: Baryon Acoustic Oscillations from the Lyman Alpha Forest}",
      journal = {arXiv e-prints. Accepted for publication in JCAP},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2024,
        month = apr,
          eid = {arXiv:2404.03001},
        pages = {arXiv:2404.03001},
          doi = {10.48550/arXiv.2404.03001},
archivePrefix = {arXiv},
       eprint = {2404.03001},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024arXiv240403001D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DESI2024VI,
       author = {{DESI Collaboration} and {Adame}, A.~G. and {Aguilar}, J. and {Ahlen}, S. and {Alam}, S. and {Alexander}, D.~M. and {Alvarez}, M. and {Alves}, O. and {Anand}, A. and {Andrade}, U. and {Armengaud}, E. and {Avila}, S. and {Aviles}, A. and {Awan}, H. and {Bahr-Kalus}, B. and {Bailey}, S. and {Baltay}, C. and {Bault}, A. and {Behera}, J. and {BenZvi}, S. and {Bera}, A. and {Beutler}, F. and {Bianchi}, D. and {Blake}, C. and {Blum}, R. and {Brieden}, S. and {Brodzeller}, A. and {Brooks}, D. and {Buckley-Geer}, E. and {Burtin}, E. and {Calderon}, R. and {Canning}, R. and {Carnero Rosell}, A. and {Cereskaite}, R. and {Cervantes-Cota}, J.~L. and {Chabanier}, S. and {Chaussidon}, E. and {Chaves-Montero}, J. and {Chen}, S. and {Chen}, X. and {Claybaugh}, T. and {Cole}, S. and {Cuceu}, A. and {Davis}, T.~M. and {Dawson}, K. and {de la Macorra}, A. and {de Mattia}, A. and {Deiosso}, N. and {Dey}, A. and {Dey}, B. and {Ding}, Z. and {Doel}, P. and {Edelstein}, J. and {Eftekharzadeh}, S. and {Eisenstein}, D.~J. and {Elliott}, A. and {Fagrelius}, P. and {Fanning}, K. and {Ferraro}, S. and {Ereza}, J. and {Findlay}, N. and {Flaugher}, B. and {Font-Ribera}, A. and {Forero-S{\'a}nchez}, D. and {Forero-Romero}, J.~E. and {Frenk}, C.~S. and {Garcia-Quintero}, C. and {Gazta{\~n}aga}, E. and {Gil-Mar{\'\i}n}, H. and {Gontcho}, S. Gontcho A and {Gonzalez-Morales}, A.~X. and {Gonzalez-Perez}, V. and {Gordon}, C. and {Green}, D. and {Gruen}, D. and {Gsponer}, R. and {Gutierrez}, G. and {Guy}, J. and {Hadzhiyska}, B. and {Hahn}, C. and {Hanif}, M.~M. S and {Herrera-Alcantar}, H.~K. and {Honscheid}, K. and {Howlett}, C. and {Huterer}, D. and {Ir{\v{s}}i{\v{c}}}, V. and {Ishak}, M. and {Juneau}, S. and {Kara{\c{c}}ayl{\i}}, N.~G. and {Kehoe}, R. and {Kent}, S. and {Kirkby}, D. and {Kremin}, A. and {Krolewski}, A. and {Lai}, Y. and {Lan}, T. -W. and {Landriau}, M. and {Lang}, D. and {Lasker}, J. and {Le Goff}, J.~M. and {Le Guillou}, L. and {Leauthaud}, A. and {Levi}, M.~E. and {Li}, T.~S. and {Linder}, E. and {Lodha}, K. and {Magneville}, C. and {Manera}, M. and {Margala}, D. and {Martini}, P. and {Maus}, M. and {McDonald}, P. and {Medina-Varela}, L. and {Meisner}, A. and {Mena-Fern{\'a}ndez}, J. and {Miquel}, R. and {Moon}, J. and {Moore}, S. and {Moustakas}, J. and {Mudur}, N. and {Mueller}, E. and {Mu{\~n}oz-Guti{\'e}rrez}, A. and {Myers}, A.~D. and {Nadathur}, S. and {Napolitano}, L. and {Neveux}, R. and {Newman}, J.~A. and {Nguyen}, N.~M. and {Nie}, J. and {Niz}, G. and {Noriega}, H.~E. and {Padmanabhan}, N. and {Paillas}, E. and {Palanque-Delabrouille}, N. and {Pan}, J. and {Penmetsa}, S. and {Percival}, W.~J. and {Pieri}, M.~M. and {Pinon}, M. and {Poppett}, C. and {Porredon}, A. and {Prada}, F. and {P{\'e}rez-Fern{\'a}ndez}, A. and {P{\'e}rez-R{\`a}fols}, I. and {Rabinowitz}, D. and {Raichoor}, A. and {Ram{\'\i}rez-P{\'e}rez}, C. and {Ramirez-Solano}, S. and {Ravoux}, C. and {Rashkovetskyi}, M. and {Rezaie}, M. and {Rich}, J. and {Rocher}, A. and {Rockosi}, C. and {Roe}, N.~A. and {Rosado-Marin}, A. and {Ross}, A.~J. and {Rossi}, G. and {Ruggeri}, R. and {Ruhlmann-Kleider}, V. and {Samushia}, L. and {Sanchez}, E. and {Saulder}, C. and {Schlafly}, E.~F. and {Schlegel}, D. and {Schubnell}, M. and {Seo}, H. and {Shafieloo}, A. and {Sharples}, R. and {Silber}, J. and {Slosar}, A. and {Smith}, A. and {Sprayberry}, D. and {Tan}, T. and {Tarl{\'e}}, G. and {Taylor}, P. and {Trusov}, S. and {Ure{\~n}a-L{\'o}pez}, L.~A. and {Vaisakh}, R. and {Valcin}, D. and {Valdes}, F. and {Vargas-Maga{\~n}a}, M. and {Verde}, L. and {Walther}, M. and {Wang}, B. and {Wang}, M.~S. and {Weaver}, B.~A. and {Weaverdyck}, N. and {Wechsler}, R.~H. and {Weinberg}, D.~H. and {White}, M. and {Yu}, J. and {Yu}, Y. and {Yuan}, S. and {Y{\`e}che}, C. and {Zaborowski}, E.~A. and {Zarrouk}, P. and {Zhang}, H. and {Zhao}, C. and {Zhao}, R. and {Zhou}, R. and {Zhuang}, T. and {Zou}, H.},
        title = "{DESI 2024 VI: Cosmological Constraints from the Measurements of Baryon Acoustic Oscillations}",
      journal = {arXiv e-prints. Accepted for publication in JCAP},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2024,
        month = apr,
          eid = {arXiv:2404.03002},
        pages = {arXiv:2404.03002},
          doi = {10.48550/arXiv.2404.03002},
archivePrefix = {arXiv},
       eprint = {2404.03002},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024arXiv240403002D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Dey2018a,
       author = {{Dey}, Arjun and {Schlegel}, David J. and {Lang}, Dustin and
         {Blum}, Robert and {Burleigh}, Kaylan and {Fan}, Xiaohui and
         {Findlay}, Joseph R. and {Finkbeiner}, Doug and {Herrera}, David and
         {Juneau}, St{\'e}phanie and {Landriau}, Martin and {Levi}, Michael and
         {McGreer}, Ian and {Meisner}, Aaron and {Myers}, Adam D. and
         {Moustakas}, John and {Nugent}, Peter and {Patej}, Anna and
         {Schlafly}, Edward F. and {Walker}, Alistair R. and
         {Valdes}, Francisco and {Weaver}, Benjamin A. and
         {Y{\`e}che}, Christophe and {Zou}, Hu and {Zhou}, Xu and
         {Abareshi}, Behzad and {Abbott}, T.~M.~C. and {Abolfathi}, Bela and
         {Aguilera}, C. and {Alam}, Shadab and {Allen}, Lori and {Alvarez}, A. and
         {Annis}, James and {Ansarinejad}, Behzad and {Aubert}, Marie and
         {Beechert}, Jacqueline and {Bell}, Eric F. and {BenZvi}, Segev Y. and
         {Beutler}, Florian and {Bielby}, Richard M. and {Bolton}, Adam S. and
         {Brice{\~n}o}, C{\'e}sar and {Buckley-Geer}, Elizabeth J. and
         {Butler}, Karen and {Calamida}, Annalisa and {Carlberg}, Raymond G. and
         {Carter}, Paul and {Casas}, Ricard and {Castander}, Francisco J. and
         {Choi}, Yumi and {Comparat}, Johan and {Cukanovaite}, Elena and
         {Delubac}, Timoth{\'e}e and {DeVries}, Kaitlin and {Dey}, Sharmila and
         {Dhungana}, Govinda and {Dickinson}, Mark and {Ding}, Zhejie and
         {Donaldson}, John B. and {Duan}, Yutong and
         {Duckworth}, Christopher J. and {Eftekharzadeh}, Sarah and
         {Eisenstein}, Daniel J. and {Etourneau}, Thomas and
         {Fagrelius}, Parker A. and {Farihi}, Jay and {Fitzpatrick}, Mike and
         {Font-Ribera}, Andreu and {Fulmer}, Leah and {G{\"a}nsicke}, Boris T. and
         {Gaztanaga}, Enrique and {George}, Koshy and {Gerdes}, David W. and
         {Gontcho}, Satya Gontcho A. and {Gorgoni}, Claudio and
         {Green}, Gregory and {Guy}, Julien and {Harmer}, Diane and {Hernand
        ez}, M. and {Honscheid}, Klaus and {Huang}, Lijuan Wendy and
         {James}, David J. and {Jannuzi}, Buell T. and {Jiang}, Linhua and
         {Joyce}, Richard and {Karcher}, Armin and {Karkar}, Sonia and
         {Kehoe}, Robert and {Kneib}, Jean-Paul and {Kueter-Young}, Andrea and
         {Lan}, Ting-Wen and {Lauer}, Tod R. and {Le Guillou}, Laurent and
         {Le Van Suu}, Auguste and {Lee}, Jae Hyeon and {Lesser}, Michael and
         {Perreault Levasseur}, Laurence and {Li}, Ting S. and
         {Mann}, Justin L. and {Marshall}, Robert and
         {Mart{\'\i}nez-V{\'a}zquez}, C.~E. and {Martini}, Paul and
         {du Mas des Bourboux}, H{\'e}lion and {McManus}, Sean and
         {Meier}, Tobias Gabriel and {M{\'e}nard}, Brice and {Metcalfe}, Nigel and
         {Mu{\~n}oz-Guti{\'e}rrez}, Andrea and {Najita}, Joan and
         {Napier}, Kevin and {Narayan}, Gautham and {Newman}, Jeffrey A. and
         {Nie}, Jundan and {Nord}, Brian and {Norman}, Dara J. and
         {Olsen}, Knut A.~G. and {Paat}, Anthony and
         {Palanque-Delabrouille}, Nathalie and {Peng}, Xiyan and
         {Poppett}, Claire L. and {Poremba}, Megan R. and {Prakash}, Abhishek and
         {Rabinowitz}, David and {Raichoor}, Anand and {Rezaie}, Mehdi and
         {Robertson}, A.~N. and {Roe}, Natalie A. and {Ross}, Ashley J. and
         {Ross}, Nicholas P. and {Rudnick}, Gregory and {Safonova}, Sasha and
         {Saha}, Abhijit and {S{\'a}nchez}, F. Javier and {Savary}, Elodie and
         {Schweiker}, Heidi and {Scott}, Adam and {Seo}, Hee-Jong and
         {Shan}, Huanyuan and {Silva}, David R. and {Slepian}, Zachary and
         {Soto}, Christian and {Sprayberry}, David and {Staten}, Ryan and
         {Stillman}, Coley M. and {Stupak}, Robert J. and {Summers}, David L. and
         {Sien Tie}, Suk and {Tirado}, H. and {Vargas-Maga{\~n}a}, Mariana and
         {Vivas}, A. Katherina and {Wechsler}, Risa H. and {Williams}, Doug and
         {Yang}, Jinyi and {Yang}, Qian and {Yapici}, Tolga and
         {Zaritsky}, Dennis and {Zenteno}, A. and {Zhang}, Kai and
         {Zhang}, Tianmeng and {Zhou}, Rongpu and {Zhou}, Zhimin},
        title = "{Overview of the DESI Legacy Imaging Surveys}",
      journal = {\aj},
     keywords = {catalogs, surveys, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2019,
        month = may,
       volume = {157},
       number = {5},
          eid = {168},
        pages = {168},
          doi = {10.3847/1538-3881/ab089d},
archivePrefix = {arXiv},
       eprint = {1804.08657},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019AJ....157..168D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Duncan2022,
       author = {{Duncan}, Kenneth J.},
        title = "{All-purpose, all-sky photometric redshifts for the Legacy Imaging Surveys Data Release 8}",
      journal = {\mnras},
     keywords = {catalogues, galaxies: distances and redshifts, quasars: general, radio continuum: galaxies, X-rays: galaxies, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2022,
        month = may,
       volume = {512},
       number = {3},
        pages = {3662-3683},
          doi = {10.1093/mnras/stac608},
archivePrefix = {arXiv},
       eprint = {2203.01949},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.512.3662D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Falco1985,
       author = {{Falco}, E.~E. and {Gorenstein}, M.~V. and {Shapiro}, I.~I.},
        title = "{On model-dependent bounds on H 0 from gravitational images : application to Q 0957+561 A, B.}",
      journal = {\apjl},
     keywords = {Astronomical Models, Background Radiation, Gravitational Lenses, Mass Distribution, Quasars, Radiation Sources, Galactic Clusters, Geometrical Optics, Hubble Diagram, Astrophysics},
         year = 1985,
        month = feb,
       volume = {289},
        pages = {L1-L4},
          doi = {10.1086/184422},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1985ApJ...289L...1F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{ForemanMackey2014a,
       author = {{Foreman-Mackey}, Dan and {Sick}, Jonathan and {Johnson}, Ben},
        title = "{Python-Fsps: Python Bindings To Fsps (V0.1.1)}",
         year = 2014,
        month = oct,
          eid = {10.5281/zenodo.12157},
          doi = {10.5281/zenodo.12157},
      version = {v0.1.1},
    publisher = {Zenodo},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014zndo.....12157F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fremling2020,
       author = {{Fremling}, C. and {Miller}, A.~A. and {Sharma}, Y. and {Dugas}, A. and {Perley}, D.~A. and {Taggart}, K. and {Sollerman}, J. and {Goobar}, A. and {Graham}, M.~L. and {Neill}, J.~D. and {Nordin}, J. and {Rigault}, M. and {Walters}, R. and {Andreoni}, I. and {Bagdasaryan}, A. and {Belicki}, J. and {Cannella}, C. and {Bellm}, E.~C. and {Cenko}, S.~B. and {De}, K. and {Dekany}, R. and {Frederick}, S. and {Golkhou}, V.~Z. and {Graham}, M.~J. and {Helou}, G. and {Ho}, A.~Y.~Q. and {Kasliwal}, M.~M. and {Kupfer}, T. and {Laher}, R.~R. and {Mahabal}, A. and {Masci}, F.~J. and {Riddle}, R. and {Rusholme}, B. and {Schulze}, S. and {Shupe}, D.~L. and {Smith}, R.~M. and {van Velzen}, S. and {Yan}, Lin and {Yao}, Y. and {Zhuang}, Z. and {Kulkarni}, S.~R.},
        title = "{The Zwicky Transient Facility Bright Transient Survey. I. Spectroscopic Classification and the Redshift Completeness of Local Galaxy Catalogs}",
      journal = {\apj},
     keywords = {Supernovae, Galaxies, Redshift surveys, Surveys, 1668, 573, 1378, 1671, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = may,
       volume = {895},
       number = {1},
          eid = {32},
        pages = {32},
          doi = {10.3847/1538-4357/ab8943},
archivePrefix = {arXiv},
       eprint = {1910.12973},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...895...32F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Frye2023,
       author = {{Frye}, Brenda L. and {Pascale}, Massimo and {Pierel}, Justin and {Chen}, Wenlei and {Foo}, Nicholas and {Leimbach}, Reagen and {Garuda}, Nikhil and {Cohen}, Seth H. and {Kamieneski}, Patrick S. and {Windhorst}, Rogier A. and {Koekemoer}, Anton M. and {Kelly}, Pat and {Summers}, Jake and {Engesser}, Michael and {Liu}, Daizhong and {Furtak}, Lukas J. and {Polletta}, Maria del Caren and {Harrington}, Kevin C. and {Willner}, S.~P. and {Diego}, Jose M. and {Jansen}, Rolf A. and {Coe}, Dan and {Conselice}, Christopher J. and {Dai}, Liang and {Dole}, Herv{\'e} and {D'Silva}, Jordan C.~J. and {Driver}, Simon P. and {Grogin}, Norman A. and {Marshall}, Madeline A. and {Meena}, Ashish K. and {Nonino}, Mario and {Ortiz}, Rafael and {Pirzkal}, Nor and {Robotham}, Aaron and {Ryan}, Russell E. and {Strolger}, Lou and {Tompkins}, Scott and {Willmer}, Christopher N.~A. and {Yan}, Haojing and {Yun}, Min S. and {Zitrin}, Adi},
        title = "{The JWST Discovery of the Triply Imaged Type Ia ``Supernova H0pe'' and Observations of the Galaxy Cluster PLCK G165.7+67.0}",
      journal = {\apj},
     keywords = {Strong gravitational lensing, Rich galaxy clusters, High-redshift galaxy clusters, Galaxy cluster counts, Galaxy spectroscopy, 1643, 2005, 2007, 583, 2171, Astrophysics - Astrophysics of Galaxies},
         year = 2024,
        month = feb,
       volume = {961},
       number = {2},
          eid = {171},
        pages = {171},
          doi = {10.3847/1538-4357/ad1034},
archivePrefix = {arXiv},
       eprint = {2309.07326},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024ApJ...961..171F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GalYam2009,
       author = {{Gal-Yam}, A. and {Mazzali}, P. and {Ofek}, E.~O. and {Nugent}, P.~E. and {Kulkarni}, S.~R. and {Kasliwal}, M.~M. and {Quimby}, R.~M. and {Filippenko}, A.~V. and {Cenko}, S.~B. and {Chornock}, R. and {Waldman}, R. and {Kasen}, D. and {Sullivan}, M. and {Beshore}, E.~C. and {Drake}, A.~J. and {Thomas}, R.~C. and {Bloom}, J.~S. and {Poznanski}, D. and {Miller}, A.~A. and {Foley}, R.~J. and {Silverman}, J.~M. and {Arcavi}, I. and {Ellis}, R.~S. and {Deng}, J.},
        title = "{Supernova 2007bi as a pair-instability explosion}",
      journal = {\nat},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2009,
        month = dec,
       volume = {462},
       number = {7273},
        pages = {624-627},
          doi = {10.1038/nature08579},
archivePrefix = {arXiv},
       eprint = {1001.1156},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009Natur.462..624G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GalYam2012,
       author = {{Gal-Yam}, Avishay},
        title = "{Luminous Supernovae}",
      journal = {Science},
     keywords = {ASTRONOMY, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = aug,
       volume = {337},
       number = {6097},
        pages = {927},
          doi = {10.1126/science.1203601},
archivePrefix = {arXiv},
       eprint = {1208.3217},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012Sci...337..927G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Gkini2022,
       author = {{Gkini}, A. and {Yan}, L. and {Perley}, D.~A. and {Lunnan}, R. and {Chen}, T. and {Schulze}, S. and {Kangas}, T. and {Sollerman}, J. and {Gal-Yam}, A.},
        title = "{ZTF superluminous supernova candidates}",
      journal = {Transient Name Server AstroNote},
     keywords = {Supernova, Transient, ZTF22aadrjte, 2022hdn, AT2022hdn, AT 2022hdn, ZTF22aadeqlh, 2022fwi, AT2022fwi, AT 2022fwi, ZTF22aadqmen, 2022gxk, AT2022gxk, AT 2022gxk, ZTF22aagzbux, 2022hwk, AT2022hwk, AT 2022hwk, ZTF22aagyrdr, 2022hvd, AT2022hvd, AT 2022hvd, ZTF22aaibiqg, 2022ise, AT2022ise, AT 2022ise, ZTF22aahmgmv, 2022iab, AT2022iab, AT 2022iab, ZTF22aafafbt, 2022hmx, AT2022hmx, AT 2022hmx, ZTF22aahiien, 2022ifk, AT2022ifk, AT 2022ifk},
         year = 2022,
        month = jun,
       volume = {124},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022TNSAN.124....1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Goldstein2017,
       author = {{Goldstein}, Daniel A. and {Nugent}, Peter E.},
        title = "{How to Find Gravitationally Lensed Type Ia Supernovae}",
      journal = {\apjl},
     keywords = {methods: observational, supernovae: general, surveys, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = jan,
       volume = {834},
       number = {1},
          eid = {L5},
        pages = {L5},
          doi = {10.3847/2041-8213/834/1/L5},
archivePrefix = {arXiv},
       eprint = {1611.09459},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...834L...5G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Goldstein2019,
       author = {{Goldstein}, Daniel A. and {Nugent}, Peter E. and {Goobar}, Ariel},
        title = "{Rates and Properties of Supernovae Strongly Gravitationally Lensed by Elliptical Galaxies in Time-domain Imaging Surveys}",
      journal = {\apjs},
     keywords = {gravitational lensing: strong, supernovae: general, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2019,
        month = jul,
       volume = {243},
       number = {1},
          eid = {6},
        pages = {6},
          doi = {10.3847/1538-4365/ab1fe0},
archivePrefix = {arXiv},
       eprint = {1809.10147},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJS..243....6G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Goobar2002,
       author = {{Goobar}, A. and {M{\"o}rtsell}, E. and {Amanullah}, R. and {Nugent}, P.},
        title = "{Cosmological parameters from lensed supernovae}",
      journal = {\aap},
     keywords = {gravitational lensing, cosmology: cosmological parameters, Astrophysics},
         year = 2002,
        month = oct,
       volume = {393},
        pages = {25-32},
          doi = {10.1051/0004-6361:20020987},
archivePrefix = {arXiv},
       eprint = {astro-ph/0207139},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002A&A...393...25G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Goobar2009,
       author = {{Goobar}, A. and {Paech}, K. and {Stanishev}, V. and {Amanullah}, R. and {Dahl{\'e}n}, T. and {J{\"o}nsson}, J. and {Kneib}, J.~P. and {Lidman}, C. and {Limousin}, M. and {M{\"o}rtsell}, E. and {Nobili}, S. and {Richard}, J. and {Riehm}, T. and {von Strauss}, M.},
        title = "{Near-IR search for lensed supernovae behind galaxy clusters. II. First detection and future prospects}",
      journal = {\aap},
     keywords = {cosmology: observations, stars: supernovae: general, galaxies: clusters: general, gravitational lensing, Astrophysics},
         year = 2009,
        month = nov,
       volume = {507},
       number = {1},
        pages = {71-83},
          doi = {10.1051/0004-6361/200811254},
archivePrefix = {arXiv},
       eprint = {0810.4932},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009A&A...507...71G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Goobar2017,
       author = {{Goobar}, A. and {Amanullah}, R. and {Kulkarni}, S.~R. and {Nugent}, P.~E. and {Johansson}, J. and {Steidel}, C. and {Law}, D. and {M{\"o}rtsell}, E. and {Quimby}, R. and {Blagorodnova}, N. and {Brandeker}, A. and {Cao}, Y. and {Cooray}, A. and {Ferretti}, R. and {Fremling}, C. and {Hangard}, L. and {Kasliwal}, M. and {Kupfer}, T. and {Lunnan}, R. and {Masci}, F. and {Miller}, A.~A. and {Nayyeri}, H. and {Neill}, J.~D. and {Ofek}, E.~O. and {Papadogiannakis}, S. and {Petrushevska}, T. and {Ravi}, V. and {Sollerman}, J. and {Sullivan}, M. and {Taddia}, F. and {Walters}, R. and {Wilson}, D. and {Yan}, L. and {Yaron}, O.},
        title = "{iPTF16geu: A multiply imaged, gravitationally lensed type Ia supernova}",
      journal = {Science},
     keywords = {ASTRONOMY, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2017,
        month = apr,
       volume = {356},
       number = {6335},
        pages = {291-295},
          doi = {10.1126/science.aal2729},
archivePrefix = {arXiv},
       eprint = {1611.00014},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017Sci...356..291G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Goobar2023,
       author = {{Goobar}, Ariel and {Johansson}, Joel and {Schulze}, Steve and {Arendse}, Nikki and {Carracedo}, Ana Sagu{\'e}s and {Dhawan}, Suhail and {M{\"o}rtsell}, Edvard and {Fremling}, Christoffer and {Yan}, Lin and {Perley}, Daniel and {Sollerman}, Jesper and {Joseph}, R{\'e}my and {Hinds}, K. -Ryan and {Meynardie}, William and {Andreoni}, Igor and {Bellm}, Eric and {Bloom}, Josh and {Collett}, Thomas E. and {Drake}, Andrew and {Graham}, Matthew and {Kasliwal}, Mansi and {Kulkarni}, Shri R. and {Lemon}, Cameron and {Miller}, Adam A. and {Neill}, James D. and {Nordin}, Jakob and {Pierel}, Justin and {Richard}, Johan and {Riddle}, Reed and {Rigault}, Mickael and {Rusholme}, Ben and {Sharma}, Yashvi and {Stein}, Robert and {Stewart}, Gabrielle and {Townsend}, Alice and {Vinko}, Jozsef and {Wheeler}, J. Craig and {Wold}, Avery},
        title = "{Uncovering a population of gravitational lens galaxies with magnified standard candle SN Zwicky}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2023,
        month = jun,
       volume = {7},
        pages = {1098-1107},
          doi = {10.1038/s41550-023-01981-3},
archivePrefix = {arXiv},
       eprint = {2211.00656},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023NatAs...7.1098G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Goobar2024,
       author = {{Goobar}, Ariel and {Johansson}, Joel and {Sagu{\'e}s Carracedo}, Ana},
        title = "{Strongly lensed supernovae: lessons learned}",
      journal = {arXiv e-prints. Accepted for publication in Philosophical Transactions A},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2024,
        month = jun,
          eid = {arXiv:2406.13519},
        pages = {arXiv:2406.13519},
          doi = {10.48550/arXiv.2406.13519},
archivePrefix = {arXiv},
       eprint = {2406.13519},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024arXiv240613519G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Graham2019,
       author = {{Graham}, Matthew J. and {Kulkarni}, S.~R. and {Bellm}, Eric C. and {Adams}, Scott M. and {Barbarino}, Cristina and {Blagorodnova}, Nadejda and {Bodewits}, Dennis and {Bolin}, Bryce and {Brady}, Patrick R. and {Cenko}, S. Bradley and {Chang}, Chan-Kao and {Coughlin}, Michael W. and {De}, Kishalay and {Eadie}, Gwendolyn and {Farnham}, Tony L. and {Feindt}, Ulrich and {Franckowiak}, Anna and {Fremling}, Christoffer and {Gezari}, Suvi and {Ghosh}, Shaon and {Goldstein}, Daniel A. and {Golkhou}, V. Zach and {Goobar}, Ariel and {Ho}, Anna Y.~Q. and {Huppenkothen}, Daniela and {Ivezi{\'c}}, {\v{Z}}eljko and {Jones}, R. Lynne and {Juric}, Mario and {Kaplan}, David L. and {Kasliwal}, Mansi M. and {Kelley}, Michael S.~P. and {Kupfer}, Thomas and {Lee}, Chien-De and {Lin}, Hsing Wen and {Lunnan}, Ragnhild and {Mahabal}, Ashish A. and {Miller}, Adam A. and {Ngeow}, Chow-Choong and {Nugent}, Peter and {Ofek}, Eran O. and {Prince}, Thomas A. and {Rauch}, Ludwig and {van Roestel}, Jan and {Schulze}, Steve and {Singer}, Leo P. and {Sollerman}, Jesper and {Taddia}, Francesco and {Yan}, Lin and {Ye}, Quan-Zhi and {Yu}, Po-Chieh and {Barlow}, Tom and {Bauer}, James and {Beck}, Ron and {Belicki}, Justin and {Biswas}, Rahul and {Brinnel}, Valery and {Brooke}, Tim and {Bue}, Brian and {Bulla}, Mattia and {Burruss}, Rick and {Connolly}, Andrew and {Cromer}, John and {Cunningham}, Virginia and {Dekany}, Richard and {Delacroix}, Alex and {Desai}, Vandana and {Duev}, Dmitry A. and {Feeney}, Michael and {Flynn}, David and {Frederick}, Sara and {Gal-Yam}, Avishay and {Giomi}, Matteo and {Groom}, Steven and {Hacopians}, Eugean and {Hale}, David and {Helou}, George and {Henning}, John and {Hover}, David and {Hillenbrand}, Lynne A. and {Howell}, Justin and {Hung}, Tiara and {Imel}, David and {Ip}, Wing-Huen and {Jackson}, Edward and {Kaspi}, Shai and {Kaye}, Stephen and {Kowalski}, Marek and {Kramer}, Emily and {Kuhn}, Michael and {Landry}, Walter and {Laher}, Russ R. and {Mao}, Peter and {Masci}, Frank J. and {Monkewitz}, Serge and {Murphy}, Patrick and {Nordin}, Jakob and {Patterson}, Maria T. and {Penprase}, Bryan and {Porter}, Michael and {Rebbapragada}, Umaa and {Reiley}, Dan and {Riddle}, Reed and {Rigault}, Mickael and {Rodriguez}, Hector and {Rusholme}, Ben and {van Santen}, Jakob and {Shupe}, David L. and {Smith}, Roger M. and {Soumagnac}, Maayane T. and {Stein}, Robert and {Surace}, Jason and {Szkody}, Paula and {Terek}, Scott and {Van Sistine}, Angela and {van Velzen}, Sjoert and {Vestrand}, W. Thomas and {Walters}, Richard and {Ward}, Charlotte and {Zhang}, Chaoran and {Zolkower}, Jeffry},
        title = "{The Zwicky Transient Facility: Science Objectives}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = jul,
       volume = {131},
       number = {1001},
        pages = {078001},
          doi = {10.1088/1538-3873/ab006c},
archivePrefix = {arXiv},
       eprint = {1902.01945},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PASP..131g8001G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Guillochon2013,
       author = {{Guillochon}, James and {Ramirez-Ruiz}, Enrico},
        title = "{Hydrodynamical Simulations to Determine the Feeding Rate of Black Holes by the Tidal Disruption of Stars: The Importance of the Impact Parameter and Stellar Structure}",
      journal = {\apj},
     keywords = {accretion, accretion disks, black hole physics, gravitation, hydrodynamics, methods: numerical, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = apr,
       volume = {767},
       number = {1},
          eid = {25},
        pages = {25},
          doi = {10.1088/0004-637X/767/1/25},
archivePrefix = {arXiv},
       eprint = {1206.2350},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...767...25G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Guillochon2018,
       author = {{Guillochon}, James and {Nicholl}, Matt and {Villar}, V. Ashley and {Mockler}, Brenna and {Narayan}, Gautham and {Mandel}, Kaisey S. and {Berger}, Edo and {Williams}, Peter K.~G.},
        title = "{MOSFiT: Modular Open Source Fitter for Transients}",
      journal = {\apjs},
     keywords = {catalogs, methods: data analysis, methods: numerical, methods: statistical, supernovae: general, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = may,
       volume = {236},
       number = {1},
          eid = {6},
        pages = {6},
          doi = {10.3847/1538-4365/aab761},
archivePrefix = {arXiv},
       eprint = {1710.02145},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJS..236....6G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Guy2007,
       author = {{Guy}, J. and {Astier}, P. and {Baumont}, S. and {Hardin}, D. and {Pain}, R. and {Regnault}, N. and {Basa}, S. and {Carlberg}, R.~G. and {Conley}, A. and {Fabbro}, S. and {Fouchez}, D. and {Hook}, I.~M. and {Howell}, D.~A. and {Perrett}, K. and {Pritchet}, C.~J. and {Rich}, J. and {Sullivan}, M. and {Antilogus}, P. and {Aubourg}, E. and {Bazin}, G. and {Bronder}, J. and {Filiol}, M. and {Palanque-Delabrouille}, N. and {Ripoche}, P. and {Ruhlmann-Kleider}, V.},
        title = "{SALT2: using distant supernovae to improve the use of type Ia supernovae as distance indicators}",
      journal = {\aap},
     keywords = {supernovae: general, cosmology: observations, Astrophysics},
         year = 2007,
        month = apr,
       volume = {466},
       number = {1},
        pages = {11-21},
          doi = {10.1051/0004-6361:20066930},
archivePrefix = {arXiv},
       eprint = {astro-ph/0701828},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007A&A...466...11G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Howell2006,
       author = {{Howell}, D. Andrew and {Sullivan}, Mark and {Nugent}, Peter E. and {Ellis}, Richard S. and {Conley}, Alexander J. and {Le Borgne}, Damien and {Carlberg}, Raymond G. and {Guy}, Julien and {Balam}, David and {Basa}, Stephane and {Fouchez}, Dominique and {Hook}, Isobel M. and {Hsiao}, Eric Y. and {Neill}, James D. and {Pain}, Reynald and {Perrett}, Kathryn M. and {Pritchet}, Christopher J.},
        title = "{The type Ia supernova SNLS-03D3bb from a super-Chandrasekhar-mass white dwarf star}",
      journal = {\nat},
     keywords = {Astrophysics},
         year = 2006,
        month = sep,
       volume = {443},
       number = {7109},
        pages = {308-311},
          doi = {10.1038/nature05103},
archivePrefix = {arXiv},
       eprint = {astro-ph/0609616},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006Natur.443..308H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hsiao2020,
       author = {{Hsiao}, E.~Y. and {Hoeflich}, P. and {Ashall}, C. and {Lu}, J. and {Contreras}, C. and {Burns}, C.~R. and {Phillips}, M.~M. and {Galbany}, L. and {Anderson}, J.~P. and {Baltay}, C. and {Baron}, E. and {Castell{\'o}n}, S. and {Davis}, S. and {Freedman}, Wendy L. and {Gall}, C. and {Gonzalez}, C. and {Graham}, M.~L. and {Hamuy}, M. and {Holoien}, T.~W. -S. and {Karamehmetoglu}, E. and {Krisciunas}, K. and {Kumar}, S. and {Kuncarayakti}, H. and {Morrell}, N. and {Moriya}, T.~J. and {Nugent}, P.~E. and {Perlmutter}, S. and {Persson}, S.~E. and {Piro}, A.~L. and {Rabinowitz}, D. and {Roth}, M. and {Shahbandeh}, M. and {Shappee}, B.~J. and {Stritzinger}, M.~D. and {Suntzeff}, N.~B. and {Taddia}, F. and {Uddin}, S.~A.},
        title = "{Carnegie Supernova Project II: The Slowest Rising Type Ia Supernova LSQ14fmg and Clues to the Origin of Super-Chandrasekhar/03fg-like Events}",
      journal = {\apj},
     keywords = {Type Ia supernovae, Asymptotic giant branch stars, Stellar winds, 1728, 2100, 1636, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = sep,
       volume = {900},
       number = {2},
          eid = {140},
        pages = {140},
          doi = {10.3847/1538-4357/abaf4c},
archivePrefix = {arXiv},
       eprint = {2008.05614},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...900..140H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Ivezic2019,
       author = {{Ivezi{\'c}}, {\v{Z}}eljko and {Kahn}, Steven M. and {Tyson}, J. Anthony and {Abel}, Bob and {Acosta}, Emily and {Allsman}, Robyn and {Alonso}, David and {AlSayyad}, Yusra and {Anderson}, Scott F. and {Andrew}, John and {Angel}, James Roger P. and {Angeli}, George Z. and {Ansari}, Reza and {Antilogus}, Pierre and {Araujo}, Constanza and {Armstrong}, Robert and {Arndt}, Kirk T. and {Astier}, Pierre and {Aubourg}, {\'E}ric and {Auza}, Nicole and {Axelrod}, Tim S. and {Bard}, Deborah J. and {Barr}, Jeff D. and {Barrau}, Aurelian and {Bartlett}, James G. and {Bauer}, Amanda E. and {Bauman}, Brian J. and {Baumont}, Sylvain and {Bechtol}, Ellen and {Bechtol}, Keith and {Becker}, Andrew C. and {Becla}, Jacek and {Beldica}, Cristina and {Bellavia}, Steve and {Bianco}, Federica B. and {Biswas}, Rahul and {Blanc}, Guillaume and {Blazek}, Jonathan and {Blandford}, Roger D. and {Bloom}, Josh S. and {Bogart}, Joanne and {Bond}, Tim W. and {Booth}, Michael T. and {Borgland}, Anders W. and {Borne}, Kirk and {Bosch}, James F. and {Boutigny}, Dominique and {Brackett}, Craig A. and {Bradshaw}, Andrew and {Brandt}, William Nielsen and {Brown}, Michael E. and {Bullock}, James S. and {Burchat}, Patricia and {Burke}, David L. and {Cagnoli}, Gianpietro and {Calabrese}, Daniel and {Callahan}, Shawn and {Callen}, Alice L. and {Carlin}, Jeffrey L. and {Carlson}, Erin L. and {Chandrasekharan}, Srinivasan and {Charles-Emerson}, Glenaver and {Chesley}, Steve and {Cheu}, Elliott C. and {Chiang}, Hsin-Fang and {Chiang}, James and {Chirino}, Carol and {Chow}, Derek and {Ciardi}, David R. and {Claver}, Charles F. and {Cohen-Tanugi}, Johann and {Cockrum}, Joseph J. and {Coles}, Rebecca and {Connolly}, Andrew J. and {Cook}, Kem H. and {Cooray}, Asantha and {Covey}, Kevin R. and {Cribbs}, Chris and {Cui}, Wei and {Cutri}, Roc and {Daly}, Philip N. and {Daniel}, Scott F. and {Daruich}, Felipe and {Daubard}, Guillaume and {Daues}, Greg and {Dawson}, William and {Delgado}, Francisco and {Dellapenna}, Alfred and {de Peyster}, Robert and {de Val-Borro}, Miguel and {Digel}, Seth W. and {Doherty}, Peter and {Dubois}, Richard and {Dubois-Felsmann}, Gregory P. and {Durech}, Josef and {Economou}, Frossie and {Eifler}, Tim and {Eracleous}, Michael and {Emmons}, Benjamin L. and {Fausti Neto}, Angelo and {Ferguson}, Henry and {Figueroa}, Enrique and {Fisher-Levine}, Merlin and {Focke}, Warren and {Foss}, Michael D. and {Frank}, James and {Freemon}, Michael D. and {Gangler}, Emmanuel and {Gawiser}, Eric and {Geary}, John C. and {Gee}, Perry and {Geha}, Marla and {Gessner}, Charles J.~B. and {Gibson}, Robert R. and {Gilmore}, D. Kirk and {Glanzman}, Thomas and {Glick}, William and {Goldina}, Tatiana and {Goldstein}, Daniel A. and {Goodenow}, Iain and {Graham}, Melissa L. and {Gressler}, William J. and {Gris}, Philippe and {Guy}, Leanne P. and {Guyonnet}, Augustin and {Haller}, Gunther and {Harris}, Ron and {Hascall}, Patrick A. and {Haupt}, Justine and {Hernandez}, Fabio and {Herrmann}, Sven and {Hileman}, Edward and {Hoblitt}, Joshua and {Hodgson}, John A. and {Hogan}, Craig and {Howard}, James D. and {Huang}, Dajun and {Huffer}, Michael E. and {Ingraham}, Patrick and {Innes}, Walter R. and {Jacoby}, Suzanne H. and {Jain}, Bhuvnesh and {Jammes}, Fabrice and {Jee}, M. James and {Jenness}, Tim and {Jernigan}, Garrett and {Jevremovi{\'c}}, Darko and {Johns}, Kenneth and {Johnson}, Anthony S. and {Johnson}, Margaret W.~G. and {Jones}, R. Lynne and {Juramy-Gilles}, Claire and {Juri{\'c}}, Mario and {Kalirai}, Jason S. and {Kallivayalil}, Nitya J. and {Kalmbach}, Bryce and {Kantor}, Jeffrey P. and {Karst}, Pierre and {Kasliwal}, Mansi M. and {Kelly}, Heather and {Kessler}, Richard and {Kinnison}, Veronica and {Kirkby}, David and {Knox}, Lloyd and {Kotov}, Ivan V. and {Krabbendam}, Victor L. and {Krughoff}, K. Simon and {Kub{\'a}nek}, Petr and {Kuczewski}, John and {Kulkarni}, Shri and {Ku}, John and {Kurita}, Nadine R. and {Lage}, Craig S. and {Lambert}, Ron and {Lange}, Travis and {Langton}, J. Brian and {Le Guillou}, Laurent and {Levine}, Deborah and {Liang}, Ming and {Lim}, Kian-Tat and {Lintott}, Chris J. and {Long}, Kevin E. and {Lopez}, Margaux and {Lotz}, Paul J. and {Lupton}, Robert H. and {Lust}, Nate B. and {MacArthur}, Lauren A. and {Mahabal}, Ashish and {Mandelbaum}, Rachel and {Markiewicz}, Thomas W. and {Marsh}, Darren S. and {Marshall}, Philip J. and {Marshall}, Stuart and {May}, Morgan and {McKercher}, Robert and {McQueen}, Michelle and {Meyers}, Joshua and {Migliore}, Myriam and {Miller}, Michelle and {Mills}, David J. and {Miraval}, Connor and {Moeyens}, Joachim and {Moolekamp}, Fred E. and {Monet}, David G. and {Moniez}, Marc and {Monkewitz}, Serge and {Montgomery}, Christopher and {Morrison}, Christopher B. and {Mueller}, Fritz and {Muller}, Gary P. and {Mu{\~n}oz Arancibia}, Freddy and {Neill}, Douglas R. and {Newbry}, Scott P. and {Nief}, Jean-Yves and {Nomerotski}, Andrei and {Nordby}, Martin and {O'Connor}, Paul and {Oliver}, John and {Olivier}, Scot S. and {Olsen}, Knut and {O'Mullane}, William and {Ortiz}, Sandra and {Osier}, Shawn and {Owen}, Russell E. and {Pain}, Reynald and {Palecek}, Paul E. and {Parejko}, John K. and {Parsons}, James B. and {Pease}, Nathan M. and {Peterson}, J. Matt and {Peterson}, John R. and {Petravick}, Donald L. and {Libby Petrick}, M.~E. and {Petry}, Cathy E. and {Pierfederici}, Francesco and {Pietrowicz}, Stephen and {Pike}, Rob and {Pinto}, Philip A. and {Plante}, Raymond and {Plate}, Stephen and {Plutchak}, Joel P. and {Price}, Paul A. and {Prouza}, Michael and {Radeka}, Veljko and {Rajagopal}, Jayadev and {Rasmussen}, Andrew P. and {Regnault}, Nicolas and {Reil}, Kevin A. and {Reiss}, David J. and {Reuter}, Michael A. and {Ridgway}, Stephen T. and {Riot}, Vincent J. and {Ritz}, Steve and {Robinson}, Sean and {Roby}, William and {Roodman}, Aaron and {Rosing}, Wayne and {Roucelle}, Cecille and {Rumore}, Matthew R. and {Russo}, Stefano and {Saha}, Abhijit and {Sassolas}, Benoit and {Schalk}, Terry L. and {Schellart}, Pim and {Schindler}, Rafe H. and {Schmidt}, Samuel and {Schneider}, Donald P. and {Schneider}, Michael D. and {Schoening}, William and {Schumacher}, German and {Schwamb}, Megan E. and {Sebag}, Jacques and {Selvy}, Brian and {Sembroski}, Glenn H. and {Seppala}, Lynn G. and {Serio}, Andrew and {Serrano}, Eduardo and {Shaw}, Richard A. and {Shipsey}, Ian and {Sick}, Jonathan and {Silvestri}, Nicole and {Slater}, Colin T. and {Smith}, J. Allyn and {Smith}, R. Chris and {Sobhani}, Shahram and {Soldahl}, Christine and {Storrie-Lombardi}, Lisa and {Stover}, Edward and {Strauss}, Michael A. and {Street}, Rachel A. and {Stubbs}, Christopher W. and {Sullivan}, Ian S. and {Sweeney}, Donald and {Swinbank}, John D. and {Szalay}, Alexander and {Takacs}, Peter and {Tether}, Stephen A. and {Thaler}, Jon J. and {Thayer}, John Gregg and {Thomas}, Sandrine and {Thornton}, Adam J. and {Thukral}, Vaikunth and {Tice}, Jeffrey and {Trilling}, David E. and {Turri}, Max and {Van Berg}, Richard and {Vanden Berk}, Daniel and {Vetter}, Kurt and {Virieux}, Francoise and {Vucina}, Tomislav and {Wahl}, William and {Walkowicz}, Lucianne and {Walsh}, Brian and {Walter}, Christopher W. and {Wang}, Daniel L. and {Wang}, Shin-Yawn and {Warner}, Michael and {Wiecha}, Oliver and {Willman}, Beth and {Winters}, Scott E. and {Wittman}, David and {Wolff}, Sidney C. and {Wood-Vasey}, W. Michael and {Wu}, Xiuqin and {Xin}, Bo and {Yoachim}, Peter and {Zhan}, Hu},
        title = "{LSST: From Science Drivers to Reference Design and Anticipated Data Products}",
      journal = {\apj},
     keywords = {astrometry, cosmology: observations, Galaxy: general, methods: observational, stars: general, surveys, Astrophysics},
         year = 2019,
        month = mar,
       volume = {873},
       number = {2},
          eid = {111},
        pages = {111},
          doi = {10.3847/1538-4357/ab042c},
archivePrefix = {arXiv},
       eprint = {0805.2366},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...873..111I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Johansson2021,
       author = {{Johansson}, J. and {Goobar}, A. and {Price}, S.~H. and {Sagu{\'e}s Carracedo}, A. and {Della Bruna}, L. and {Nugent}, P.~E. and {Dhawan}, S. and {M{\"o}rtsell}, E. and {Papadogiannakis}, S. and {Amanullah}, R. and {Goldstein}, D. and {Cenko}, S.~B. and {De}, K. and {Dugas}, A. and {Kasliwal}, M.~M. and {Kulkarni}, S.~R. and {Lunnan}, R.},
        title = "{Spectroscopy of the first resolved strongly lensed Type Ia supernova iPTF16geu}",
      journal = {\mnras},
     keywords = {gravitational lensing: strong, supernovae: general, supernova: individual (iPTF16geu), Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = mar,
       volume = {502},
       number = {1},
        pages = {510-520},
          doi = {10.1093/mnras/staa3829},
archivePrefix = {arXiv},
       eprint = {2004.10164},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.502..510J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Johnson2021a,
       author = {{Johnson}, Benjamin D. and {Leja}, Joel and {Conroy}, Charlie and {Speagle}, Joshua S.},
        title = "{Stellar Population Inference with Prospector}",
      journal = {\apjs},
     keywords = {Galaxy evolution, Spectral energy distribution, Astronomy data modeling, 594, 2129, 1859, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2021,
        month = jun,
       volume = {254},
       number = {2},
          eid = {22},
        pages = {22},
          doi = {10.3847/1538-4365/abef67},
archivePrefix = {arXiv},
       eprint = {2012.01426},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJS..254...22J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kasen2010,
       author = {{Kasen}, Daniel and {Bildsten}, Lars},
        title = "{Supernova Light Curves Powered by Young Magnetars}",
      journal = {\apj},
     keywords = {radiative transfer, stars: neutron, supernovae: general, supernovae: individual: SN 2005ap SN 2008es SN 2007bi, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2010,
        month = jul,
       volume = {717},
       number = {1},
        pages = {245-249},
          doi = {10.1088/0004-637X/717/1/245},
archivePrefix = {arXiv},
       eprint = {0911.0680},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...717..245K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Kelly2015,
       author = {{Kelly}, Patrick L. and {Rodney}, Steven A. and {Treu}, Tommaso and {Foley}, Ryan J. and {Brammer}, Gabriel and {Schmidt}, Kasper B. and {Zitrin}, Adi and {Sonnenfeld}, Alessandro and {Strolger}, Louis-Gregory and {Graur}, Or and {Filippenko}, Alexei V. and {Jha}, Saurabh W. and {Riess}, Adam G. and {Bradac}, Marusa and {Weiner}, Benjamin J. and {Scolnic}, Daniel and {Malkan}, Matthew A. and {von der Linden}, Anja and {Trenti}, Michele and {Hjorth}, Jens and {Gavazzi}, Raphael and {Fontana}, Adriano and {Merten}, Julian C. and {McCully}, Curtis and {Jones}, Tucker and {Postman}, Marc and {Dressler}, Alan and {Patel}, Brandon and {Cenko}, S. Bradley and {Graham}, Melissa L. and {Tucker}, Bradley E.},
        title = "{Multiple images of a highly magnified supernova formed by an early-type cluster galaxy lens}",
      journal = {Science},
     keywords = {ASTRONOMY, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = mar,
       volume = {347},
       number = {6226},
        pages = {1123-1126},
          doi = {10.1126/science.aaa3350},
archivePrefix = {arXiv},
       eprint = {1411.6009},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015Sci...347.1123K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Krisciunas2017,
       author = {{Krisciunas}, Kevin and {Contreras}, Carlos and {Burns}, Christopher R. and {Phillips}, M.~M. and {Stritzinger}, Maximilian D. and {Morrell}, Nidia and {Hamuy}, Mario and {Anais}, Jorge and {Boldt}, Luis and {Busta}, Luis and {Campillay}, Abdo and {Castell{\'o}n}, Sergio and {Folatelli}, Gast{\'o}n and {Freedman}, Wendy L. and {Gonz{\'a}lez}, Consuelo and {Hsiao}, Eric Y. and {Krzeminski}, Wojtek and {Persson}, Sven Eric and {Roth}, Miguel and {Salgado}, Francisco and {Ser{\'o}n}, Jacqueline and {Suntzeff}, Nicholas B. and {Torres}, Sim{\'o}n and {Filippenko}, Alexei V. and {Li}, Weidong and {Madore}, Barry F. and {DePoy}, D.~L. and {Marshall}, Jennifer L. and {Rheault}, Jean-Philippe and {Villanueva}, Steven},
        title = "{The Carnegie Supernova Project. I. Third Photometry Data Release of Low-redshift Type Ia Supernovae and Other White Dwarf Explosions}",
      journal = {\aj},
     keywords = {instrumentation: photometers, supernovae: general, surveys, techniques: photometric, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = nov,
       volume = {154},
       number = {5},
          eid = {211},
        pages = {211},
          doi = {10.3847/1538-3881/aa8df0},
archivePrefix = {arXiv},
       eprint = {1709.05146},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017AJ....154..211K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Lang2014a,
       author = {{Lang}, D.},
        title = "{unWISE: Unblurred Coadds of the WISE Imaging}",
      journal = {\aj},
     keywords = {methods: data analysis, surveys, techniques: image processing, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2014",
        month = "May",
       volume = {147},
          eid = {108},
        pages = {108},
          doi = {10.1088/0004-6256/147/5/108},
archivePrefix = {arXiv},
       eprint = {1405.0308},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2014AJ....147..108L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Leja2017a,
   author = {{Leja}, J. and {Johnson}, B.~D. and {Conroy}, C. and {van Dokkum}, P.~G. and {Byler}, N.},
   title = "{Deriving Physical Properties from Broadband Photometry with Prospector: Description of the Model and a Demonstration of its Accuracy Using 129 Galaxies in the Local Universe}",
   journal = {\apj},
   year = 2017,
   volume = 837,
   pages = {170},
   eprint = {1609.09073},
   doi = {10.3847/1538-4357/aa5ffe},
  adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...837..170L},
}

@ARTICLE{Leloudas2015,
       author = {{Leloudas}, G. and {Schulze}, S. and {Kr{\"u}hler}, T. and {Gorosabel}, J. and {Christensen}, L. and {Mehner}, A. and {de Ugarte Postigo}, A. and {Amor{\'\i}n}, R. and {Th{\"o}ne}, C.~C. and {Anderson}, J.~P. and {Bauer}, F.~E. and {Gallazzi}, A. and {He{\l}miniak}, K.~G. and {Hjorth}, J. and {Ibar}, E. and {Malesani}, D. and {Morell}, N. and {Vinko}, J. and {Wheeler}, J.~C.},
        title = "{Spectroscopy of superluminous supernova host galaxies. A preference of hydrogen-poor events for extreme emission line galaxies}",
      journal = {\mnras},
     keywords = {supernovae: general, galaxies: abundances, galaxies: starburst, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = may,
       volume = {449},
       number = {1},
        pages = {917-932},
          doi = {10.1093/mnras/stv320},
archivePrefix = {arXiv},
       eprint = {1409.8331},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.449..917L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lu2021,
       author = {{Lu}, J. and {Ashall}, C. and {Hsiao}, E.~Y. and {Hoeflich}, P. and {Galbany}, L. and {Baron}, E. and {Phillips}, M.~M. and {Contreras}, C. and {Burns}, C.~R. and {Suntzeff}, N.~B. and {Stritzinger}, M.~D. and {Anais}, J. and {Anderson}, J.~P. and {Brown}, P.~J. and {Busta}, L. and {Castell{\'o}n}, S. and {Davis}, S. and {Diamond}, T. and {Falco}, E. and {Gonzalez}, C. and {Hamuy}, M. and {Holmbo}, S. and {Holoien}, T.~W. -S. and {Krisciunas}, K. and {Kirshner}, R.~P. and {Kumar}, S. and {Kuncarayakti}, H. and {Marion}, G.~H. and {Morrell}, N. and {Persson}, S.~E. and {Piro}, A.~L. and {Prieto}, J.~L. and {Sand}, D.~J. and {Shahbandeh}, M. and {Shappee}, B.~J. and {Taddia}, F.},
        title = "{ASASSN-15hy: An Underluminous, Red 03fg-like Type Ia Supernova}",
      journal = {\apj},
     keywords = {White dwarf stars, Type Ia supernovae, Supernovae, 1799, 1728, 1668, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = oct,
       volume = {920},
       number = {2},
          eid = {107},
        pages = {107},
          doi = {10.3847/1538-4357/ac1606},
archivePrefix = {arXiv},
       eprint = {2107.08150},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...920..107L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Lunnan2014,
       author = {{Lunnan}, R. and {Chornock}, R. and {Berger}, E. and {Laskar}, T. and {Fong}, W. and {Rest}, A. and {Sanders}, N.~E. and {Challis}, P.~M. and {Drout}, M.~R. and {Foley}, R.~J. and {Huber}, M.~E. and {Kirshner}, R.~P. and {Leibler}, C. and {Marion}, G.~H. and {McCrum}, M. and {Milisavljevic}, D. and {Narayan}, G. and {Scolnic}, D. and {Smartt}, S.~J. and {Smith}, K.~W. and {Soderberg}, A.~M. and {Tonry}, J.~L. and {Burgett}, W.~S. and {Chambers}, K.~C. and {Flewelling}, H. and {Hodapp}, K.~W. and {Kaiser}, N. and {Magnier}, E.~A. and {Price}, P.~A. and {Wainscoat}, R.~J.},
        title = "{Hydrogen-poor Superluminous Supernovae and Long-duration Gamma-Ray Bursts Have Similar Host Galaxies}",
      journal = {\apj},
     keywords = {galaxies: abundances, galaxies: dwarf, galaxies: star formation, supernovae: general, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = jun,
       volume = {787},
       number = {2},
          eid = {138},
        pages = {138},
          doi = {10.1088/0004-637X/787/2/138},
archivePrefix = {arXiv},
       eprint = {1311.0026},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...787..138L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mainzer2014a,
       author = {{Mainzer}, A. and {Bauer}, J. and {Cutri}, R.~M. and {Grav}, T. and
         {Masiero}, J. and {Beck}, R. and {Clarkson}, P. and {Conrow}, T. and
         {Dailey}, J. and {Eisenhardt}, P. and {Fabinsky}, B. and
         {Fajardo-Acosta}, S. and {Fowler}, J. and {Gelino}, C. and
         {Grillmair}, C. and {Heinrichsen}, I. and {Kendall}, M. and
         {Kirkpatrick}, J. Davy and {Liu}, F. and {Masci}, F. and
         {McCallon}, H. and {Nugent}, C.~R. and {Papin}, M. and {Rice}, E. and
         {Royer}, D. and {Ryan}, T. and {Sevilla}, P. and {Sonnett}, S. and
         {Stevenson}, R. and {Thompson}, D.~B. and {Wheelock}, S. and
         {Wiemer}, D. and {Wittman}, M. and {Wright}, E. and {Yan}, L.},
        title = "{Initial Performance of the NEOWISE Reactivation Mission}",
      journal = {\apj},
     keywords = {comets: general, infrared: general, minor planets, asteroids: general, space vehicles, surveys, Astrophysics - Earth and Planetary Astrophysics},
         year = 2014,
        month = sep,
       volume = {792},
       number = {1},
          eid = {30},
        pages = {30},
          doi = {10.1088/0004-637X/792/1/30},
archivePrefix = {arXiv},
       eprint = {1406.6025},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...792...30M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Martin2005a,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...619L...1M},
	Author = {{Martin}, D.~C. and {Fanson}, J. and {Schiminovich}, D. and {Morrissey}, P. and {Friedman}, P.~G. and {Barlow}, T.~A. and {Conrow}, T. and {Grange}, R. and {Jelinsky}, P.~N. and {Milliard}, B. and {Siegmund}, O.~H.~W. and {Bianchi}, L. and {Byun}, Y.-I. and {Donas}, J. and {Forster}, K. and {Heckman}, T.~M. and {Lee}, Y.-W. and {Madore}, B.~F. and {Malina}, R.~F. and {Neff}, S.~G. and {Rich}, R.~M. and {Small}, T. and {Surber}, F. and {Szalay}, A.~S. and {Welsh}, B. and {Wyder}, T.~K.},
	Doi = {10.1086/426387},
	Eprint = {astro-ph/0411302},
	Journal = {\apj},
	Keywords = {Galaxies: Evolution, Galaxies: General, Space Vehicles: Instruments, Surveys, Ultraviolet: Galaxies, Ultraviolet: General},
	Month = jan,
	Pages = {L1},
	Title = {{The Galaxy Evolution Explorer: A Space Ultraviolet Survey Mission}},
	Volume = 619,
	Year = 2005,
	Bdsk-Url-1 = {http://dx.doi.org/10.1086/426387}}

@ARTICLE{Meisner2017a,
       author = {{Meisner}, Aaron M. and {Lang}, Dustin and {Schlegel}, David J.},
        title = "{Full-depth Coadds of the WISE and First-year NEOWISE-reactivation Images}",
      journal = {\aj},
     keywords = {infrared: general, methods: data analysis, surveys, techniques: image processing, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2017",
        month = "Jan",
       volume = {153},
          eid = {38},
        pages = {38},
          doi = {10.3847/1538-3881/153/1/38},
archivePrefix = {arXiv},
       eprint = {1603.05664},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2017AJ....153...38M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mockler2019,
       author = {{Mockler}, Brenna and {Guillochon}, James and {Ramirez-Ruiz}, Enrico},
        title = "{Weighing Black Holes Using Tidal Disruption Events}",
      journal = {\apj},
     keywords = {galaxies: active, quasars: supermassive black holes, stars: black holes, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = feb,
       volume = {872},
       number = {2},
          eid = {151},
        pages = {151},
          doi = {10.3847/1538-4357/ab010f},
archivePrefix = {arXiv},
       eprint = {1801.08221},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...872..151M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Nordin2014,
       author = {{Nordin}, J. and {Rubin}, D. and {Richard}, J. and {Rykoff}, E. and {Aldering}, G. and {Amanullah}, R. and {Atek}, H. and {Barbary}, K. and {Deustua}, S. and {Fakhouri}, H.~K. and {Fruchter}, A.~S. and {Goobar}, A. and {Hook}, I. and {Hsiao}, E.~Y. and {Huang}, X. and {Kneib}, J. -P. and {Lidman}, C. and {Meyers}, J. and {Perlmutter}, S. and {Saunders}, C. and {Spadafora}, A.~L. and {Suzuki}, N. and {Supernova Cosmology Project}},
        title = "{Lensed Type Ia supernovae as probes of cluster mass models}",
      journal = {\mnras},
     keywords = {gravitational lensing: strong, supernovae: general, galaxies: clusters: general, cosmology: observations, dark matter, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = may,
       volume = {440},
       number = {3},
        pages = {2742-2754},
          doi = {10.1093/mnras/stu376},
archivePrefix = {arXiv},
       eprint = {1312.2576},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.440.2742N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Magee2023,
       author = {{Magee}, M.~R. and {Sainz de Murieta}, A. and {Collett}, T.~E. and {Enzi}, W.},
        title = "{A search for gravitationally lensed supernovae within the Zwicky transient facility public survey}",
      journal = {\mnras},
     keywords = {gravitational lensing: strong, supernovae: general, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2023,
        month = oct,
       volume = {525},
       number = {1},
        pages = {542-560},
          doi = {10.1093/mnras/stad2263},
archivePrefix = {arXiv},
       eprint = {2303.15439},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023MNRAS.525..542M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Masci2019,
       author = {{Masci}, Frank J. and {Laher}, Russ R. and {Rusholme}, Ben and {Shupe}, David L. and {Groom}, Steven and {Surace}, Jason and {Jackson}, Edward and {Monkewitz}, Serge and {Beck}, Ron and {Flynn}, David and {Terek}, Scott and {Landry}, Walter and {Hacopians}, Eugean and {Desai}, Vandana and {Howell}, Justin and {Brooke}, Tim and {Imel}, David and {Wachter}, Stefanie and {Ye}, Quan-Zhi and {Lin}, Hsing-Wen and {Cenko}, S. Bradley and {Cunningham}, Virginia and {Rebbapragada}, Umaa and {Bue}, Brian and {Miller}, Adam A. and {Mahabal}, Ashish and {Bellm}, Eric C. and {Patterson}, Maria T. and {Juri{\'c}}, Mario and {Golkhou}, V. Zach and {Ofek}, Eran O. and {Walters}, Richard and {Graham}, Matthew and {Kasliwal}, Mansi M. and {Dekany}, Richard G. and {Kupfer}, Thomas and {Burdge}, Kevin and {Cannella}, Christopher B. and {Barlow}, Tom and {Van Sistine}, Angela and {Giomi}, Matteo and {Fremling}, Christoffer and {Blagorodnova}, Nadejda and {Levitan}, David and {Riddle}, Reed and {Smith}, Roger M. and {Helou}, George and {Prince}, Thomas A. and {Kulkarni}, Shrinivas R.},
        title = "{The Zwicky Transient Facility: Data Processing, Products, and Archive}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2019,
        month = jan,
       volume = {131},
       number = {995},
        pages = {018003},
          doi = {10.1088/1538-3873/aae8ac},
archivePrefix = {arXiv},
       eprint = {1902.01872},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PASP..131a8003M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@misc{Masci2023,
      title={A New Forced Photometry Service for the Zwicky Transient Facility}, 
      author={Frank J. Masci and Russ R. Laher and Benjamin Rusholme and David Shupe and Roberta Paladini and Steve Groom and Avery Wold and Adam A. Miller and Andrew Drake},
      year={2023},
      eprint={2305.16279},
      archivePrefix={arXiv},
      primaryClass={astro-ph.IM},
      url={https://arxiv.org/abs/2305.16279}, 
}


@ARTICLE{Millon2020,
       author = {{Millon}, M. and {Galan}, A. and {Courbin}, F. and {Treu}, T. and {Suyu}, S.~H. and {Ding}, X. and {Birrer}, S. and {Chen}, G.~C. -F. and {Shajib}, A.~J. and {Sluse}, D. and {Wong}, K.~C. and {Agnello}, A. and {Auger}, M.~W. and {Buckley-Geer}, E.~J. and {Chan}, J.~H.~H. and {Collett}, T. and {Fassnacht}, C.~D. and {Hilbert}, S. and {Koopmans}, L.~V.~E. and {Motta}, V. and {Mukherjee}, S. and {Rusu}, C.~E. and {Sonnenfeld}, A. and {Spiniello}, C. and {Van de Vyvere}, L.},
        title = "{TDCOSMO. I. An exploration of systematic uncertainties in the inference of H$_{0}$ from time-delay cosmography}",
      journal = {\aap},
     keywords = {gravitational lensing: strong, methods: data analysis, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = jul,
       volume = {639},
          eid = {A101},
        pages = {A101},
          doi = {10.1051/0004-6361/201937351},
archivePrefix = {arXiv},
       eprint = {1912.08027},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...639A.101M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mortsell2020,
       author = {{M{\"o}rtsell}, E. and {Johansson}, J. and {Dhawan}, S. and {Goobar}, A. and {Amanullah}, R. and {Goldstein}, D.~A.},
        title = "{Lens modelling of the strongly lensed Type Ia supernova iPTF16geu}",
      journal = {\mnras},
     keywords = {gravitational lensing: strong, distance scale, supernovae: individual, gravitational lensing: micro, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = aug,
       volume = {496},
       number = {3},
        pages = {3270-3280},
          doi = {10.1093/mnras/staa1600},
archivePrefix = {arXiv},
       eprint = {1907.06609},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.496.3270M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Nordin2019,
       author = {{Nordin}, J. and {Brinnel}, V. and {van Santen}, J. and {Bulla}, M. and {Feindt}, U. and {Franckowiak}, A. and {Fremling}, C. and {Gal-Yam}, A. and {Giomi}, M. and {Kowalski}, M. and {Mahabal}, A. and {Miranda}, N. and {Rauch}, L. and {Reusch}, S. and {Rigault}, M. and {Schulze}, S. and {Sollerman}, J. and {Stein}, R. and {Yaron}, O. and {van Velzen}, S. and {Ward}, C.},
        title = "{Transient processing and analysis using AMPEL: alert management, photometry, and evaluation of light curves}",
      journal = {\aap},
     keywords = {methods: data analysis, astronomical databases: miscellaneous, virtual observatory tools, supernovae: general, cosmology: observations, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2019,
        month = nov,
       volume = {631},
          eid = {A147},
        pages = {A147},
          doi = {10.1051/0004-6361/201935634},
archivePrefix = {arXiv},
       eprint = {1904.05922},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...631A.147N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Patel2014,
       author = {{Patel}, Brandon and {McCully}, Curtis and {Jha}, Saurabh W. and {Rodney}, Steven A. and {Jones}, David O. and {Graur}, Or and {Merten}, Julian and {Zitrin}, Adi and {Riess}, Adam G. and {Matheson}, Thomas and {Sako}, Masao and {Holoien}, Thomas W. -S. and {Postman}, Marc and {Coe}, Dan and {Bartelmann}, Matthias and {Balestra}, Italo and {Ben{\'\i}tez}, Narciso and {Bouwens}, Rychard and {Bradley}, Larry and {Broadhurst}, Tom and {Cenko}, S. Bradley and {Donahue}, Megan and {Filippenko}, Alexei V. and {Ford}, Holland and {Garnavich}, Peter and {Grillo}, Claudio and {Infante}, Leopoldo and {Jouvel}, St{\'e}phanie and {Kelson}, Daniel and {Koekemoer}, Anton and {Lahav}, Ofer and {Lemze}, Doron and {Maoz}, Dan and {Medezinski}, Elinor and {Melchior}, Peter and {Meneghetti}, Massimo and {Molino}, Alberto and {Moustakas}, John and {Moustakas}, Leonidas A. and {Nonino}, Mario and {Rosati}, Piero and {Seitz}, Stella and {Strolger}, Louis G. and {Umetsu}, Keiichi and {Zheng}, Wei},
        title = "{Three Gravitationally Lensed Supernovae behind CLASH Galaxy Clusters}",
      journal = {\apj},
     keywords = {cosmology: observations, galaxies: clusters: general, gravitational lensing: weak, supernovae: general, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = may,
       volume = {786},
       number = {1},
          eid = {9},
        pages = {9},
          doi = {10.1088/0004-637X/786/1/9},
archivePrefix = {arXiv},
       eprint = {1312.0943},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...786....9P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Patterson2019,
       author = {{Patterson}, Maria T. and {Bellm}, Eric C. and {Rusholme}, Ben and {Masci}, Frank J. and {Juric}, Mario and {Krughoff}, K. Simon and {Golkhou}, V. Zach and {Graham}, Matthew J. and {Kulkarni}, Shrinivas R. and {Helou}, George and {Zwicky Transient Facility Collaboration}},
        title = "{The Zwicky Transient Facility Alert Distribution System}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2019,
        month = jan,
       volume = {131},
       number = {995},
        pages = {018001},
          doi = {10.1088/1538-3873/aae904},
archivePrefix = {arXiv},
       eprint = {1902.02227},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PASP..131a8001P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Perley2016,
       author = {{Perley}, D.~A. and {Quimby}, R.~M. and {Yan}, L. and {Vreeswijk}, P.~M. and {De Cia}, A. and {Lunnan}, R. and {Gal-Yam}, A. and {Yaron}, O. and {Filippenko}, A.~V. and {Graham}, M.~L. and {Laher}, R. and {Nugent}, P.~E.},
        title = "{Host-galaxy Properties of 32 Low-redshift Superluminous Supernovae from the Palomar Transient Factory}",
      journal = {\apj},
     keywords = {galaxies: abundances, galaxies: dwarf, galaxies: photometry, supernovae: general, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = oct,
       volume = {830},
       number = {1},
          eid = {13},
        pages = {13},
          doi = {10.3847/0004-637X/830/1/13},
archivePrefix = {arXiv},
       eprint = {1604.08207},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...830...13P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Perley2020,
       author = {{Perley}, Daniel A. and {Fremling}, Christoffer and {Sollerman}, Jesper and {Miller}, Adam A. and {Dahiwale}, Aishwarya S. and {Sharma}, Yashvi and {Bellm}, Eric C. and {Biswas}, Rahul and {Brink}, Thomas G. and {Bruch}, Rachel J. and {De}, Kishalay and {Dekany}, Richard and {Drake}, Andrew J. and {Duev}, Dmitry A. and {Filippenko}, Alexei V. and {Gal-Yam}, Avishay and {Goobar}, Ariel and {Graham}, Matthew J. and {Graham}, Melissa L. and {Ho}, Anna Y.~Q. and {Irani}, Ido and {Kasliwal}, Mansi M. and {Kim}, Young-Lo and {Kulkarni}, S.~R. and {Mahabal}, Ashish and {Masci}, Frank J. and {Modak}, Shaunak and {Neill}, James D. and {Nordin}, Jakob and {Riddle}, Reed L. and {Soumagnac}, Maayane T. and {Strotjohann}, Nora L. and {Schulze}, Steve and {Taggart}, Kirsty and {Tzanidakis}, Anastasios and {Walters}, Richard S. and {Yan}, Lin},
        title = "{The Zwicky Transient Facility Bright Transient Survey. II. A Public Statistical Sample for Exploring Supernova Demographics}",
      journal = {\apj},
     keywords = {Supernovae, Catalogs, Surveys, Transient sources, Time domain astronomy, 1668, 205, 1671, 1851, 2109, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = nov,
       volume = {904},
       number = {1},
          eid = {35},
        pages = {35},
          doi = {10.3847/1538-4357/abbd98},
archivePrefix = {arXiv},
       eprint = {2009.01242},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...904...35P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Petrushevska2016,
       author = {{Petrushevska}, T. and {Amanullah}, R. and {Goobar}, A. and {Fabbro}, S. and {Johansson}, J. and {Kjellsson}, T. and {Lidman}, C. and {Paech}, K. and {Richard}, J. and {Dahle}, H. and {Ferretti}, R. and {Kneib}, J.~P. and {Limousin}, M. and {Nordin}, J. and {Stanishev}, V.},
        title = "{High-redshift supernova rates measured with the gravitational telescope A 1689}",
      journal = {\aap},
     keywords = {supernovae: general, gravitational lensing: strong, galaxies: star formation, galaxies: clusters: individual: A 1689, techniques: photometric, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2016,
        month = oct,
       volume = {594},
          eid = {A54},
        pages = {A54},
          doi = {10.1051/0004-6361/201628925},
archivePrefix = {arXiv},
       eprint = {1607.01617},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...594A..54P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Petrushevska2017,
       author = {{Petrushevska}, T. and {Amanullah}, R. and {Bulla}, M. and {Kromer}, M. and {Ferretti}, R. and {Goobar}, A. and {Papadogiannakis}, S.},
        title = "{Testing for redshift evolution of Type Ia supernovae using the strongly lensed PS1-10afx at z = 1.4}",
      journal = {\aap},
     keywords = {supernovae: individual: PS1-10afx, gravitational lensing: strong, supernovae: general, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = jul,
       volume = {603},
          eid = {A136},
        pages = {A136},
          doi = {10.1051/0004-6361/201730989},
archivePrefix = {arXiv},
       eprint = {1706.03770},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...603A.136P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pierel2023,
       author = {{Pierel}, J.~D.~R. and {Arendse}, N. and {Ertl}, S. and {Huang}, X. and {Moustakas}, L.~A. and {Schuldt}, S. and {Shajib}, A.~J. and {Shu}, Y. and {Birrer}, S. and {Bronikowski}, M. and {Hjorth}, J. and {Suyu}, S.~H. and {Agarwal}, S. and {Agnello}, A. and {Bolton}, A.~S. and {Chakrabarti}, S. and {Cold}, C. and {Courbin}, F. and {Della Costa}, J.~M. and {Dhawan}, S. and {Engesser}, M. and {Fox}, Ori D. and {Gall}, C. and {Gomez}, S. and {Goobar}, A. and {Jha}, S.~W. and {Jimenez}, C. and {Johansson}, J. and {Larison}, C. and {Li}, G. and {Marques-Chaves}, R. and {Mao}, S. and {Mazzali}, P.~A. and {Perez-Fournon}, I. and {Petrushevska}, T. and {Poidevin}, F. and {Rest}, A. and {Sheu}, W. and {Shirley}, R. and {Silver}, E. and {Storfer}, C. and {Strolger}, L.~G. and {Treu}, T. and {Wojtak}, R. and {Zenati}, Y.},
        title = "{LensWatch. I. Resolved HST Observations and Constraints on the Strongly Lensed Type Ia Supernova 2022qmx (``SN Zwicky'')}",
      journal = {\apj},
     keywords = {Type Ia supernovae, Strong gravitational lensing, 1728, 1643, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2023,
        month = may,
       volume = {948},
       number = {2},
          eid = {115},
        pages = {115},
          doi = {10.3847/1538-4357/acc7a6},
archivePrefix = {arXiv},
       eprint = {2211.03772},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023ApJ...948..115P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pierel2024,
       author = {{Pierel}, J.~D.~R. and {Newman}, A.~B. and {Dhawan}, S. and {Gu}, M. and {Joshi}, B.~A. and {Li}, T. and {Schuldt}, S. and {Strolger}, L.~G. and {Suyu}, S.~H. and {Caminha}, G.~B. and {Cohen}, S.~H. and {Diego}, J.~M. and {D{\'S}ilva}, J.~C.~J. and {Ertl}, S. and {Frye}, B.~L. and {Granata}, G. and {Grillo}, C. and {Koekemoer}, A.~M. and {Li}, J. and {Robotham}, A. and {Summers}, J. and {Treu}, T. and {Windhorst}, R.~A. and {Zitrin}, A. and {Agarwal}, S. and {Agrawal}, A. and {Arendse}, N. and {Belli}, S. and {Burns}, C. and {Ca{\~n}ameras}, R. and {Chakrabarti}, S. and {Chen}, W. and {Collett}, T.~E. and {Coulter}, D.~A. and {Ellis}, R.~S. and {Engesser}, M. and {Foo}, N. and {Fox}, O.~D. and {Gall}, C. and {Garuda}, N. and {Gezari}, S. and {Gomez}, S. and {Glazebrook}, K. and {Hjorth}, J. and {Huang}, X. and {Jha}, S.~W. and {Kamieneski}, P.~S. and {Kelly}, P. and {Larison}, C. and {Moustakas}, L.~A. and {Pascale}, M. and {P{\'e}rez-Fournon}, I. and {Petrushevska}, T. and {Poidevin}, F. and {Rest}, A. and {Shahbandeh}, M. and {Shajib}, A.~J. and {Siebert}, M. and {Storfer}, C. and {Talbot}, M. and {Wang}, Q. and {Wevers}, T. and {Zenati}, Y.},
        title = "{Lensed Type Ia Supernova ``Encore'' at z = 2: The First Instance of Two Multiply Imaged Supernovae in the Same Host Galaxy}",
      journal = {\apjl},
     keywords = {Gravitational lensing, Cosmology, Type Ia supernovae, Supernovae, Galaxy clusters, 670, 343, 1728, 1668, 584, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2024,
        month = jun,
       volume = {967},
       number = {2},
          eid = {L37},
        pages = {L37},
          doi = {10.3847/2041-8213/ad4648},
archivePrefix = {arXiv},
       eprint = {2404.02139},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024ApJ...967L..37P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Planck2020,
       author = {{Planck Collaboration} and {Aghanim}, N. and {Akrami}, Y. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Ballardini}, M. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartolo}, N. and {Basak}, S. and {Battye}, R. and {Benabed}, K. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bielewicz}, P. and {Bock}, J.~J. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bucher}, M. and {Burigana}, C. and {Butler}, R.~C. and {Calabrese}, E. and {Cardoso}, J. -F. and {Carron}, J. and {Challinor}, A. and {Chiang}, H.~C. and {Chluba}, J. and {Colombo}, L.~P.~L. and {Combet}, C. and {Contreras}, D. and {Crill}, B.~P. and {Cuttaia}, F. and {de Bernardis}, P. and {de Zotti}, G. and {Delabrouille}, J. and {Delouis}, J. -M. and {Di Valentino}, E. and {Diego}, J.~M. and {Dor{\'e}}, O. and {Douspis}, M. and {Ducout}, A. and {Dupac}, X. and {Dusini}, S. and {Efstathiou}, G. and {Elsner}, F. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Fantaye}, Y. and {Farhang}, M. and {Fergusson}, J. and {Fernandez-Cobos}, R. and {Finelli}, F. and {Forastieri}, F. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Frolov}, A. and {Galeotta}, S. and {Galli}, S. and {Ganga}, K. and {G{\'e}nova-Santos}, R.~T. and {Gerbino}, M. and {Ghosh}, T. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gratton}, S. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {Hamann}, J. and {Handley}, W. and {Hansen}, F.~K. and {Herranz}, D. and {Hildebrandt}, S.~R. and {Hivon}, E. and {Huang}, Z. and {Jaffe}, A.~H. and {Jones}, W.~C. and {Karakci}, A. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kiiveri}, K. and {Kim}, J. and {Kisner}, T.~S. and {Knox}, L. and {Krachmalnicoff}, N. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {Lamarre}, J. -M. and {Lasenby}, A. and {Lattanzi}, M. and {Lawrence}, C.~R. and {Le Jeune}, M. and {Lemos}, P. and {Lesgourgues}, J. and {Levrier}, F. and {Lewis}, A. and {Liguori}, M. and {Lilje}, P.~B. and {Lilley}, M. and {Lindholm}, V. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Ma}, Y. -Z. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maggio}, G. and {Maino}, D. and {Mandolesi}, N. and {Mangilli}, A. and {Marcos-Caballero}, A. and {Maris}, M. and {Martin}, P.~G. and {Martinelli}, M. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Matarrese}, S. and {Mauri}, N. and {McEwen}, J.~D. and {Meinhold}, P.~R. and {Melchiorri}, A. and {Mennella}, A. and {Migliaccio}, M. and {Millea}, M. and {Mitra}, S. and {Miville-Desch{\^e}nes}, M. -A. and {Molinari}, D. and {Montier}, L. and {Morgante}, G. and {Moss}, A. and {Natoli}, P. and {N{\o}rgaard-Nielsen}, H.~U. and {Pagano}, L. and {Paoletti}, D. and {Partridge}, B. and {Patanchon}, G. and {Peiris}, H.~V. and {Perrotta}, F. and {Pettorino}, V. and {Piacentini}, F. and {Polastri}, L. and {Polenta}, G. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reinecke}, M. and {Remazeilles}, M. and {Renzi}, A. and {Rocha}, G. and {Rosset}, C. and {Roudier}, G. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Ruiz-Granados}, B. and {Salvati}, L. and {Sandri}, M. and {Savelainen}, M. and {Scott}, D. and {Shellard}, E.~P.~S. and {Sirignano}, C. and {Sirri}, G. and {Spencer}, L.~D. and {Sunyaev}, R. and {Suur-Uski}, A. -S. and {Tauber}, J.~A. and {Tavagnacco}, D. and {Tenti}, M. and {Toffolatti}, L. and {Tomasi}, M. and {Trombetti}, T. and {Valenziano}, L. and {Valiviita}, J. and {Van Tent}, B. and {Vibert}, L. and {Vielva}, P. and {Villa}, F. and {Vittorio}, N. and {Wandelt}, B.~D. and {Wehus}, I.~K. and {White}, M. and {White}, S.~D.~M. and {Zacchei}, A. and {Zonca}, A.},
        title = "{Planck 2018 results. VI. Cosmological parameters}",
      journal = {\aap},
     keywords = {cosmic background radiation, cosmological parameters, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = sep,
       volume = {641},
          eid = {A6},
        pages = {A6},
          doi = {10.1051/0004-6361/201833910},
archivePrefix = {arXiv},
       eprint = {1807.06209},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...641A...6P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Quimby2013,
       author = {{Quimby}, Robert M. and {Werner}, Marcus C. and {Oguri}, Masamune and {More}, Surhud and {More}, Anupreeta and {Tanaka}, Masayuki and {Nomoto}, Ken'ichi and {Moriya}, Takashi J. and {Folatelli}, Gaston and {Maeda}, Keiichi and {Bersten}, Melina},
        title = "{Extraordinary Magnification of the Ordinary Type Ia Supernova PS1-10afx}",
      journal = {\apjl},
     keywords = {dark matter, gravitational lensing: micro, gravitational lensing: strong, supernovae: individual: PS1-10afx, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = may,
       volume = {768},
       number = {1},
          eid = {L20},
        pages = {L20},
          doi = {10.1088/2041-8205/768/1/L20},
archivePrefix = {arXiv},
       eprint = {1302.2785},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...768L..20Q},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Quimby2014,
       author = {{Quimby}, Robert M. and {Oguri}, Masamune and {More}, Anupreeta and {More}, Surhud and {Moriya}, Takashi J. and {Werner}, Marcus C. and {Tanaka}, Masayuki and {Folatelli}, Gaston and {Bersten}, Melina C. and {Maeda}, Keiichi and {Nomoto}, Ken'ichi},
        title = "{Detection of the Gravitational Lens Magnifying a Type Ia Supernova}",
      journal = {Science},
     keywords = {ASTRONOMY, Astronomy, Sociology, Chemistry, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = apr,
       volume = {344},
       number = {6182},
        pages = {396-399},
          doi = {10.1126/science.1250903},
archivePrefix = {arXiv},
       eprint = {1404.6014},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014Sci...344..396Q},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Refsdal1964,
       author = {{Refsdal}, S.},
        title = "{On the possibility of determining Hubble's parameter and the masses of galaxies from the gravitational lens effect}",
      journal = {\mnras},
         year = 1964,
        month = jan,
       volume = {128},
        pages = {307},
          doi = {10.1093/mnras/128.4.307},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1964MNRAS.128..307R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reusch2022,
       author = {{Reusch}, Simeon and {Stein}, Robert and {Kowalski}, Marek and {van Velzen}, Sjoert and {Franckowiak}, Anna and {Lunardini}, Cecilia and {Murase}, Kohta and {Winter}, Walter and {Miller-Jones}, James C.~A. and {Kasliwal}, Mansi M. and {Gilfanov}, Marat and {Garrappa}, Simone and {Paliya}, Vaidehi S. and {Ahumada}, Tom{\'a}s and {Anand}, Shreya and {Barbarino}, Cristina and {Bellm}, Eric C. and {Brinnel}, Val{\'e}ry and {Buson}, Sara and {Cenko}, S. Bradley and {Coughlin}, Michael W. and {De}, Kishalay and {Dekany}, Richard and {Frederick}, Sara and {Gal-Yam}, Avishay and {Gezari}, Suvi and {Giroletti}, Marcello and {Graham}, Matthew J. and {Karambelkar}, Viraj and {Kimura}, Shigeo S. and {Kong}, Albert K.~H. and {Kool}, Erik C. and {Laher}, Russ R. and {Medvedev}, Pavel and {Necker}, Jannis and {Nordin}, Jakob and {Perley}, Daniel A. and {Rigault}, Mickael and {Rusholme}, Ben and {Schulze}, Steve and {Schweyer}, Tassilo and {Singer}, Leo P. and {Sollerman}, Jesper and {Strotjohann}, Nora Linn and {Sunyaev}, Rashid and {van Santen}, Jakob and {Walters}, Richard and {Zhang}, B. Theodore and {Zimmerman}, Erez},
        title = "{Candidate Tidal Disruption Event AT2019fdr Coincident with a High-Energy Neutrino}",
      journal = {\prl},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2022,
        month = jun,
       volume = {128},
       number = {22},
          eid = {221101},
        pages = {221101},
          doi = {10.1103/PhysRevLett.128.221101},
archivePrefix = {arXiv},
       eprint = {2111.09390},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022PhRvL.128v1101R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@software{Reusch2023,
  author       = {Simeon Reusch},
  title        = {simeonreusch/fpbot: Release 1.1.2},
  month        = mar,
  year         = 2023,
  publisher    = {Zenodo},
  version      = {v1.1.2},
  doi          = {10.5281/zenodo.7781291},
  url          = {https://doi.org/10.5281/zenodo.7781291}
}

@ARTICLE{Rodney2015,
       author = {{Rodney}, Steven A. and {Patel}, Brandon and {Scolnic}, Daniel and {Foley}, Ryan J. and {Molino}, Alberto and {Brammer}, Gabriel and {Jauzac}, Mathilde and {Brada{\v{c}}}, Maru{\v{s}}a and {Broadhurst}, Tom and {Coe}, Dan and {Diego}, Jose M. and {Graur}, Or and {Hjorth}, Jens and {Hoag}, Austin and {Jha}, Saurabh W. and {Johnson}, Traci L. and {Kelly}, Patrick and {Lam}, Daniel and {McCully}, Curtis and {Medezinski}, Elinor and {Meneghetti}, Massimo and {Merten}, Julian and {Richard}, Johan and {Riess}, Adam and {Sharon}, Keren and {Strolger}, Louis-Gregory and {Treu}, Tommaso and {Wang}, Xin and {Williams}, Liliya L.~R. and {Zitrin}, Adi},
        title = "{Illuminating a Dark Lens : A Type Ia Supernova Magnified by the Frontier Fields Galaxy Cluster Abell 2744}",
      journal = {\apj},
     keywords = {galaxies: clusters: general, galaxies: clusters: individual: Abell 2744, gravitational lensing: strong, gravitational lensing: weak, supernovae: general, supernovae: individual: HFF14Tom, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2015,
        month = sep,
       volume = {811},
       number = {1},
          eid = {70},
        pages = {70},
          doi = {10.1088/0004-637X/811/1/70},
archivePrefix = {arXiv},
       eprint = {1505.06211},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...811...70R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rodney2021,
       author = {{Rodney}, Steven A. and {Brammer}, Gabriel B. and {Pierel}, Justin D.~R. and {Richard}, Johan and {Toft}, Sune and {O'Connor}, Kyle F. and {Akhshik}, Mohammad and {Whitaker}, Katherine E.},
        title = "{A gravitationally lensed supernova with an observable two-decade time delay}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = sep,
       volume = {5},
        pages = {1118-1125},
          doi = {10.1038/s41550-021-01450-9},
archivePrefix = {arXiv},
       eprint = {2106.08935},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021NatAs...5.1118R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ryu2020,
       author = {{Ryu}, Taeho and {Krolik}, Julian and {Piran}, Tsvi},
        title = "{Measuring Stellar and Black Hole Masses of Tidal Disruption Events}",
      journal = {\apj},
     keywords = {Black hole physics, Supermassive black holes, Gravitation, Stellar physics, Tidal disruption, Galaxy nuclei, 159, 1663, 661, 1621, 1696, 609, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = nov,
       volume = {904},
       number = {1},
          eid = {73},
        pages = {73},
          doi = {10.3847/1538-4357/abbf4d},
archivePrefix = {arXiv},
       eprint = {2007.13765},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...904...73R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{SaguesCarracedo2024,
       author = {{Sagu{\'e}s Carracedo}, A. and {Goobar}, A. and {M{\"o}rtsell}, E. and {Arendse}, N. and {Johansson}, J. and {Townsend}, A. and {Dhawan}, S. and {Nordin}, J. and {Sollerman}, J. and {Schulze}, S.},
        title = "{Detectability and Characterisation of Strongly Lensed Supernova Lightcurves in the Zwicky Transient Facility}",
      journal = {arXiv e-prints. Submitted to A\&A.},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2024,
        month = may,
          eid = {arXiv:2406.00052},
        pages = {arXiv:2406.00052},
          doi = {10.48550/arXiv.2406.00052},
archivePrefix = {arXiv},
       eprint = {2406.00052},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024arXiv240600052S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Saini2000,
       author = {{Saini}, Tarun Deep and {Raychaudhury}, Somak and {Shchekinov}, Yuri A.},
        title = "{Observing high-redshift supernovae in lensed galaxies}",
      journal = {\aap},
     keywords = {COSMOLOGY: GRAVITATIONAL LENSING, COSMOLOGY: DISTANCE SCALE, GALAXIES: CLUSTERS: GENERAL, STARS: SUPERNOVAE: GENERAL, Astrophysics},
         year = 2000,
        month = nov,
       volume = {363},
        pages = {349-354},
archivePrefix = {arXiv},
       eprint = {astro-ph/0002448},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000A&A...363..349S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{SainzdeMurieta2023,
       author = {{Sainz de Murieta}, Ana and {Collett}, Thomas E. and {Magee}, Mark R. and {Weisenbach}, Luke and {Krawczyk}, Coleman M. and {Enzi}, Wolfgang},
        title = "{Lensed Type Ia supernovae in light of SN Zwicky and iPTF16geu}",
      journal = {\mnras},
     keywords = {gravitational lensing: strong, transients: supernovae, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2023,
        month = dec,
       volume = {526},
       number = {3},
        pages = {4296-4307},
          doi = {10.1093/mnras/stad3031},
archivePrefix = {arXiv},
       eprint = {2307.12881},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023MNRAS.526.4296S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sarin2024,
       author = {{Sarin}, Nikhil and {H{\"u}bner}, Moritz and {Omand}, Conor M.~B. and {Setzer}, Christian N. and {Schulze}, Steve and {Adhikari}, Naresh and {Sagu{\'e}s-Carracedo}, Ana and {Galaudage}, Shanika and {Wallace}, Wendy F. and {Lamb}, Gavin P. and {Lin}, En-Tzu},
        title = "{REDBACK: a Bayesian inference software package for electromagnetic transients}",
      journal = {\mnras},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2024,
        month = jun,
       volume = {531},
       number = {1},
        pages = {1203-1227},
          doi = {10.1093/mnras/stae1238},
archivePrefix = {arXiv},
       eprint = {2308.12806},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024MNRAS.531.1203S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Schulze2018,
       author = {{Schulze}, S. and {Kr{\"u}hler}, T. and {Leloudas}, G. and {Gorosabel}, J. and {Mehner}, A. and {Buchner}, J. and {Kim}, S. and {Ibar}, E. and {Amor{\'\i}n}, R. and {Herrero-Illana}, R. and {Anderson}, J.~P. and {Bauer}, F.~E. and {Christensen}, L. and {de Pasquale}, M. and {de Ugarte Postigo}, A. and {Gallazzi}, A. and {Hjorth}, J. and {Morrell}, N. and {Malesani}, D. and {Sparre}, M. and {Stalder}, B. and {Stark}, A.~A. and {Th{\"o}ne}, C.~C. and {Wheeler}, J.~C.},
        title = "{Cosmic evolution and metal aversion in superluminous supernova host galaxies}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: high-redshift, galaxies: luminosity function, mass function, galaxies: starburst, galaxies: star formation, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = jan,
       volume = {473},
       number = {1},
        pages = {1258-1285},
          doi = {10.1093/mnras/stx2352},
archivePrefix = {arXiv},
       eprint = {1612.05978},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.473.1258S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Schulze2021a,
       author = {{Schulze}, Steve and {Yaron}, Ofer and {Sollerman}, Jesper and {Leloudas}, Giorgos and {Gal}, Amit and {Wright}, Angus H. and {Lunnan}, Ragnhild and {Gal-Yam}, Avishay and {Ofek}, Eran O. and {Perley}, Daniel A. and {Filippenko}, Alexei V. and {Kasliwal}, Mansi M. and {Kulkarni}, Shrinivas R. and {Neill}, James D. and {Nugent}, Peter E. and {Quimby}, Robert M. and {Sullivan}, Mark and {Strotjohann}, Nora Linn and {Arcavi}, Iair and {Ben-Ami}, Sagi and {Bianco}, Federica and {Bloom}, Joshua S. and {De}, Kishalay and {Fraser}, Morgan and {Fremling}, Christoffer U. and {Horesh}, Assaf and {Johansson}, Joel and {Kelly}, Patrick L. and {Kne{\v{z}}evi{\'c}}, Nikola and {Kne{\v{z}}evi{\'c}}, Sladjana and {Maguire}, Kate and {Nyholm}, Anders and {Papadogiannakis}, Sem{\'e}li and {Petrushevska}, Tanja and {Rubin}, Adam and {Yan}, Lin and {Yang}, Yi and {Adams}, Scott M. and {Bufano}, Filomena and {Clubb}, Kelsey I. and {Foley}, Ryan J. and {Green}, Yoav and {Harmanen}, Jussi and {Ho}, Anna Y.~Q. and {Hook}, Isobel M. and {Hosseinzadeh}, Griffin and {Howell}, D. Andrew and {Kong}, Albert K.~H. and {Kotak}, Rubina and {Matheson}, Thomas and {McCully}, Curtis and {Milisavljevic}, Dan and {Pan}, Yen-Chen and {Poznanski}, Dovi and {Shivvers}, Isaac and {van Velzen}, Sjoert and {Verbeek}, Kars K.},
        title = "{The Palomar Transient Factory Core-collapse Supernova Host-galaxy Sample. I. Host-galaxy Distribution Functions and Environment Dependence of Core-collapse Supernovae}",
      journal = {\apjs},
     keywords = {Supernovae, Core-collapse supernovae, Galaxies, Galactic and extragalactic astronomy, 1668, 304, 573, 563, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = aug,
       volume = {255},
       number = {2},
          eid = {29},
        pages = {29},
          doi = {10.3847/1538-4365/abff5e},
archivePrefix = {arXiv},
       eprint = {2008.05988},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJS..255...29S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schulze2024,
       author = {{Schulze}, Steve and {Fransson}, Claes and {Kozyreva}, Alexandra and {Chen}, Ting-Wan and {Yaron}, Ofer and {Jerkstrand}, Anders and {Gal-Yam}, Avishay and {Sollerman}, Jesper and {Yan}, Lin and {Kangas}, Tuomas and {Leloudas}, Giorgos and {Omand}, Conor M.~B. and {Smartt}, Stephen J. and {Yang}, Yi and {Nicholl}, Matt and {Sarin}, Nikhil and {Yao}, Yuhan and {Brink}, Thomas G. and {Sharon}, Amir and {Rossi}, Andrea and {Chen}, Ping and {Chen}, Zhihao and {Cikota}, Aleksandar and {De}, Kishalay and {Drake}, Andrew J. and {Filippenko}, Alexei V. and {Fremling}, Christoffer and {Fr{\'e}our}, Laurane and {Fynbo}, Johan P.~U. and {Ho}, Anna Y.~Q. and {Inserra}, Cosimo and {Irani}, Ido and {Kuncarayakti}, Hanindyo and {Lunnan}, Ragnhild and {Mazzali}, Paolo and {Ofek}, Eran O. and {Palazzi}, Eliana and {Perley}, Daniel A. and {Pursiainen}, Miika and {Rothberg}, Barry and {Shingles}, Luke J. and {Smith}, Ken and {Taggart}, Kirsty and {Tartaglia}, Leonardo and {Zheng}, WeiKang and {Anderson}, Joseph P. and {Cassara}, Letizia and {Christensen}, Eric and {George Djorgovski}, S. and {Galbany}, Llu{\'\i}s and {Gkini}, Anamaria and {Graham}, Matthew J. and {Gromadzki}, Mariusz and {Groom}, Steven L. and {Hiramatsu}, Daichi and {Andrew Howell}, D. and {Kasliwal}, Mansi M. and {McCully}, Curtis and {M{\"u}ller-Bravo}, Tom{\'a}s E. and {Paiano}, Simona and {Paraskeva}, Emmanouela and {Pessi}, Priscila J. and {Polishook}, David and {Rau}, Arne and {Rigault}, Mickael and {Rusholme}, Ben},
        title = "{1100 days in the life of the supernova 2018ibb. The best pair-instability supernova candidate, to date}",
      journal = {\aap},
     keywords = {supernovae: individual: SN 2018ibb, supernovae: individual: ATLAS18unu, supernovae: individual: Gaia19cvo, supernovae: individual: PS19crg, supernovae: individual: ZTF18acenqto, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2024,
        month = mar,
       volume = {683},
          eid = {A223},
        pages = {A223},
          doi = {10.1051/0004-6361/202346855},
archivePrefix = {arXiv},
       eprint = {2305.05796},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024A&A...683A.223S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Schwarz1978,
       author = {{Schwarz}, Gideon},
        title = "{Estimating the Dimension of a Model}",
      journal = {Annals of Statistics},
         year = 1978,
        month = jul,
       volume = {6},
       number = {2},
        pages = {461-464},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1978AnSta...6..461S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Shajib2020,
       author = {{Shajib}, A.~J. and {Birrer}, S. and {Treu}, T. and {Agnello}, A. and {Buckley-Geer}, E.~J. and {Chan}, J.~H.~H. and {Christensen}, L. and {Lemon}, C. and {Lin}, H. and {Millon}, M. and {Poh}, J. and {Rusu}, C.~E. and {Sluse}, D. and {Spiniello}, C. and {Chen}, G.~C. -F. and {Collett}, T. and {Courbin}, F. and {Fassnacht}, C.~D. and {Frieman}, J. and {Galan}, A. and {Gilman}, D. and {More}, A. and {Anguita}, T. and {Auger}, M.~W. and {Bonvin}, V. and {McMahon}, R. and {Meylan}, G. and {Wong}, K.~C. and {Abbott}, T.~M.~C. and {Annis}, J. and {Avila}, S. and {Bechtol}, K. and {Brooks}, D. and {Brout}, D. and {Burke}, D.~L. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Carretero}, J. and {Castander}, F.~J. and {Costanzi}, M. and {da Costa}, L.~N. and {De Vicente}, J. and {Desai}, S. and {Dietrich}, J.~P. and {Doel}, P. and {Drlica-Wagner}, A. and {Evrard}, A.~E. and {Finley}, D.~A. and {Flaugher}, B. and {Fosalba}, P. and {Garc{\'\i}a-Bellido}, J. and {Gerdes}, D.~W. and {Gruen}, D. and {Gruendl}, R.~A. and {Gschwend}, J. and {Gutierrez}, G. and {Hollowood}, D.~L. and {Honscheid}, K. and {Huterer}, D. and {James}, D.~J. and {Jeltema}, T. and {Krause}, E. and {Kuropatkin}, N. and {Li}, T.~S. and {Lima}, M. and {MacCrann}, N. and {Maia}, M.~A.~G. and {Marshall}, J.~L. and {Melchior}, P. and {Miquel}, R. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Plazas}, A.~A. and {Romer}, A.~K. and {Roodman}, A. and {Sako}, M. and {Sanchez}, E. and {Santiago}, B. and {Scarpine}, V. and {Schubnell}, M. and {Scolnic}, D. and {Serrano}, S. and {Sevilla-Noarbe}, I. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Tarle}, G. and {Thomas}, D. and {Walker}, A.~R. and {Zhang}, Y.},
        title = "{STRIDES: a 3.9 per cent measurement of the Hubble constant from the strong lens system DES J0408-5354}",
      journal = {\mnras},
     keywords = {gravitational lensing: strong, cosmological parameters, distance scale, cosmology: observations, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = jun,
       volume = {494},
       number = {4},
        pages = {6072-6102},
          doi = {10.1093/mnras/staa828},
archivePrefix = {arXiv},
       eprint = {1910.06306},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.494.6072S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Sharma2023,
       author = {{Sharma}, Yashvi and {Sollerman}, Jesper and {Fremling}, Christoffer and {Kulkarni}, Shrinivas R. and {De}, Kishalay and {Irani}, Ido and {Schulze}, Steve and {Strotjohann}, Nora Linn and {Gal-Yam}, Avishay and {Maguire}, Kate and {Perley}, Daniel A. and {Bellm}, Eric C. and {Kool}, Erik C. and {Brink}, Thomas G. and {Bruch}, Rachel and {Deckers}, Maxime and {Dekany}, Richard and {Dugas}, Alison and {Filippenko}, Alexei V. and {Goldwasser}, Samantha and {Graham}, Matthew J. and {Graham}, Melissa L. and {Groom}, Steven L. and {Hankins}, Matt and {Jencson}, Jacob and {Johansson}, Joel P. and {Karambelkar}, Viraj and {Kasliwal}, Mansi M. and {Masci}, Frank J. and {Medford}, Michael S. and {Neill}, James D. and {Nir}, Guy and {Riddle}, Reed L. and {Rigault}, Mickael and {Schweyer}, Tassilo and {Terwel}, Jacco H. and {Yan}, Lin and {Yang}, Yi and {Yao}, Yuhan},
        title = "{A Systematic Study of Ia-CSM Supernovae from the ZTF Bright Transient Survey}",
      journal = {\apj},
     keywords = {Supernovae, Type Ia supernovae, 1668, 1728, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2023,
        month = may,
       volume = {948},
       number = {1},
          eid = {52},
        pages = {52},
          doi = {10.3847/1538-4357/acbc16},
archivePrefix = {arXiv},
       eprint = {2301.04637},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023ApJ...948...52S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Shu2018,
       author = {{Shu}, Yiping and {Bolton}, Adam S. and {Mao}, Shude and {Kang}, Xi and {Li}, Guoliang and {Soraisam}, Monika},
        title = "{Prediction of Supernova Rates in Known Galaxy-Galaxy Strong-lens Systems}",
      journal = {\apj},
     keywords = {cosmology: observations, gravitational lensing: strong, supernovae: general, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = sep,
       volume = {864},
       number = {1},
          eid = {91},
        pages = {91},
          doi = {10.3847/1538-4357/aad5ea},
archivePrefix = {arXiv},
       eprint = {1803.07569},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...864...91S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Skrutskie2006a,
   author = {{Skrutskie}, M.~F. and {Cutri}, R.~M. and {Stiening}, R. and 
	{Weinberg}, M.~D. and {Schneider}, S. and {Carpenter}, J.~M. and 
	{Beichman}, C. and {Capps}, R. and {Chester}, T. and {Elias}, J. and 
	{Huchra}, J. and {Liebert}, J. and {Lonsdale}, C. and {Monet}, D.~G. and 
	{Price}, S. and {Seitzer}, P. and {Jarrett}, T. and {Kirkpatrick}, J.~D. and 
	{Gizis}, J.~E. and {Howard}, E. and {Evans}, T. and {Fowler}, J. and 
	{Fullmer}, L. and {Hurt}, R. and {Light}, R. and {Kopan}, E.~L. and 
	{Marsh}, K.~A. and {McCallon}, H.~L. and {Tam}, R. and {Van Dyk}, S. and 
	{Wheelock}, S.},
    title = "{The Two Micron All Sky Survey (2MASS)}",
  journal = {\aj},
 keywords = {Catalogs, Infrared: General, Surveys},
     year = 2006,
    month = feb,
   volume = 131,
    pages = {1163-1183},
      doi = {10.1086/498708},
   adsurl = {http://adsabs.harvard.edu/abs/2006AJ....131.1163S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Smith2007,
       author = {{Smith}, Nathan and {Li}, Weidong and {Foley}, Ryan J. and {Wheeler}, J. Craig and {Pooley}, David and {Chornock}, Ryan and {Filippenko}, Alexei V. and {Silverman}, Jeffrey M. and {Quimby}, Robert and {Bloom}, Joshua S. and {Hansen}, Charles},
        title = "{SN 2006gy: Discovery of the Most Luminous Supernova Ever Recorded, Powered by the Death of an Extremely Massive Star like {\ensuremath{\eta}} Carinae}",
      journal = {\apj},
     keywords = {Stars: Circumstellar Matter, Stars: Evolution, supernovae: individual (SN 2006gy), Astrophysics},
         year = 2007,
        month = sep,
       volume = {666},
       number = {2},
        pages = {1116-1128},
          doi = {10.1086/519949},
archivePrefix = {arXiv},
       eprint = {astro-ph/0612617},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...666.1116S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@software{sncosmo,
  author       = {Barbary, Kyle and
                  Bailey, Stephen and
                  Barentsen, Geert and
                  Barclay, Tom and
                  Biswas, Rahul and
                  Boone, Kyle and
                  Craig, Matt and
                  Feindt, Ulrich and
                  Friesen, Brian and
                  Goldstein, Danny and
                  Jha, Saurabh W. and
                  Jones, David O. and
                  Mondon, Florian and
                  Papadogiannakis, Seméli and
                  Perrefort, Daniel and
                  Pierel, Justin and
                  Rodney, Steve and
                  Rose, Benjamin and
                  Saunders, Clare and
                  Sipőcz, Brigitta and
                  Sofiatti, Caroline and
                  Thomas, Rollin C. and
                  van Santen, Jakob and
                  Vincenzi, Maria and
                  Wang, David and
                  Wood-Vasey, Michael},
  title        = {SNCosmo},
  month        = sep,
  year         = 2022,
  publisher    = {Zenodo},
  version      = {v2.9.0},
  doi          = {10.5281/zenodo.7117347},
  url          = {https://doi.org/10.5281/zenodo.7117347}
}

@ARTICLE{Sonnenfeld2020,
       author = {{Sonnenfeld}, A. and {Verma}, A. and {More}, A. and {Beaten}, E. and {MacMillan}, C. and {Wong}, K.~C. and {Chan}, J.~H.~H. and {Jaelani}, A.~T. and {Lee}, C. and {Oguri}, M. and {Rusu}, C.~E. and {Veldthuis}, M. and {Trouille}, L. and {Marshall}, P.~J. and {Hutchings}, R. and {Allen}, C. and {O'Donnell}, J. and {Cornen}, C. and {Davis}, C.~P. and {McMaster}, A. and {Lintott}, C. and {Miller}, G.},
        title = "{VizieR Online Data Catalog: SuGOHI VI. List up to 2020 (Sonnenfeld+, 2020)}",
      journal = {VizieR Online Data Catalog},
     keywords = {Gravitational lensing, Redshifts},
         year = 2020,
        month = aug,
          eid = {J/A+A/642/A148},
        pages = {J/A+A/642/A148},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020yCat..36420148S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Soumagnac2018,
       author = {{Soumagnac}, Maayane T. and {Ofek}, Eran O.},
        title = "{catsHTM: A Tool for Fast Accessing and Cross-matching Large Astronomical Catalogs}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = jul,
       volume = {130},
       number = {989},
        pages = {075002},
          doi = {10.1088/1538-3873/aac410},
archivePrefix = {arXiv},
       eprint = {1805.02666},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018PASP..130g5002S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Speagle2020a,
       author = {{Speagle}, Joshua S.},
        title = "{DYNESTY: a dynamic nested sampling package for estimating Bayesian posteriors and evidences}",
      journal = {\mnras},
     keywords = {methods: data analysis, methods: statistical, Astrophysics - Instrumentation and Methods for Astrophysics, Statistics - Computation},
         year = 2020,
        month = apr,
       volume = {493},
       number = {3},
        pages = {3132-3158},
          doi = {10.1093/mnras/staa278},
archivePrefix = {arXiv},
       eprint = {1904.02180},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.493.3132S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sullivan2000,
       author = {{Sullivan}, Mark and {Ellis}, Richard and {Nugent}, Peter and {Smail}, Ian and {Madau}, Piero},
        title = "{A strategy for finding gravitationally lensed distant supernovae}",
      journal = {\mnras},
     keywords = {SUPERNOVAE: GENERAL, GALAXIES: CLUSTERS: GENERAL, COSMOLOGY: OBSERVATIONS, GRAVITATIONAL LENSING, Astrophysics},
         year = 2000,
        month = dec,
       volume = {319},
       number = {2},
        pages = {549-556},
          doi = {10.1046/j.1365-8711.2000.03875.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0007228},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000MNRAS.319..549S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Taubenberger2011,
       author = {{Taubenberger}, S. and {Benetti}, S. and {Childress}, M. and {Pakmor}, R. and {Hachinger}, S. and {Mazzali}, P.~A. and {Stanishev}, V. and {Elias-Rosa}, N. and {Agnoletto}, I. and {Bufano}, F. and {Ergon}, M. and {Harutyunyan}, A. and {Inserra}, C. and {Kankare}, E. and {Kromer}, M. and {Navasardyan}, H. and {Nicolas}, J. and {Pastorello}, A. and {Prosperi}, E. and {Salgado}, F. and {Sollerman}, J. and {Stritzinger}, M. and {Turatto}, M. and {Valenti}, S. and {Hillebrandt}, W.},
        title = "{High luminosity, slow ejecta and persistent carbon lines: SN 2009dc challenges thermonuclear explosion scenarios}",
      journal = {\mnras},
     keywords = {supernovae: general, supernovae: individual: SN 2006gz, supernovae: individual: SN 2007if, supernovae: individual: SN 2009dc, galaxies: individual: UGC 10063, galaxies: individual: UGC 10064, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = apr,
       volume = {412},
       number = {4},
        pages = {2735-2762},
          doi = {10.1111/j.1365-2966.2010.18107.x},
archivePrefix = {arXiv},
       eprint = {1011.5665},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.412.2735T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wevers2017,
       author = {{Wevers}, Thomas and {van Velzen}, Sjoert and {Jonker}, Peter G. and {Stone}, Nicholas C. and {Hung}, Tiara and {Onori}, Francesca and {Gezari}, Suvi and {Blagorodnova}, Nadejda},
        title = "{Black hole masses of tidal disruption event host galaxies}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, galaxies: bulges, galaxies: fundamental parameters, galaxies: kinematics and dynamics, galaxies: nuclei, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = oct,
       volume = {471},
       number = {2},
        pages = {1694-1708},
          doi = {10.1093/mnras/stx1703},
archivePrefix = {arXiv},
       eprint = {1706.08965},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.471.1694W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@software{Williamsnessai,
   author       = {Michael J. Williams},
   title        = {nessai: Nested Sampling with Artificial Intelligence},
   month        = feb,
   year         = 2021,
   publisher    = {Zenodo},
   version      = {latest},
   doi          = {10.5281/zenodo.4550693},
   url          = {https://doi.org/10.5281/zenodo.4550693}
 }

 @article{Williams2021,
   author = "Williams, Michael J. and Veitch, John and Messenger, Chris",
   title = "{Nested sampling with normalizing flows for gravitational-wave inference}",
   eprint = "2102.11056",
   archivePrefix = "arXiv",
   primaryClass = "gr-qc",
   doi = "10.1103/PhysRevD.103.103006",
   journal = "Phys. Rev. D",
   volume = "103",
   number = "10",
   pages = "103006",
   year = "2021"
}

@article{Williams2023,
   author = "Williams, Michael J. and Veitch, John and Messenger, Chris",
   title = "{Importance nested sampling with normalising flows}",
   eprint = "2302.08526",
   archivePrefix = "arXiv",
   primaryClass = "astro-ph.IM",
   reportNumber = "LIGO-P2200283",
   month = "2",
   year = "2023"
}


@ARTICLE{Wojtak2019,
       author = {{Wojtak}, Rados{\l}aw and {Hjorth}, Jens and {Gall}, Christa},
        title = "{Magnified or multiply imaged? - Search strategies for gravitationally lensed supernovae in wide-field surveys}",
      journal = {\mnras},
     keywords = {gravitational lensing: strong, methods: statistical, supernovae: general, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2019,
        month = aug,
       volume = {487},
       number = {3},
        pages = {3342-3355},
          doi = {10.1093/mnras/stz1516},
archivePrefix = {arXiv},
       eprint = {1903.07687},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.487.3342W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wong2020,
       author = {{Wong}, Kenneth C. and {Suyu}, Sherry H. and {Chen}, Geoff C. -F. and {Rusu}, Cristian E. and {Millon}, Martin and {Sluse}, Dominique and {Bonvin}, Vivien and {Fassnacht}, Christopher D. and {Taubenberger}, Stefan and {Auger}, Matthew W. and {Birrer}, Simon and {Chan}, James H.~H. and {Courbin}, Frederic and {Hilbert}, Stefan and {Tihhonova}, Olga and {Treu}, Tommaso and {Agnello}, Adriano and {Ding}, Xuheng and {Jee}, Inh and {Komatsu}, Eiichiro and {Shajib}, Anowar J. and {Sonnenfeld}, Alessandro and {Blandford}, Roger D. and {Koopmans}, L{\'e}on V.~E. and {Marshall}, Philip J. and {Meylan}, Georges},
        title = "{H0LiCOW - XIII. A 2.4 per cent measurement of H$_{0}$ from lensed quasars: 5.3{\ensuremath{\sigma}} tension between early- and late-Universe probes}",
      journal = {\mnras},
     keywords = {gravitational lensing: strong, cosmological parameters, distance scale, cosmology: observations, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = oct,
       volume = {498},
       number = {1},
        pages = {1420-1439},
          doi = {10.1093/mnras/stz3094},
archivePrefix = {arXiv},
       eprint = {1907.04869},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.498.1420W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Woosley2010,
       author = {{Woosley}, S.~E.},
        title = "{Bright Supernovae from Magnetar Birth}",
      journal = {\apjl},
     keywords = {hydrodynamics, shock waves, supernovae: general, turbulence, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2010,
        month = aug,
       volume = {719},
       number = {2},
        pages = {L204-L207},
          doi = {10.1088/2041-8205/719/2/L204},
archivePrefix = {arXiv},
       eprint = {0911.0698},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...719L.204W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{Wright2010a,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2010AJ....140.1868W},
	Archiveprefix = {arXiv},
	Author = {{Wright}, E.~L. and {Eisenhardt}, P.~R.~M. and {Mainzer}, A.~K. and {Ressler}, M.~E. and {Cutri}, R.~M. and {Jarrett}, T. and {Kirkpatrick}, J.~D. and {Padgett}, D. and {McMillan}, R.~S. and {Skrutskie}, M. and {Stanford}, S.~A. and {Cohen}, M. and {Walker}, R.~G. and {Mather}, J.~C. and {Leisawitz}, D. and {Gautier}, III, T.~N. and {McLean}, I. and {Benford}, D. and {Lonsdale}, C.~J. and {Blain}, A. and {Mendez}, B. and {Irace}, W.~R. and {Duval}, V. and {Liu}, F. and {Royer}, D. and {Heinrichsen}, I. and {Howard}, J. and {Shannon}, M. and {Kendall}, M. and {Walsh}, A.~L. and {Larsen}, M. and {Cardon}, J.~G. and {Schick}, S. and {Schwalm}, M. and {Abid}, M. and {Fabinsky}, B. and {Naes}, L. and {Tsai}, C.-W.},
	Doi = {10.1088/0004-6256/140/6/1868},
	Eid = {1868},
	Eprint = {1008.0031},
	Journal = {\aj},
	Keywords = {infrared: general, space vehicles, surveys},
	Month = dec,
	Pages = {1868-1881},
	Primaryclass = {astro-ph.IM},
	Title = {{The Wide-field Infrared Survey Explorer (WISE): Mission Description and Initial On-orbit Performance}},
	Volume = 140,
	Year = 2010,
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/0004-6256/140/6/1868}}

@ARTICLE{Wright2016a,
   author = {{Wright}, A.~H. and {Robotham}, A.~S.~G. and {Bourne}, N. and 
	{Driver}, S.~P. and {Dunne}, L. and {Maddox}, S.~J. and {Alpaslan}, M. and 
	{Andrews}, S.~K. and {Bauer}, A.~E. and {Bland-Hawthorn}, J. and 
	{Brough}, S. and {Brown}, M.~J.~I. and {Clarke}, C. and {Cluver}, M. and 
	{Davies}, L.~J.~M. and {Grootes}, M.~W. and {Holwerda}, B.~W. and 
	{Hopkins}, A.~M. and {Jarrett}, T.~H. and {Kafle}, P.~R. and 
	{Lange}, R. and {Liske}, J. and {Loveday}, J. and {Moffett}, A.~J. and 
	{Norberg}, P. and {Popescu}, C.~C. and {Smith}, M. and {Taylor}, E.~N. and 
	{Tuffs}, R.~J. and {Wang}, L. and {Wilkins}, S.~M.},
    title = "{Galaxy And Mass Assembly: accurate panchromatic photometry from optical priors using LAMBDAR}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1604.01923},
 keywords = {techniques: photometric, astronomical data bases: miscellaneous, galaxies: evolution, galaxies: general, galaxies: photometry},
     year = 2016,
    month = jul,
   volume = 460,
    pages = {765},
      doi = {10.1093/mnras/stw832},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.460..765W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yang2022,
       author = {{Yang}, Jiawen and {Wang}, Lifan and {Suntzeff}, Nicholas and {Hu}, Lei and {Aldoroty}, Lauren and {Brown}, Peter J. and {Krisciunas}, Kevin and {Arcavi}, Iair and {Burke}, Jamison and {Galbany}, Llu{\'\i}s and {Hiramatsu}, Daichi and {Hosseinzadeh}, Griffin and {Howell}, D. Andrew and {McCully}, Curtis and {Pellegrino}, Craig and {Valenti}, Stefano},
        title = "{Using 1991T/1999aa-like Type Ia Supernovae as Standardizable Candles}",
      journal = {\apj},
     keywords = {Supernovae, Type Ia supernovae, 1668, 1728, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2022,
        month = oct,
       volume = {938},
       number = {1},
          eid = {83},
        pages = {83},
          doi = {10.3847/1538-4357/ac8c97},
archivePrefix = {arXiv},
       eprint = {2209.06301},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022ApJ...938...83Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Yao2022,
       author = {{Yao}, Y. and {Somalwar}, J. and {Hammerstein}, E. and {Gezari}, S. and {Velzen}, S.~V. and {Ravi}, V.},
        title = "{ZTF Transient Classification Report for 2022-04-09}",
      journal = {Transient Name Server Classification Report},
     keywords = {Transient, 2021uvz, AT2021uvz, AT 2021uvz},
         year = 2022,
        month = apr,
       volume = {2022-925},
        pages = {1},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022TNSCR.925....1Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
